Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition

Human Activity Recognition (HAR) using on-body devices identifies specific human actions in unconstrained environments. HAR is challenging due to the inter and intra-variance of human movements; moreover, annotated datasets from on-body devices are scarce. This problem is mainly due to the difficulty of data creation, i.e., recording, expensive annotation, and lack of standard definitions of human activities. Previous works demonstrated that transfer learning is a good strategy for addressing scenarios with scarce data. However, the scarcity of annotated on-body device datasets remains. This paper proposes using datasets intended for human-pose estimation as a source for transfer learning; specifically, it deploys sequences of annotated pixel coordinates of human joints from video datasets for HAR and human pose estimation. We pre-train a deep architecture on four benchmark video-based source datasets. Finally, an evaluation is carried out on three on-body device datasets improving HAR performance.

==> Images/preambel.tex <==
% Add Packages
% -------------------------------------------------------------------
% URLs
\usepackage{url}

% -------------------------------------------------------------------
% Misc Utility
\usepackage[cmex10]{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{eqparbox}

% -------------------------------------------------------------------
% Grafikpakete einbinden
\usepackage{amssymb}
\usepackage{flafter}
\usepackage{listings}

% -------------------------------------------------------------------
% Korrekte Darstellung der Umlaute
\usepackage[T1]{fontenc}
\usepackage{ae,aecompl}
\usepackage[utf8]{inputenc}
\usepackage[english,german,ngerman]{babel}

% -------------------------------------------------------------------
% Anführungszeichen
\usepackage[babel,german=quotes]{csquotes}

% -------------------------------------------------------------------
% Classic thesis:
\usepackage{classicthesis-ldpkg} 
% Options for classicthesis.sty:
\usepackage[eulerchapternumbers,subfig,beramono,eulermath,parts]{classicthesis}

% -------------------------------------------------------------------
% Setup and Finetuning
\newlength{\abcd} % for ab..z string length calculation
\newcommand{\myfloatalign}{\centering} % how all the floats will be aligned
\setlength{\extrarowheight}{3pt} % increase table row height

% -------------------------------------------------------------------
%Equation and figure numbering
\numberwithin{equation}{section} 
%sets equation numbers <chapter>.<section>.<index>
\numberwithin{table}{section} 
%sets equation numbers <chapter>.<section>.<index>
\numberwithin{figure}{section} 
%sets figure numbers <chapter>.<section>.<index>

% Captions look and feel
% -------------------------------------------------------------------
\captionsetup{format=hang,font=small}

\usepackage{tikz} % must be imported after classicthesis-ldpkg


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Tables/gestures_cnn.tex <==
\begin{table}
%\centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Ges}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[10, 30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN_{Ges}$, trained on the training set of the Opportunity-Gestures, denotes the baseline. Std $wF1[\%]$ lies around $0.01$. The performance of the $tCNN-IMU_{D_s}^{MM}$ is similar, thus, not shown.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c c|c}
        \hline
        \multicolumn{10}{c}{\bm{$tCNN_{D_s}^{Ges}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn}  & 
        \multicolumn{2}{c|}{D$_s$=NTU}  & 
        \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\ 
        [0.1em]
        \hline
        \hline
        $c_{1}$     & \textbf{88.66} & \textbf{89.05} &\textbf{88.82}  & \textbf{88.72}  &      \textbf{88.77}   &  \textbf{88.96}   &  \textbf{89.19} &       \textbf{89.03} & \multirow{4}{*}{87.36}     \\  
        %\cline{2-9}
        $c_{1,2}$  & \textbf{88.83} & \textbf{88.97}  & \textbf{88.75}  & \textbf{88.80} & \textbf{88.67} & \textbf{88.53} &  \textbf{88.93} &  \textbf{88.81}& \\  
        %\cline{2-9}
        $c_{1-3}$  &  \textbf{88.79} &    \textbf{88.94}   &  \textbf{88.92} &     \textbf{88.99}    & \textbf{88.58}     &      \textbf{88.12} &  \textbf{88.63} &  \textbf{88.59} &\\  
        %\cline{2-9}
        $c_{1-4}$ &  \textbf{88.87} &  \textbf{88.75}  &  \textbf{88.99}  &  \textbf{89.11}  & \textbf{88.51}     &  \textbf{87.84} &  \textbf{88.46} &      \textbf{88.56}& \\ 
        \hline
        \hline
        75\bm{$\%D_t$}  & {87.33} & {87.41} & \textbf{87.44}  & {87.12}  & \textbf{87.92}   &   {87.21}    & 
        \textbf{88.14} &
        \textbf{88.28} & 86.40                        \\ 
        %\cline{2-9}
        50\bm{$\%D_t$}  & \textbf{87.06} & \textbf{87.04}  & \textbf{87.01}  & \textbf{86.77}  & \textbf{87.34}   &   \textbf{87.52}   & \textbf{86.96} & \textbf{86.77} & 85.40                        \\ 
        %\cline{2-9}
        30\bm{$\%D_t$}  & \textbf{85.22} & \textbf{85.06}  & \textbf{84.62} & \textbf{84.93}  & \textbf{86.70}    &   \textbf{85.02}    &
        84.80 & 84.60 & 83.40                        \\ 
        %\cline{2-9}
        10\bm{$\%D_t$}  & {76.47} & {75.99}  & {76.54} & {76.11}  &     75.67     &  75.67 & 75.67 & 75.67  & 75.57  \\
        \hline
    \end{tabular}
}
    \label{tab:TL_S_Ges}
\end{table}

==> Tables/gestures_cnnimu.tex <==
\begin{table}
%\centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Ges}$ and the \textit{tCNN-IMU}$_{D_s}^{Ges}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[10, 30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN_{Ges}$, trained on the training set of the Opportunity-Gestures, denotes the baseline. The values in bold have the corresponding testing accuracy significantly higher than the baseline one, based on a permutation test.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|p{10mm}|c c|c c|c c|c c|c|}
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN_{D_s}^{Ges}$}} \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn}  & 
        \multicolumn{2}{c|}{D$_s$=NTU}  & 
        \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\ 
        [0.1em]
        \hline
        $c_{1}$     & \textbf{88.66} & \textbf{89.05} &\textbf{88.82}  & \textbf{88.72}  &      \textbf{88.77}   &  \textbf{88.96}   & 89.19 &       89.03 & \multirow{4}{*}{87.36}     \\  
        \cline{2-7}
        $c_{1,2}$  & \textbf{88.83} & \textbf{88.97}  & \textbf{88.75}  & \textbf{88.80} & \textbf{88.67} & \textbf{88.53} & 88.93 & 88.81& \\  
        \cline{2-9}
        $c_{1-3}$  & 88.79 &   88.94   & 88.92 &    88.99    & \textbf{88.58}     &     88.12 & 88.63 & 88.59 &\\  
        \cline{2-9}
        $c_{1-4}$ & 88.87 & 88.75  & 88.99  & 89.11  & \textbf{88.51}     & 87.84 & 88.46 &     88.56& \\ 
        \hline
        \hline
        75\bm{$\%D_t$}  & \textbf{87.33} & \textbf{87.41} & \textbf{87.44}  & \textbf{87.12}  & \textbf{87.92}   &   \textbf{87.21}    & 
        88.14 &
        88.28 & 86.40                        \\ 
        \cline{2-9}
        50\bm{$\%D_t$}  & \textbf{87.06} & \textbf{87.04}  & \textbf{87.01}  & \textbf{86.77}  & 87.34   &   \textbf{87.52}   & 86.96 & 86.77 & 85.40                        \\ 
        \cline{2-9}
        30\bm{$\%D_t$}  & \textbf{85.22} & \textbf{85.06}  & \textbf{84.62} & \textbf{84.93}  & \textbf{86.70}    &   \textbf{85.02}    &
        84.80 & 84.60 & 83.40                        \\ 
        \cline{2-9}
        10\bm{$\%D_t$}  & \textbf{76.47} & \textbf{75.99}  & \textbf{76.54} & \textbf{76.11}  &     75.67     &  75.67 &75.67 & 75.67  & 75.57  \\
        \hline
        %
        \multicolumn{10}{c}{\vspace{2mm}}\\
        %
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN-IMU_{D_s}^{Ges}$}}  \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} &\textbf{Baseline} \\ 
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        \hline
        $c_{1}$     & {88.97} & 88.80 & {88.69}  & {88.57}  & 88.77 & 88.96 &    {88.93}    &  {88.98}    &  \multirow{4}{*}{88.50}     \\ 
        \cline{2-7}
        $c_{1,2}$  & {88.86} & {89.10}  & {88.50}  & {87.35}& 88.62 & 88.81 & 88.85 & {88.69}   &  \\  
        \cline{2-7}
        $c_{1-3}$  & 89.04 &   87.81   & 88.13 &    87.56    & 88.59 & 88.01 & 88.74 &    88.29   & \\  
        \cline{2-7}
        $c_{1-4}$ & 89 & 87.42  & 88.06  & 87.49 & 88.51 & 87.91 & 88.69 & 88.05   &  \\ 
        \hline
        \hline
        75\bm{$\%D_t$}  & {87.23} & {86.83} & {87.58}  & {86.22} & 88.42 & 87.10 & {87.23}   &   {87.45}       &  87.61  \\ 
        \cline{2-10}
        50\bm{$\%D_t$}  & {86.23} & {86.49}  & {86.49}  & {85.57} & \textbf{87.24} & 86.09  & 86.78   &   86.63   &  86.02 \\ 
        \cline{2-10}
        30\bm{$\%D_t$}  & {84.39} & {82.67}  & {84.37} & {83.05}  & \textbf{86.70} &  \textbf{85.02} & {84.29}    &   {83.74}    &  83.48  \\ 
        \cline{2-10}
        10\bm{$\%D_t$}  & {76.62} & {75.92}  & {76.47} & {76.15}  & 75.67 & 75.67 &            75.67  &   75.98     &  75.47 \\
        \hline
    \end{tabular}
}
    \label{tab:TL_S_Ges}
\end{table}

==> Tables/locomotion_cnnimu.tex <==
\begin{table}
    %\centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Loc}$ and \textit{tCNN-IMU}$_{D_s}^{Loc}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN_{Loc}$, trained on the training set of the Opportunity-Locomotion, denotes the baseline. The values in bold have the corresponding testing accuracy significantly higher than the baseline one, based on a permutation test.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|p{10mm}|c c|c c|c c|c c|c|}
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN_{D_s}^{Loc}$}} \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        [0.1em]
        \hline
        $c_1$ & \textbf{86.70}   & \textbf{86.84} & \textbf{86.87} & 86.28  & \textbf{86.70}  & 86.10 & 86.34 & \textbf{86.51} & \multirow{4}{*}{85.38 }     \\ 
        \cline{2-9}
        $c_{1,2}$& \textbf{86.54} & \textbf{86.80} & 86.40 & 86.15  & \textbf{86.54} & 85.97 &   \textbf{86.62} & \textbf{86.77} &   \\ 
        \cline{2-9}
        $c_{1-3}$ & 86.40 & \textbf{86.74} & 86.21 & 86.08  & 86.20& 85.86 &  \textbf{87.01} & \textbf{86.96} &  \\ 
        \cline{2-9}
        $c_{1-4}$ & 86.26 & \textbf{86.72} & 86.02 & 85.96 & 86.01 & 85.49 &  \textbf{87.21} & \textbf{87.05} &   \\
        \hline
        \hline
        75\bm{$\%D_t$} & 85.90  & \textbf{87.33} & 86.01 & 85.67& 85.66 & 85.13 & 86.67& 86.26 & 85.87       \\ 
        \cline{2-9}
        50\bm{$\%D_t$} & {85.18}  & \textbf{85.60} & \textbf{85.62}   & \textbf{85.46}  & 85.10  & 84.13 & \textbf{85.62}   & 85.03  & 84.44     \\ 
        \cline{2-9}
        30\bm{$\%D_t$} & \textbf{84.23} & {84.05} & \textbf{84.32} & 83.74  & \textbf{84.20} & 83.83 &  83.78  & 81.46 & 83.11     \\ 
        \cline{2-9}
        10\bm{$\%D_t$} & \textbf{55.16} & \textbf{54.77} & \textbf{54.90} & 53.12  & \textbf{55.33} & \textbf{55.54} & 53.90 & 53.61  & 52.60      \\       
        \hline
        %
        \multicolumn{8}{c}{\vspace{1mm}}\\
        %
        %\resizebox{\columnwidth}{!}{
        %\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN-IMU_{D_s}^{Loc}$}}  \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\  
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        \hline
        $c_1$ & 85.48   & 85.34 & \textbf{87.00} & \textbf{87.09}  & 84.88  & \textbf{85.33} & 84.88 & 85.33  & \multirow{4}{*}{84.98 }     \\ 
        \cline{2-9}
        $c_{1,2}$& 84.95 & 85.16 & 86.37 & \textbf{86.57}  & 84.67 & 84.92 & 84.59 & 84.87& \\ 
        \cline{2-9}
        $c_{1,2,3}$ & 84.61  & 84.44 & 85.06 & 85.85  & 84.25& 84.15 &  84.34 & 84.29 & \\ 
        \cline{2-9}
        $c_{1,2,3,4}$ & 84.39 & 83.80 & 84.44 & 86.14 & 84.12& 83.89 &  84.12 & 83.89  &  \\ 
        \hline
        \hline
        75\bm{$\%D_t$} & 84.64  & 83.59 & \textbf{85.83} & \textbf{85.89} & 84.14  & 84.34 & 84.14 & 84.34  & 83.83       \\ 
        \cline{2-9}
        50\bm{$\%D_t$}& \textbf{83.83}  & \textbf{83.15} & \textbf{83.86}   & \textbf{85.73}  & \textbf{83.51} & \textbf{83.66} & \textbf{83.15} & \textbf{83.25}  & 81.93      \\ 
        \cline{2-9}
        30\bm{$\%D_t$}& \textbf{81.87} & \textbf{82.71} & \textbf{82.02} & \textbf{83.09}  & \textbf{81.52} &  \textbf{81.81} & \textbf{81.52} & \textbf{81.80}  & 79.48      \\ 
        \cline{2-9}
        10\bm{$\%D_t$} & 44.09& {47.74} & 48.98 & 48.43  & 44.00 & 46.14 & 44.00 & 46.14  & 52.27   \\       
        \hline
    \end{tabular}
}
    \label{tab:TL_S_Loc}
\end{table}

==> Tables/pamap2_cnnimu.tex <==
\begin{center}
\begin{table}
%\centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multicolumn{2}{|l|}{}                                  & \multicolumn{2}{l|}{\bm{$tCI_{JHMDB}^{Pamap2}$}} & \multicolumn{2}{l|}{\bm{$tCI_{CAD60}^{Pamap2}$}} & \multicolumn{2}{l|}{\bm{$tCI_{NTU}^{Pamap2}$}}               & \textbf{$tCI^{Pamap2}$} \\  \cline{3-9} 
        \multicolumn{2}{|l|}{} &  \textbf{\%wF1 synth}  & \textbf{\%wF1 Pose}  & \textbf{\%wF1 synth}  & \textbf{\%wF1 Pose}  & \textbf{\%wF1 synth}                & \textbf{\%wF1 Pose} & \textbf{\%wF1}  \\ \hline
       \multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Transf. layers}}}}           &$c_1$                                          & 87.72$\pm$0.214   & 87.34$\pm$0.003 & 87.68$\pm$0.004          & 88.56$\pm$0.02         & $\pm$                          & $\pm$         & \multirow{4}{*}{86.31$\pm$ 0.006}      \\  
       \cline{2-8}
                    &$c_{1,2}$                                       & 87.52$\pm$0.007   & 86.54$\pm$0.004 & 86.73$\pm$0.009        & 88.12$\pm$0.022       & $\pm$& $\pm$      &       \\  
        \cline{2-8}
                    &$c_{1,2,3}$                                    & 85.35$\pm$0.007          & 86.38$\pm$0.004       & 85.84$\pm$0.007      & 87.67$\pm$0.009      & $\pm$                     & \textbf{$\pm$} &     \\  
        \cline{2-8}
                  &$c_{1,2,3,4}$                                  & 80.22$\pm$0.06   & 86.34$\pm$0.003  & 85.93$\pm$0.003          & 86.81$\pm$0.004     & $\pm$     & $\pm$       &      \\ 
        \hline
        \hline
        \multirow{3}{*} {\bm{$\%D_t$}}            & 75                             & 86.25$\pm$0.004   & 86.23$\pm$0.005   & 86.14$\pm$0.003   & 85.84$\pm$0.006    & $\pm$                      & \textbf{$\pm$}         & 79.86$\pm$0.004  \\  
        \cline{2-9}
                    & 50                              & 85.38$\pm$0.01   & 85.65$\pm$0.005 & 83.63$\pm$0.024  & 83.49$\pm$0.004  & $\pm$    & $\pm$    & 79.37$\pm$0.004  \\  
        \cline{2-9}
                    & 25                              & 67.71$\pm$0.06 & 70.01$\pm$0.02  & 64.43$\pm$0.03 & 60.29$\pm$0.05  & $\pm$ & $\pm$ & 60.35$\pm$0.04 \\ 
        
        \cline{2-9}
                    & 10                              & 40.20$\pm$0.016   & 40.20$\pm$0.025  & \textbf{$\pm$ }  & \textbf{$\pm$}        &                &           & 40.20$\pm$0.034       \\        
        \hline
    \end{tabular}
    }
    \caption{\scriptsize{The mean and std of $wF1[\%]$ of the $tCNN-IMU_{D_s}^{Pamap2}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN-IMU^{Pamap2}$, trained on the training set of the Pamap2, denotes the baseline. The values in bold have the corresponding testing accuracy significantly higher than the baseline one, based on a permutation test.}}
    \label{tab:TL_S_Pamap2}
\end{table}
\end{center}

==> Tables/step_size.tex <==
\begin{table}[h]
    \caption{\scriptsize{The $wF1[\%]$ for HAR on the three $D_s$: JHMDB$_{synth}$, CAD60$_{synth}$ and Penn$_{synth}$. The predictions on test set were unsegmented before computing the $wF1[\%]$. Multiple experiments were performed by fixing $W=1$ and varying the $s$.}}
    \resizebox{\columnwidth}{!}{
        \centering
        \begin{tabular}{cc|cccccc}
            \hline
            \multicolumn{2}{l}{\textbf{}}    & \multicolumn{6}{c}{\textbf{Step Size (s)}}  \\ 
            \textbf{Dataset} & \textbf{Hz} & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{5}     & \multicolumn{1}{l}{10}    & \multicolumn{1}{l}{12}    & \multicolumn{1}{l}{20}    & 25    \\ 
            \hline
            \hline
            \textbf{JHMDB}   & 100         & \multicolumn{1}{l}{36.66$\pm$0.56} & \multicolumn{1}{l}{46.76$\pm$0.72} & \multicolumn{1}{l}{70.13$\pm$0.39} & \multicolumn{1}{l}{85.68$\pm$0.81} & \multicolumn{1}{l}{66.81$\pm$0.12} & 60.16$\pm$0.42 \\ 
            \textbf{CAD60}   & 100         & \multicolumn{1}{l}{47.66$\pm$0.42} & \multicolumn{1}{l}{49.30$\pm$0.26} & \multicolumn{1}{l}{56.28$\pm$0.12} & \multicolumn{1}{l}{57.16$\pm$0.06} & \multicolumn{1}{l}{51.12$\pm$0.09} & 47.02$\pm$0.42 \\ 
            \textbf{Penn}    & 100         & \multicolumn{1}{l}{96.00$\pm$0.08} & \multicolumn{1}{l}{87.60$\pm$0.72}  & \multicolumn{1}{l}{84.13$\pm$0.18} & \multicolumn{1}{l}{81.81$\pm$0.22} & \multicolumn{1}{l}{77.84$\pm$0.31} & 74.48$\pm$0.09 \\ 
            \hline
        \end{tabular}
    }
    \label{tab:step_size}
\end{table}

==> Tables/window_size.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
    \caption{\scriptsize{The $wF1[\%]$ for HAR on the three $D_s$: JHMDB$_{synth}$, CAD60$_{synth}$ and Penn$_{synth}$. The predictions on test set were unsegmented before computing the $wF1[\%]$. Multiple experiments were performed by fixing the $s$ and varying the $W$.}}
    \resizebox{\columnwidth}{!}{
        \centering
        \begin{tabular}{ll|llllll}
            \hline
            \multicolumn{2}{l}{\textbf{}}    & \multicolumn{6}{c}{\textbf{Window Size (W)}}      \\ 
            \textbf{Dataset}                & \textbf{Hz} & \multicolumn{1}{l}{1} & \multicolumn{1}{l}{2}     & \multicolumn{1}{l}{3}     & \multicolumn{1}{l}{4}     & \multicolumn{1}{l}{5}     & 6     \\ 
            \hline
            \hline
            \multirow{2}{*}{\textbf{JHMDB}} & 25             & \multicolumn{1}{l}{26.58$\pm$0.06}  & \multicolumn{1}{l}{25.47$\pm$0.08} & \multicolumn{1}{l}{25.01$\pm$0.11} & \multicolumn{1}{l}{23.57$\pm$0.09} & \multicolumn{1}{l}{23.50$\pm$0.18} &       \\  
            & 100             & \multicolumn{1}{l}{85.68$\pm$0.81}  & \multicolumn{1}{l}{83.43$\pm$0.82} & \multicolumn{1}{l}{66.88$\pm$0.48} & \multicolumn{1}{l}{54.69$\pm$0.38} & \multicolumn{1}{l}{49.27$\pm$0.51} &       \\ 
            \hline
            \multirow{2}{*}{\textbf{CAD60}} & 30             & \multicolumn{1}{l}{50.11$\pm$0.06}  & \multicolumn{1}{l}{88.34$\pm$0.11} & \multicolumn{1}{l}{91.11$\pm$0.09} & \multicolumn{1}{l}{91.94$\pm$0.10} & \multicolumn{1}{l}{94.10$\pm$0.09} & 93.58$\pm$0.19 \\
            & 100             & \multicolumn{1}{l}{57.16$\pm$0.06}  & \multicolumn{1}{l}{56.52$\pm$0.09} & \multicolumn{1}{l}{78.03$\pm$0.15} & \multicolumn{1}{l}{86.63$\pm$0.21} & \multicolumn{1}{l}{92.01$\pm$0.18} & 90.51$\pm$0.09 \\ 
            \hline
            \textbf{Penn}                   & 100            & \multicolumn{1}{l}{96.00$\pm$0.08}  & \multicolumn{1}{l}{95.10$\pm$0.28} & \multicolumn{1}{l}{94.30$\pm$0.37} & \multicolumn{1}{l}{93.10$\pm$0.18} & \multicolumn{1}{l}{92.46$\pm$0.73} &       \\ 
            \hline
        \end{tabular}
    }
    \label{tab:window_size}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Images/preambel.tex <==
% Add Packages
% -------------------------------------------------------------------
% URLs
\usepackage{url}

% -------------------------------------------------------------------
% Misc Utility
\usepackage[cmex10]{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{eqparbox}

% -------------------------------------------------------------------
% Grafikpakete einbinden
\usepackage{amssymb}
\usepackage{flafter}
\usepackage{listings}

% -------------------------------------------------------------------
% Korrekte Darstellung der Umlaute
\usepackage[T1]{fontenc}
\usepackage{ae,aecompl}
\usepackage[utf8]{inputenc}
\usepackage[english,german,ngerman]{babel}

% -------------------------------------------------------------------
% Anführungszeichen
\usepackage[babel,german=quotes]{csquotes}

% -------------------------------------------------------------------
% Classic thesis:
\usepackage{classicthesis-ldpkg} 
% Options for classicthesis.sty:
\usepackage[eulerchapternumbers,subfig,beramono,eulermath,parts]{classicthesis}

% -------------------------------------------------------------------
% Setup and Finetuning
\newlength{\abcd} % for ab..z string length calculation
\newcommand{\myfloatalign}{\centering} % how all the floats will be aligned
\setlength{\extrarowheight}{3pt} % increase table row height

% -------------------------------------------------------------------
%Equation and figure numbering
\numberwithin{equation}{section} 
%sets equation numbers <chapter>.<section>.<index>
\numberwithin{table}{section} 
%sets equation numbers <chapter>.<section>.<index>
\numberwithin{figure}{section} 
%sets figure numbers <chapter>.<section>.<index>

% Captions look and feel
% -------------------------------------------------------------------
\captionsetup{format=hang,font=small}

\usepackage{tikz} % must be imported after classicthesis-ldpkg


==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/gestures_cnn.tex <==
\begin{table}
%\centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Ges}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[10, 30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN_{Ges}$, trained on the training set of the Opportunity-Gestures, denotes the baseline. Std $wF1[\%]$ lies around $0.01$. The performance of the $tCNN-IMU_{D_s}^{MM}$ is similar, thus, not shown.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c c|c}
        \hline
        \multicolumn{10}{c}{\bm{$tCNN_{D_s}^{Ges}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn}  & 
        \multicolumn{2}{c|}{D$_s$=NTU}  & 
        \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\ 
        [0.1em]
        \hline
        \hline
        $c_{1}$     & \textbf{88.66} & \textbf{89.05} &\textbf{88.82}  & \textbf{88.72}  &      \textbf{88.77}   &  \textbf{88.96}   &  \textbf{89.19} &       \textbf{89.03} & \multirow{4}{*}{87.36}     \\  
        %\cline{2-9}
        $c_{1,2}$  & \textbf{88.83} & \textbf{88.97}  & \textbf{88.75}  & \textbf{88.80} & \textbf{88.67} & \textbf{88.53} &  \textbf{88.93} &  \textbf{88.81}& \\  
        %\cline{2-9}
        $c_{1-3}$  &  \textbf{88.79} &    \textbf{88.94}   &  \textbf{88.92} &     \textbf{88.99}    & \textbf{88.58}     &      \textbf{88.12} &  \textbf{88.63} &  \textbf{88.59} &\\  
        %\cline{2-9}
        $c_{1-4}$ &  \textbf{88.87} &  \textbf{88.75}  &  \textbf{88.99}  &  \textbf{89.11}  & \textbf{88.51}     &  \textbf{87.84} &  \textbf{88.46} &      \textbf{88.56}& \\ 
        \hline
        \hline
        75\bm{$\%D_t$}  & {87.33} & {87.41} & \textbf{87.44}  & {87.12}  & \textbf{87.92}   &   {87.21}    & 
        \textbf{88.14} &
        \textbf{88.28} & 86.40                        \\ 
        %\cline{2-9}
        50\bm{$\%D_t$}  & \textbf{87.06} & \textbf{87.04}  & \textbf{87.01}  & \textbf{86.77}  & \textbf{87.34}   &   \textbf{87.52}   & \textbf{86.96} & \textbf{86.77} & 85.40                        \\ 
        %\cline{2-9}
        30\bm{$\%D_t$}  & \textbf{85.22} & \textbf{85.06}  & \textbf{84.62} & \textbf{84.93}  & \textbf{86.70}    &   \textbf{85.02}    &
        84.80 & 84.60 & 83.40                        \\ 
        %\cline{2-9}
        10\bm{$\%D_t$}  & {76.47} & {75.99}  & {76.54} & {76.11}  &     75.67     &  75.67 & 75.67 & 75.67  & 75.57  \\
        \hline
    \end{tabular}
}
    \label{tab:TL_S_Ges}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/gestures_cnnimu.tex <==
\begin{table}
%\centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Ges}$ and the \textit{tCNN-IMU}$_{D_s}^{Ges}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[10, 30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN_{Ges}$, trained on the training set of the Opportunity-Gestures, denotes the baseline. The values in bold have the corresponding testing accuracy significantly higher than the baseline one, based on a permutation test.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|p{10mm}|c c|c c|c c|c c|c|}
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN_{D_s}^{Ges}$}} \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn}  & 
        \multicolumn{2}{c|}{D$_s$=NTU}  & 
        \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\ 
        [0.1em]
        \hline
        $c_{1}$     & \textbf{88.66} & \textbf{89.05} &\textbf{88.82}  & \textbf{88.72}  &      \textbf{88.77}   &  \textbf{88.96}   & 89.19 &       89.03 & \multirow{4}{*}{87.36}     \\  
        \cline{2-7}
        $c_{1,2}$  & \textbf{88.83} & \textbf{88.97}  & \textbf{88.75}  & \textbf{88.80} & \textbf{88.67} & \textbf{88.53} & 88.93 & 88.81& \\  
        \cline{2-9}
        $c_{1-3}$  & 88.79 &   88.94   & 88.92 &    88.99    & \textbf{88.58}     &     88.12 & 88.63 & 88.59 &\\  
        \cline{2-9}
        $c_{1-4}$ & 88.87 & 88.75  & 88.99  & 89.11  & \textbf{88.51}     & 87.84 & 88.46 &     88.56& \\ 
        \hline
        \hline
        75\bm{$\%D_t$}  & \textbf{87.33} & \textbf{87.41} & \textbf{87.44}  & \textbf{87.12}  & \textbf{87.92}   &   \textbf{87.21}    & 
        88.14 &
        88.28 & 86.40                        \\ 
        \cline{2-9}
        50\bm{$\%D_t$}  & \textbf{87.06} & \textbf{87.04}  & \textbf{87.01}  & \textbf{86.77}  & 87.34   &   \textbf{87.52}   & 86.96 & 86.77 & 85.40                        \\ 
        \cline{2-9}
        30\bm{$\%D_t$}  & \textbf{85.22} & \textbf{85.06}  & \textbf{84.62} & \textbf{84.93}  & \textbf{86.70}    &   \textbf{85.02}    &
        84.80 & 84.60 & 83.40                        \\ 
        \cline{2-9}
        10\bm{$\%D_t$}  & \textbf{76.47} & \textbf{75.99}  & \textbf{76.54} & \textbf{76.11}  &     75.67     &  75.67 &75.67 & 75.67  & 75.57  \\
        \hline
        %
        \multicolumn{10}{c}{\vspace{2mm}}\\
        %
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN-IMU_{D_s}^{Ges}$}}  \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} &\textbf{Baseline} \\ 
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        \hline
        $c_{1}$     & {88.97} & 88.80 & {88.69}  & {88.57}  & 88.77 & 88.96 &    {88.93}    &  {88.98}    &  \multirow{4}{*}{88.50}     \\ 
        \cline{2-7}
        $c_{1,2}$  & {88.86} & {89.10}  & {88.50}  & {87.35}& 88.62 & 88.81 & 88.85 & {88.69}   &  \\  
        \cline{2-7}
        $c_{1-3}$  & 89.04 &   87.81   & 88.13 &    87.56    & 88.59 & 88.01 & 88.74 &    88.29   & \\  
        \cline{2-7}
        $c_{1-4}$ & 89 & 87.42  & 88.06  & 87.49 & 88.51 & 87.91 & 88.69 & 88.05   &  \\ 
        \hline
        \hline
        75\bm{$\%D_t$}  & {87.23} & {86.83} & {87.58}  & {86.22} & 88.42 & 87.10 & {87.23}   &   {87.45}       &  87.61  \\ 
        \cline{2-10}
        50\bm{$\%D_t$}  & {86.23} & {86.49}  & {86.49}  & {85.57} & \textbf{87.24} & 86.09  & 86.78   &   86.63   &  86.02 \\ 
        \cline{2-10}
        30\bm{$\%D_t$}  & {84.39} & {82.67}  & {84.37} & {83.05}  & \textbf{86.70} &  \textbf{85.02} & {84.29}    &   {83.74}    &  83.48  \\ 
        \cline{2-10}
        10\bm{$\%D_t$}  & {76.62} & {75.92}  & {76.47} & {76.15}  & 75.67 & 75.67 &            75.67  &   75.98     &  75.47 \\
        \hline
    \end{tabular}
}
    \label{tab:TL_S_Ges}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/locomotion_cnn.tex <==
\begin{table}
    %\centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Loc}$ and \textit{tCNN}$_{D_s}^{Ges}$ using the joint poses and the synthetic data. The $N_{conv}$ changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $N_{conv}$ corresponding to highest $wF1[\%]$ is fixed and $\%D_t$ is varied. The $tCNN_{Loc}$, trained on the training set of the Opp-Loc and -Ges, denotes the baseline. Std $wF1[\%]$ lies around $0.01$. The performance of the \textit{tCNN-IMU}$_{D_s}^{Loc}$ and \textit{tCNN-IMU}$_{D_s}^{Ges}$ is similar, thus, not shown.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c c|c}
        \hline
        \multicolumn{10}{c}{\bm{$tCNN_{D_s}^{Loc}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        [0.1em]
        \hline
        \hline
        $c_1$ & \textbf{86.70}   & \textbf{86.84} & \textbf{86.87} & 86.28  & \textbf{86.70}  & 86.10 & 86.34 & \textbf{86.51} & \multirow{4}{*}{85.65 }     \\ 
        %\cline{2-9}
        $c_{1,2}$& {86.54} & \textbf{86.80} & 86.40 & 86.15  & {86.54} & 85.97 &   \textbf{86.62} & \textbf{86.77} &   \\ 
        %\cline{2-9}
        $c_{1-3}$ & 86.40 & \textbf{86.74} & 86.21 & 86.08  & 86.20& 85.86 &  \textbf{87.01} & \textbf{86.96} &  \\ 
        %\cline{2-9}
        $c_{1-4}$ & 86.26 & \textbf{86.72} & 86.02 & 85.96 & 86.01 & 85.49 &  \textbf{87.21} & \textbf{87.05} &   \\
        \hline
        \hline
        75\bm{$\%D_t$} & 85.90  & \textbf{87.33} & 86.01 & 85.67& 85.66 & 85.13 &  \textbf{86.67} & 86.26 & 85.67       \\ 
        %\cline{2-9}
        50\bm{$\%D_t$} & {85.18}  & \textbf{85.60} & \textbf{85.62}   & \textbf{85.46}  & 85.10  & 84.13 & \textbf{85.62}   & 85.03  & 84.44     \\ 
        %\cline{2-9}
        30\bm{$\%D_t$} & \textbf{84.23} & {84.05} & \textbf{84.32} & 83.74  & \textbf{84.20} & 83.83 &  83.78  & 81.46 & 83.11     \\ 
        %\cline{2-9}
        10\bm{$\%D_t$} & \textbf{55.16} & \textbf{54.77} & \textbf{54.90} & 53.12  & \textbf{55.33} & \textbf{55.54} & 53.90 & 53.61  & 52.60      \\       
        \hline
        \multicolumn{6}{c}{\vspace{-1mm}}\\
    \end{tabular}
}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c c|c}
        \hline
        \multicolumn{10}{c}{\bm{$tCNN_{D_s}^{Ges}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn}  & 
        \multicolumn{2}{c|}{D$_s$=NTU}  & 
        \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\ 
        [0.1em]
        \hline
        \hline
        $c_{1}$     & \textbf{88.66} & \textbf{89.05} &\textbf{88.82}  & \textbf{88.72}  &      \textbf{88.77}   &  \textbf{88.96}   &  \textbf{89.19} &       \textbf{89.03} & \multirow{4}{*}{87.36}     \\  
        %\cline{2-9}
        $c_{1,2}$  & \textbf{88.83} & \textbf{88.97}  & \textbf{88.75}  & \textbf{88.80} & \textbf{88.67} & \textbf{88.53} &  \textbf{88.93} &  \textbf{88.81}& \\  
        %\cline{2-9}
        $c_{1-3}$  &  \textbf{88.79} &    \textbf{88.94}   &  \textbf{88.92} &     \textbf{88.99}    & \textbf{88.58}     &      \textbf{88.12} &  \textbf{88.63} &  \textbf{88.59} &\\  
        %\cline{2-9}
        $c_{1-4}$ &  \textbf{88.87} &  \textbf{88.75}  &  \textbf{88.99}  &  \textbf{89.11}  & \textbf{88.51}     &  \textbf{87.84} &  \textbf{88.46} &      \textbf{88.56}& \\ 
        \hline
        \hline
        75\bm{$\%D_t$}  & {87.33} & {87.41} & \textbf{87.44}  & {87.12}  & \textbf{87.92}   &   {87.21}    & 
        \textbf{88.14} &
        \textbf{88.28} & 86.40                        \\ 
        %\cline{2-9}
        50\bm{$\%D_t$}  & \textbf{87.06} & \textbf{87.04}  & \textbf{87.01}  & \textbf{86.77}  & \textbf{87.34}   &   \textbf{87.52}   & \textbf{86.96} & \textbf{86.77} & 85.40                        \\ 
        %\cline{2-9}
        30\bm{$\%D_t$}  & \textbf{85.22} & \textbf{85.06}  & \textbf{84.62} & \textbf{84.93}  & \textbf{86.70}    &   \textbf{85.02}    &
        84.80 & 84.60 & 83.40                        \\ 
        %\cline{2-9}
        10\bm{$\%D_t$}  & {76.47} & {75.99}  & {76.54} & {76.11}  &     75.67     &  75.67 & 75.67 & 75.67  & 75.57  \\
        \hline
        \multicolumn{6}{c}{\vspace{-7mm}}\\
    \end{tabular}
    }
    \label{tab:TL_S_Loc}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/locomotion_cnnimu.tex <==
\begin{table}
    %\centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Loc}$ and \textit{tCNN-IMU}$_{D_s}^{Loc}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN_{Loc}$, trained on the training set of the Opportunity-Locomotion, denotes the baseline. The values in bold have the corresponding testing accuracy significantly higher than the baseline one, based on a permutation test.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|p{10mm}|c c|c c|c c|c c|c|}
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN_{D_s}^{Loc}$}} \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        [0.1em]
        \hline
        $c_1$ & \textbf{86.70}   & \textbf{86.84} & \textbf{86.87} & 86.28  & \textbf{86.70}  & 86.10 & 86.34 & \textbf{86.51} & \multirow{4}{*}{85.38 }     \\ 
        \cline{2-9}
        $c_{1,2}$& \textbf{86.54} & \textbf{86.80} & 86.40 & 86.15  & \textbf{86.54} & 85.97 &   \textbf{86.62} & \textbf{86.77} &   \\ 
        \cline{2-9}
        $c_{1-3}$ & 86.40 & \textbf{86.74} & 86.21 & 86.08  & 86.20& 85.86 &  \textbf{87.01} & \textbf{86.96} &  \\ 
        \cline{2-9}
        $c_{1-4}$ & 86.26 & \textbf{86.72} & 86.02 & 85.96 & 86.01 & 85.49 &  \textbf{87.21} & \textbf{87.05} &   \\
        \hline
        \hline
        75\bm{$\%D_t$} & 85.90  & \textbf{87.33} & 86.01 & 85.67& 85.66 & 85.13 & 86.67& 86.26 & 85.87       \\ 
        \cline{2-9}
        50\bm{$\%D_t$} & {85.18}  & \textbf{85.60} & \textbf{85.62}   & \textbf{85.46}  & 85.10  & 84.13 & \textbf{85.62}   & 85.03  & 84.44     \\ 
        \cline{2-9}
        30\bm{$\%D_t$} & \textbf{84.23} & {84.05} & \textbf{84.32} & 83.74  & \textbf{84.20} & 83.83 &  83.78  & 81.46 & 83.11     \\ 
        \cline{2-9}
        10\bm{$\%D_t$} & \textbf{55.16} & \textbf{54.77} & \textbf{54.90} & 53.12  & \textbf{55.33} & \textbf{55.54} & 53.90 & 53.61  & 52.60      \\       
        \hline
        %
        \multicolumn{8}{c}{\vspace{1mm}}\\
        %
        %\resizebox{\columnwidth}{!}{
        %\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multicolumn{10}{|c|}{\bm{$tCNN-IMU_{D_s}^{Loc}$}}  \\
        [0.2em]
        \hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\  
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        \hline
        $c_1$ & 85.48   & 85.34 & \textbf{87.00} & \textbf{87.09}  & 84.88  & \textbf{85.33} & 84.88 & 85.33  & \multirow{4}{*}{84.98 }     \\ 
        \cline{2-9}
        $c_{1,2}$& 84.95 & 85.16 & 86.37 & \textbf{86.57}  & 84.67 & 84.92 & 84.59 & 84.87& \\ 
        \cline{2-9}
        $c_{1,2,3}$ & 84.61  & 84.44 & 85.06 & 85.85  & 84.25& 84.15 &  84.34 & 84.29 & \\ 
        \cline{2-9}
        $c_{1,2,3,4}$ & 84.39 & 83.80 & 84.44 & 86.14 & 84.12& 83.89 &  84.12 & 83.89  &  \\ 
        \hline
        \hline
        75\bm{$\%D_t$} & 84.64  & 83.59 & \textbf{85.83} & \textbf{85.89} & 84.14  & 84.34 & 84.14 & 84.34  & 83.83       \\ 
        \cline{2-9}
        50\bm{$\%D_t$}& \textbf{83.83}  & \textbf{83.15} & \textbf{83.86}   & \textbf{85.73}  & \textbf{83.51} & \textbf{83.66} & \textbf{83.15} & \textbf{83.25}  & 81.93      \\ 
        \cline{2-9}
        30\bm{$\%D_t$}& \textbf{81.87} & \textbf{82.71} & \textbf{82.02} & \textbf{83.09}  & \textbf{81.52} &  \textbf{81.81} & \textbf{81.52} & \textbf{81.80}  & 79.48      \\ 
        \cline{2-9}
        10\bm{$\%D_t$} & 44.09& {47.74} & 48.98 & 48.43  & 44.00 & 46.14 & 44.00 & 46.14  & 52.27   \\       
        \hline
    \end{tabular}
}
    \label{tab:TL_S_Loc}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/pamap2_activities.tex <==
\begin{table}
    \centering
    \caption{\scriptsize{Precision$[\%]$ and recall$[\%]$ values per activity of the JHMDB and Pamap2 datasets. The \textit{tCNN}$^{Pamap2}$ is considered as the baseline. The values in bold are selected based on the higher harmonic mean of precision and recall.}}
    \resizebox{\columnwidth}{!}{
    %\scalebox{0.7}{%
    \begin{tabular}{c cccccc}
        \hline
        \multirow{2}{*}{Pamap2 Act.} &
        \multicolumn{2}{c}{tCNN$_{JHMDB_{synth.}}$} &
        \multicolumn{2}{c}{tCNN$^{Pamap2}$} &
        \multicolumn{2}{c}{tCNN$_{JHMDB_{synth.}^{c1}}^{Pamap2}$} \\
        %\cline{2-7}
        & \text{Prec.}\% & \text{Rec.}\% & \text{Prec.}\% & \text{Rec.}\% & \text{Prec.}\% & \text{Rec.}\%  \\
        \hline
        \hline
        %\text{Brush Hair}&95.38 &100  & - & -& - & \\
        %\text{Catch}&94.44 &91.89  & - & - & - &\\
        %\text{Clap}&93.65 & 95.16  & - & -& - & \\
        \text{Climb stairs}&97.87 &86.79 & 73.28 & 95.01 &\bf{90.34} & \bf{95.90} \\
        %\text{Golf swing}&95.59 &100  & - & -& - & \\
        %\text{Jump}&100 &91.49 & - & -& - & \\
        %\text{Kick ball}&91.67 &89.80 & - & -& - & \\
        %\text{Pick}&87.04 &92.16 & - & - & - &\\
        %\text{Pour}&92.31 &88.89 & - & - & - &\\
        %\text{Pull-up}&92.65 &100  & - & -& - & \\
        %\text{Push}&100 &60.34 & - & -& - & \\
        \text{Run}&65.08 &85.42 & 100 & 92.26 & \bf{100} & \bf{92.91} \\
        %\text{Shoot Ball}&82.93 &100 &- & -& - & \\
        %\text{Shoot Bow}&88.73 &85.94 & - & -& - & \\
        %\text{Shoot Gun}&76.47 &84.78  & -&- & - &\\
        \text{Sit}&100 &89.13 & 94.27 & 94.32 & \bf{95.38} & \bf{94.07} \\
        \text{Stand}&94.23&100& 87.53 & 28.65 & \bf{86.46} &\bf{40.71} \\
        %\text{Baseball Swing}&92.54 &98.41  &- & - & - &\\
        %\text{Throw}&90.20 &90.20 &- & - & - &\\
        \text{Walk}&96.00 &88.89 & 92.65 & 97.86 & \bf{98.06} &\bf{99.47} \\
        %\text{Wave}&97.67 &95.45  & - & - & - & \\
        \text{Rope Jump}&-&-&\bf{83.33} &\bf{100} & 77.10 & 100 \\
        \text{Lying}&-&-&98.79  &97.21  & {100} & {96.76} \\
        \text{Cycling}&-&-&100 & 96.23 & {100} & {96.55} \\
        \text{Nordic Walk}&-&-& \bf{100} & \bf{94.53} & 90.34 & 95.90 \\
        \text{Desc. Stairs}&-&-&80.47  &84.74  & \bf{86.51} & \bf{87.80} \\
        \text{Vacuuming}&-&-&98.26 & 74.14  & \bf{96.01} & \bf{91.73} \\
        \text{Ironing}&-&-&67.62  &100 & \bf{72.04} & \bf{99.12}\\
        \hline
        \multicolumn{6}{c}{\vspace{-6mm}}\\
    \end{tabular}}
    \label{tab:TL_PR}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/pamap2_cnn.tex <==
\begin{table}
    \centering
    \caption{\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{Pamap2}$ and \textit{tCNN-IMU}$_{D_s}^{Pamap2}$ using the joint poses and the synthetic data. The $N_{conv}$ changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $N_{conv}$ corresponding to highest $wF1[\%]$ is fixed and $[10, 30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The \textit{tCNN}$^{Pamap2}$ and the \textit{tCNN-IMU}$^{Pamap2}$, trained on the training set of the Pamap2, denote the baseline. Std $wF1[\%]$ lies around $0.01$.}}
    \label{tab:TL_S_Pamap2}
    %\subcaption*{\bm{$tCNN_{D_s}^{Pamap2}$}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c c|c}
        \hline
        \multicolumn{10}{c}{\bm{$tCNN_{D_s}^{Pamap2}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c}{D$_s$=JHMDB} & \multicolumn{2}{c}{D$_s$=CAD60} & \multicolumn{2}{c}{D$_s$=Penn} & \multicolumn{2}{c}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\ 
        [0.1em]
        \hline
        \hline
        $c_1$ & \textbf{89.70}   & \textbf{88.37} & \textbf{88.70}  & \textbf{89.73}  & \textbf{89.89}  & \textbf{88.30} & \textbf{90.78} & \textbf{89.20}  &  \multirow{4}{*}{86.67}      \\
        [0.1em]
        %\cline{2-9}
        $c_{1,2}$         & 87.72   & \textbf{88.15} & 87.85  & \textbf{88.24} & \textbf{90.10} & {87.91}  & \textbf{90.36} & \textbf{89.66} &       \\  
        [0.1em]
        %\cline{2-9}
        $c_{1-3}$      & 86.51 & \textbf{88.12}  & 87.23  & 87.48 & \textbf{90.46}  & 87.56 & \textbf{89.16} & \textbf{90.73} & \\  
        [0.1em]
        %\cline{2-9}
        $c_{1-4}$    & {84.96}   & \textbf{88.13}  & 87.77  & 87.89  & \textbf{90.64}  & 87.10 &   \textbf{88.94} & \textbf{91.23} &   \\ 
        [0.1em]
        \hline
        \hline
        75\bm{$\%D_t$}   & \textbf{89.64} & \textbf{89.60}         & {88.16}  & {88.17}    & {86.46 } & 86.81  & \textbf{88.73} & {88.02} & 88.17       \\  
        [0.1em]
        %\cline{2-9}
        50\bm{$\%D_t$}    & \textbf{89.63}    & {86.93} & {85.76}  & \textbf{89.03} & {83.91 } & {83.30}   & 85.95 & 85.15 &  85.96      \\  
        [0.1em]
        %\cline{2-9}
        30\bm{$\%D_t$}    & \textbf{58.70}   & \textbf{49.00}   & \textbf{51.98}  & \textbf{50.27}        &    \textbf{74.14} & \textbf{73.04} & \textbf{81.98} & \textbf{70.71} & 44.47      \\
        [0.1em]
        %\cline{2-9}
        10\bm{$\%D_t$}    & \textbf{50.97}   & \textbf{46.75}   & \textbf{47.26}  & \textbf{45.93}        &    \textbf{50.20} & \textbf{49.20}  & \textbf{43.93} & \textbf{51.36} & 40.96       \\
        [0.1em]
        \hline
        \multicolumn{8}{c}{\vspace{-1mm}}\\
    \end{tabular}
    }
    %\bigskip
    %\subcaption*{\bm{$tCNN-IMU_{D_s}^{Pamap2}$}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c}
        \hline
        \multicolumn{8}{c}{\bm{$tCNN-IMU_{D_s}^{Pamap2}$}}  \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c}{D$_s$=JHMDB} & \multicolumn{2}{c}{D$_s$=CAD60} & \multicolumn{2}{c}{D$_s$=NTU RGB+D} &\textbf{Baseline} \\ 
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  &\textbf{Pose} & \textbf{\%wF1}  \\ 
        \hline
        \hline
        $c_1$ & 87.72   & 87.34 & 87.68   & \textbf{88.56}    & 87.24 & 86.23  & \multirow{4}{*}{86.91}      \\  
        %\cline{2-7}
        $c_{1,2}$         & 87.52   & 86.54 & 86.73        & \textbf{88.12}   &   87.75 & 86.42  &   \\  
        %\cline{2-7}
        $c_{1-3}$      & 85.35 & 86.38       & 85.84      & 87.67     &   \textbf{88.09} & 86.93  &  \\  
        %\cline{2-7}
        $c_{1-4}$    & 80.22   & 86.34  & 85.93 & 86.81     & \textbf{88.52} & 87.01 &   \\ 
        \hline
        \hline
        75\bm{$\%D_t$}   & 86.25   & 86.23 & 86.14  & 85.84   & 88.41 & 86.52  & 88.06  \\  
        %\cline{2-7}
        50\bm{$\%D_t$}    & \textbf{85.38}  & \textbf{85.65} & 83.63  & 83.49  & \textbf{85.93} & \textbf{84.91}  & 83.04  \\  
        %\cline{2-7}
        30\bm{$\%D_t$}    & \textbf{67.71} & \textbf{70.01}  & \textbf{64.43} & 60.29 & \textbf{66.96} &  \textbf{73.68}  & 60.35 \\ 
        %\cline{2-7}
        10\bm{$\%D_t$}    & 40.20   & 40.20  & 40.20 & 40.20 & \textbf{51.30}   & \textbf{59.59}  & 40.20       \\ 
        \hline
        \multicolumn{6}{c}{\vspace{-7mm}}\\
    \end{tabular}
    }
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/pamap2_cnnimu.tex <==
\begin{center}
\begin{table}
%\centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multicolumn{2}{|l|}{}                                  & \multicolumn{2}{l|}{\bm{$tCI_{JHMDB}^{Pamap2}$}} & \multicolumn{2}{l|}{\bm{$tCI_{CAD60}^{Pamap2}$}} & \multicolumn{2}{l|}{\bm{$tCI_{NTU}^{Pamap2}$}}               & \textbf{$tCI^{Pamap2}$} \\  \cline{3-9} 
        \multicolumn{2}{|l|}{} &  \textbf{\%wF1 synth}  & \textbf{\%wF1 Pose}  & \textbf{\%wF1 synth}  & \textbf{\%wF1 Pose}  & \textbf{\%wF1 synth}                & \textbf{\%wF1 Pose} & \textbf{\%wF1}  \\ \hline
       \multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Transf. layers}}}}           &$c_1$                                          & 87.72$\pm$0.214   & 87.34$\pm$0.003 & 87.68$\pm$0.004          & 88.56$\pm$0.02         & $\pm$                          & $\pm$         & \multirow{4}{*}{86.31$\pm$ 0.006}      \\  
       \cline{2-8}
                    &$c_{1,2}$                                       & 87.52$\pm$0.007   & 86.54$\pm$0.004 & 86.73$\pm$0.009        & 88.12$\pm$0.022       & $\pm$& $\pm$      &       \\  
        \cline{2-8}
                    &$c_{1,2,3}$                                    & 85.35$\pm$0.007          & 86.38$\pm$0.004       & 85.84$\pm$0.007      & 87.67$\pm$0.009      & $\pm$                     & \textbf{$\pm$} &     \\  
        \cline{2-8}
                  &$c_{1,2,3,4}$                                  & 80.22$\pm$0.06   & 86.34$\pm$0.003  & 85.93$\pm$0.003          & 86.81$\pm$0.004     & $\pm$     & $\pm$       &      \\ 
        \hline
        \hline
        \multirow{3}{*} {\bm{$\%D_t$}}            & 75                             & 86.25$\pm$0.004   & 86.23$\pm$0.005   & 86.14$\pm$0.003   & 85.84$\pm$0.006    & $\pm$                      & \textbf{$\pm$}         & 79.86$\pm$0.004  \\  
        \cline{2-9}
                    & 50                              & 85.38$\pm$0.01   & 85.65$\pm$0.005 & 83.63$\pm$0.024  & 83.49$\pm$0.004  & $\pm$    & $\pm$    & 79.37$\pm$0.004  \\  
        \cline{2-9}
                    & 25                              & 67.71$\pm$0.06 & 70.01$\pm$0.02  & 64.43$\pm$0.03 & 60.29$\pm$0.05  & $\pm$ & $\pm$ & 60.35$\pm$0.04 \\ 
        
        \cline{2-9}
                    & 10                              & 40.20$\pm$0.016   & 40.20$\pm$0.025  & \textbf{$\pm$ }  & \textbf{$\pm$}        &                &           & 40.20$\pm$0.034       \\        
        \hline
    \end{tabular}
    }
    \caption{\scriptsize{The mean and std of $wF1[\%]$ of the $tCNN-IMU_{D_s}^{Pamap2}$ using the joint poses and the synthetic data. The number of transferred convolution layers changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $c_1$ is fixed and $[30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The $tCNN-IMU^{Pamap2}$, trained on the training set of the Pamap2, denotes the baseline. The values in bold have the corresponding testing accuracy significantly higher than the baseline one, based on a permutation test.}}
    \label{tab:TL_S_Pamap2}
\end{table}
\end{center}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/pose_datasets.tex <==
\begin{table}[t]
    \caption{\scriptsize{The $wF1[\%]$ for HAR on the three $D_s$: JHMDB, CAD60 and Penn Action. The predictions on test set were unsegmented before computing the $wF1[\%]$. Multiple experiments were performed varying the stride $s$ for each $D_s$.}   {JHMDB} is not up-sampled for {JHMDB}$_{synth 30}$.}
    \resizebox{\columnwidth}{!}{
    \centering
    \begin{tabular}{p{24mm}|p{13.5mm}p{18mm}p{18mm}p{18mm}}
        \hline
        \textbf{Source Datasets $D_s$}  & \textbf{Poses} & \textbf{Synthetic OBD} & \textbf{Synthetic OBD}&\textbf{Synthetic OBD}\\ 
                                        & & & \textbf{[30Hz]}&\textbf{[100Hz]}\\ 
        \hline
        \hline
        \textbf{JHMDB[25Hz]}      & 50.90$\pm$0.05 & 26.58$\pm$0.06 & 26.58$\pm$0.06 & 85.68$\pm$0.81\\ 
        %\hline
        \textbf{CAD60[30Hz]}      & 75.75$\pm$0.02 & 50.11$\pm$0.06 &  50.11$\pm$0.06 & 57.16$\pm$0.06\\ 
        %\hline
        \textbf{Penn Action[50Hz]} & 88.05$\pm$0.27 & 95.21$\pm$0.14 & 67.14$\pm$0.32 & 96.00$\pm$0.08\\ 
        %\hline
        \textbf{NTU[30z]} & 30.07$\pm$0.15 & 6.70$\pm$1.35 & 6.70$\pm$1.35 & 36.59$\pm$0.49\\ 
        \hline
        \multicolumn{5}{c}{\vspace{-6mm}}\\
    \end{tabular}
    }
    \label{tab:ss}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/step_size.tex <==
\begin{table}[h]
    \caption{\scriptsize{The $wF1[\%]$ for HAR on the three $D_s$: JHMDB$_{synth}$, CAD60$_{synth}$ and Penn$_{synth}$. The predictions on test set were unsegmented before computing the $wF1[\%]$. Multiple experiments were performed by fixing $W=1$ and varying the $s$.}}
    \resizebox{\columnwidth}{!}{
        \centering
        \begin{tabular}{cc|cccccc}
            \hline
            \multicolumn{2}{l}{\textbf{}}    & \multicolumn{6}{c}{\textbf{Step Size (s)}}  \\ 
            \textbf{Dataset} & \textbf{Hz} & \multicolumn{1}{l}{1}     & \multicolumn{1}{l}{5}     & \multicolumn{1}{l}{10}    & \multicolumn{1}{l}{12}    & \multicolumn{1}{l}{20}    & 25    \\ 
            \hline
            \hline
            \textbf{JHMDB}   & 100         & \multicolumn{1}{l}{36.66$\pm$0.56} & \multicolumn{1}{l}{46.76$\pm$0.72} & \multicolumn{1}{l}{70.13$\pm$0.39} & \multicolumn{1}{l}{85.68$\pm$0.81} & \multicolumn{1}{l}{66.81$\pm$0.12} & 60.16$\pm$0.42 \\ 
            \textbf{CAD60}   & 100         & \multicolumn{1}{l}{47.66$\pm$0.42} & \multicolumn{1}{l}{49.30$\pm$0.26} & \multicolumn{1}{l}{56.28$\pm$0.12} & \multicolumn{1}{l}{57.16$\pm$0.06} & \multicolumn{1}{l}{51.12$\pm$0.09} & 47.02$\pm$0.42 \\ 
            \textbf{Penn}    & 100         & \multicolumn{1}{l}{96.00$\pm$0.08} & \multicolumn{1}{l}{87.60$\pm$0.72}  & \multicolumn{1}{l}{84.13$\pm$0.18} & \multicolumn{1}{l}{81.81$\pm$0.22} & \multicolumn{1}{l}{77.84$\pm$0.31} & 74.48$\pm$0.09 \\ 
            \hline
        \end{tabular}
    }
    \label{tab:step_size}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/Tables/window_size.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
    \caption{\scriptsize{The $wF1[\%]$ for HAR on the three $D_s$: JHMDB$_{synth}$, CAD60$_{synth}$ and Penn$_{synth}$. The predictions on test set were unsegmented before computing the $wF1[\%]$. Multiple experiments were performed by fixing the $s$ and varying the $W$.}}
    \resizebox{\columnwidth}{!}{
        \centering
        \begin{tabular}{ll|llllll}
            \hline
            \multicolumn{2}{l}{\textbf{}}    & \multicolumn{6}{c}{\textbf{Window Size (W)}}      \\ 
            \textbf{Dataset}                & \textbf{Hz} & \multicolumn{1}{l}{1} & \multicolumn{1}{l}{2}     & \multicolumn{1}{l}{3}     & \multicolumn{1}{l}{4}     & \multicolumn{1}{l}{5}     & 6     \\ 
            \hline
            \hline
            \multirow{2}{*}{\textbf{JHMDB}} & 25             & \multicolumn{1}{l}{26.58$\pm$0.06}  & \multicolumn{1}{l}{25.47$\pm$0.08} & \multicolumn{1}{l}{25.01$\pm$0.11} & \multicolumn{1}{l}{23.57$\pm$0.09} & \multicolumn{1}{l}{23.50$\pm$0.18} &       \\  
            & 100             & \multicolumn{1}{l}{85.68$\pm$0.81}  & \multicolumn{1}{l}{83.43$\pm$0.82} & \multicolumn{1}{l}{66.88$\pm$0.48} & \multicolumn{1}{l}{54.69$\pm$0.38} & \multicolumn{1}{l}{49.27$\pm$0.51} &       \\ 
            \hline
            \multirow{2}{*}{\textbf{CAD60}} & 30             & \multicolumn{1}{l}{50.11$\pm$0.06}  & \multicolumn{1}{l}{88.34$\pm$0.11} & \multicolumn{1}{l}{91.11$\pm$0.09} & \multicolumn{1}{l}{91.94$\pm$0.10} & \multicolumn{1}{l}{94.10$\pm$0.09} & 93.58$\pm$0.19 \\
            & 100             & \multicolumn{1}{l}{57.16$\pm$0.06}  & \multicolumn{1}{l}{56.52$\pm$0.09} & \multicolumn{1}{l}{78.03$\pm$0.15} & \multicolumn{1}{l}{86.63$\pm$0.21} & \multicolumn{1}{l}{92.01$\pm$0.18} & 90.51$\pm$0.09 \\ 
            \hline
            \textbf{Penn}                   & 100            & \multicolumn{1}{l}{96.00$\pm$0.08}  & \multicolumn{1}{l}{95.10$\pm$0.28} & \multicolumn{1}{l}{94.30$\pm$0.37} & \multicolumn{1}{l}{93.10$\pm$0.18} & \multicolumn{1}{l}{92.46$\pm$0.73} &       \\ 
            \hline
        \end{tabular}
    }
    \label{tab:window_size}
\end{table}

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/chapters/01_introduction.tex <==
\section{Introduction}
    
    Human activity recognition (HAR) concerns classifying activities of human movements. HAR is nowadays essential for applications in Industry 4.0, ambient-assisting living, health support, and smart-homes, e.g., activities of daily living (ADLs) \cite{chikhaoui2018cnn,hammerla2016_DCRMHARUW,liu2016human,niemann2020lara}. HAR methods mostly use signals from videos, marker-based motion-capturing systems (marker-based Mocap), or on-body devices. The latter comprise different sensors, e.g., accelerometers, gyroscopes, and magnetometers. On-body devices are also non-invasive, unaffected by occlusion, and do not portray personal identities. Therefore, these devices are suitable for HAR as activities can be tracked and performed in the natural environment. Nevertheless, the high inter-class and intra-class variation of human activities make HAR a challenging task. Besides, HAR datasets suffer from the class imbalance problem. 

    Deep learning-based approaches have been used successfully for solving multi-channel time-series HAR \cite{chikhaoui2018cnn,hammerla2016_DCRMHARUW,Moya_Rueda2020,ramasamy2018recent,yang2015deep}. Deep networks in HAR are layered end-to-end architectures that learn simple to abstract features of human movements. They can learn non-linear and temporal relations of basic, complex, and highly dynamic-human movements from raw time-series data. %Deep networks combine feature extraction and classification in an end-to-end approach \cite{zeng2014convolutional}. 
    They capture the local dependencies of multi-channel time-series data, which are also translation-invariant in time \cite{chen2020}. Deep networks learn more discriminative features of human actions in contrast to statistical pattern-recognition approaches \cite{yang2015deep,zeng2014convolutional}.
    
    However, the performance of multi-channel time-series HAR using deep networks has not shown a significant increase in prediction accuracy as in other fields, such as image and video classification \cite{Moya_Rueda2020,reining2019human}. Considering HAR as a supervised problem, scarcity of annotated HAR data is the primary concern \cite{demrozi2020human,kim2009human}. Supervised learning methods, e.g. deep neural networks, require a large amount of annotated data. The annotation process demands enormous resources. Additionally, annotation reliability varies based on human errors or on unclear and non-elaborated annotation protocols \cite{avsar_2021,feldhorst2016motion,kim2009human,reining2020annotation}.

    Transfer learning can alleviate the problem of scarcity of annotated data. However, it can be hindered by the enormous variation of recording settings, e.g., different recording rates, sensor resolutions, device position, or intrinsic device characteristics. Unlike transfer learning in computer vision tasks where source datasets are large, e.g., Imagenet dataset \cite{Krizhevsky2012-ICD}, source datasets for multi-channel time-series HAR remain scarce. Accordingly, we propose using datasets intended for video-based HAR and human pose estimation as a source for HAR. Specifically, we use the annotations of pixel-coordinate as sequences of human joints. This proposal relates to hybrid approaches of human-pose estimation and HAR in video-based tasks \cite{luvizon20182d,usman2019multi}.
    
    This paper is structured as follows. Sec.~\ref{chap:rw} discusses the deep learning-based methods and transfer learning for HAR. Sec.~\ref{chap:method} presents the method for implementing the transfer learning using human poses and their derivatives. Sec.~\ref{sec:dataset} introduces the three source and three target datasets used in this work. Sec.~\ref{sec:exp} presents and discusses the results obtained from various experiments. Finally, Sec.~\ref{sec:conclusion} draws the inferences. 



==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/chapters/02_relatedwork.tex <==
\section{Related Work}
\label{chap:rw}

    %Statistical pattern recognition methods are common for analysing human movements from measurements from on-body devices. A standard pipeline involves pre-processing, segmentation, hand-crafted feature extraction, and classification. Pre-processing is necessary due to sensor characteristics, sampling rate, and noise; for example, low- and high-pass filtering separates acceleration components due to gravity and the human body; besides, it reduces noise. Segmentation is commonly carried out employing a sliding window approach on the sensor measurements along the time axis. Statistical features are extracted either from the time domain (e.g., mean, variance or correlation) or frequency domain, e.g., entropy, energy or coherence of the Fourier transform \cite{bulling2014tutorial,feldhorst2016motion,laguna2011dynamic,olszewski2001generalized,reining2019human,twomey2018comprehensive}. These features are aggregated using PCA, LDA, or KDA for dimensionality reduction and finally used for training a set of parameters of a classifier. The classifier assigns a class label to an unknown sequence using its extracted and aggregated features \cite{lara2012survey,reining2019human}.
    
    Statistical pattern recognition methods are common for analysing human movements from measurements from on-body devices. A standard pipeline involves pre-processing, segmentation, hand-crafted feature extraction, and classification. Pre-processing is necessary due to sensor characteristics, sampling rate, and noise. Segmentation is commonly carried out employing a sliding window approach on the sensor measurements along the time axis. Statistical features are extracted either from the time domain or frequency domain \cite{bulling2014tutorial,feldhorst2016motion,laguna2011dynamic,olszewski2001generalized,reining2019human,twomey2018comprehensive}. These features are aggregated using PCA, LDA, or KDA for dimensionality reduction and finally used for training a set of parameters of a classifier. The classifier assigns a class label to an unknown sequence using its extracted and aggregated features \cite{lara2012survey,reining2019human}.

    Nowadays, deep learning methods are relevant for solving HAR problems. Deep architectures holistically combine feature extraction and classification, e.g., the temporal convolutional neural networks (tCNNs) for HAR \cite{grzeszick2017deep,twomey2018comprehensive}. \cite{cruciani2020feature,duffner_2014,grzeszick2017deep,moya2018_CNNHARBWS,ronao2015deep,yang2015deep} employed convolution and pooling operations along the temporal dimension to capture local temporal dependencies. Besides, the convolutional filters are shared among all the sensors. The authors in \cite{ordonez2016deep} proposed a deep architecture for HAR, which combines convolution and recurrent layers. This DeepConvLSTM consists of four convolutional layers and three LSTM layers. 
    %Convolution layers do not include a pooling operation. 
    The authors observed that the DeepConvLSTM offers better performance when identifying the start and end of activities. Also, DeepConvLSTM improved the classification performance when compared to results reported by \cite{yang2015deep}, using a four-layered tCNN. 
    %Authors of \cite{ordonez2016deep} observed that LSTM cells capture longer temporal dynamics within the data sequence compared to a tCNN.
    The authors in \cite{grzeszick2017deep,moya2018_CNNHARBWS} proposed a tCNN based architecture for HAR in an industrial setting. The architecture processes data from on-body devices in separate parallel blocks. Temporal convolutions are performed for each block. The temporal convolution layer of each on-body device shares the same weights. A fully connected layer computes an intermediate representation for each parallel block. A subsequent fully connected layer then fuses the intermediate representations. Joining the information of individual on-body devices later in the CNN architecture, i.e., late fusion, makes the IMU-CNN more powerful against slightly asynchronous and inherent characteristics of on-body devices.
    
    HAR can also be performed using human pose estimates. In \cite{luvizon20182d}, authors combined human pose estimations from images and sequences of RGB frames to create an end-to-end architecture for HAR from videos. The authors used a differentiable soft-argmax for pose estimation. This layer allowed an action recognition network to be stacked on top of the pose estimator, resulting in an end-to-end trainable network. In \cite{cippitelli2016human}, the authors proposed an activity recognition algorithm exploiting skeleton data extracted by RGBD sensors. Human joint-poses are recorded using a Microsoft Kinect. Subsequently, a multiclass Support Vector Machine classifies activities.
    
    Supervised deep learning methods require substantial labelled data to produce decent results. However, annotated on-body devices data is scarce as the annotation process is expensive, time-consuming, tedious, and requires domain expertise \cite{avsar_2021,chen2020,reining2020annotation}. In the context of deep networks, transfer learning gives an alternative to the problem of scarcity of annotated data \cite{Moya_Rueda2020,ordonez2016deep_conv}. Transfer learning uses a network trained on a source task to initialise a network on a related target one. In \cite{ordonez2016deep_conv}, authors characterised the feasibility, benefits, and drawbacks of performing transfer learning in three scenarios: subjects within a dataset, different datasets, on-body device locations, and sensor type. They created a network with three convolutional layers alternated with max-pooling layers, followed by an LSTM and a softmax layer. The authors considered windows of $9.7$ sec. They varied the number of transferred layers. For the first case, the authors concluded that the filters of the lower layers are more generic, thus, transferable. The authors inferred that performance varies when the source and target datasets are different for the second case; the type of activities in the source domain negatively affects the transfer learning performance. Finally, there was significant degradation in performance when transferring between modalities and locations irrespective of the number of transferred layers.
    
    In \cite{chikhaoui2018cnn}, authors investigated the transfer learning performance on three scenarios: across subjects of different ages using the same on-body device on the same location, different positions of on-body devices, and different sampling rates and sensor types. The authors inferred that transfer learning between any on-body device placement is possible. In addition, lower layers capture generic features independent of the sampling rate. In \cite{Moya_Rueda2020}, authors introduced a method for transfer learning from human joint-poses from a Mocap system as a source and inertial measurements obtained from on-body devices as the target dataset. They used a tCNN \cite{yang2015deep} and an IMU-CNN \cite{grzeszick2017deep,moya2018_CNNHARBWS}, trained using sequences of human joint-poses or their derivatives. They used a sliding window of $1$ sec. The authors performed transfer learning across three target domains with different activities, numbers of on-body devices, and recording rates. The authors inferred that the performance improved for both networks on three target datasets. Furthermore, results are valid even when fine-tuning with a proportion of the datasets.
    
    Transfer learning has been carried out among datasets from on-body devices. These datasets remain, however, scarce or limited sized. Besides, they contain annotations of task-related activities. Therefore, exploiting other data sources might be interesting for transferring purposes in HAR.

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/chapters/03_method.tex <==
\section{Human Poses for HAR}
\label{chap:method}
    Considering the conclusions in \cite{Moya_Rueda2020}, sequences of human poses serve as a source for transfer learning for multi-channel time-series HAR purposes. We propose to extend it by considering sequences of human poses from data of different purposes. We use \textbf{annotations} of pixel-coordinate sequences of human joints from video data intended for video pose estimation. These datasets contain annotated recordings from different scenarios with a broad range of human activities in the wild. Thus, we seek to squeeze the usability of these datasets for multi-channel time-series HAR. These human-pose annotations from videos can be considered multi-channel time-series of human movements. We use the second derivative of a smooth piecewise spline interpolation of degree five on a small-time interval from sequences of human joint-poses for simulating on-body devices attached to the poses, a sort of synthetic data. In line with \cite{gurjar2018_LDRWSUWS,Moya_Rueda2020}, synthetic data could also be beneficial for transfer learning, improving performance on a limited-sized datasets.  Fig.~\ref{fig:networks} shows the proposed method.
    %\textcolor{red}{The double differentiation helps to simulate IMU sensor data by transforming the pose data into synthetic IMU data.} 
    
    \input{figures/network}
    
\subsection{Temporal Convolutional neural network}
    \label{section:tcnn}
    
    The temporal convolutional neural network (\textit{tCNN}) and the \textit{tCNN-IMU} are used as feature extractors and classifiers, based on \cite{grzeszick2017deep,Moya_Rueda2020,moya2018_CNNHARBWS,niemann2020lara,yang2015deep}. %\textcolor{red}{The tCNN can be considered as an tCNN-IMU, but with a single branch.}
    The \textit{tCNN-IMU} \cite{grzeszick2017deep} consists of five branches, each with four temporal-convolution layers ($c1,c2,c3,c4$) having $64$ filters of size $[5,1]$. The five branches are assigned measurements of the four limbs and the torso, i.e., left-arm (LA), right-arm (RA), left-leg (LL), right-leg (RL), and head-neck or torso (N). If the measurements for one or more branches are missing, then those branches are removed. A fully-convolutional layer computes a representation per block. The five representations are concatenated and fed to a fully-convolutional layer. Finally, a softmax layer is present at the end to classify human activities. The \textit{tCNN} can be considered as an architecture with a single block. Both architectures successively process a sequence of human activity windows of dimensions $[W,D]$. %\textcolor{red}{ This work focuses on transfer learning to solve the problem of scarcity of data; therefore, we choose the state of the art techniques\cite{Moya_Rueda2020} to train the model.}
    Each architecture is trained using batch gradient descent with the RMS-Prop update rule with a momentum of $0.9$, weight decay of $5\times10^{-4}$, and three different learning rates $[10^{-3},10^{-4},10^{-5}]$. The learning rate for every experiment is selected according to the results on the validation set. Dropout is applied after the first and second fully-connected layers. The categorical cross-entropy loss function is used. Orthonormal initialization is deployed for initializing the weights. A data augmentation technique adds Gaussian noise $[\mu =0,\sigma =0.01]$ to input data. 
    
    %tCNNs are end-to-end architectures that combine learnable convolutional filters along the time axis (T) with non-linear operations with a classifier. Convolutional filters are shared among all the channels. Filters extract temporal relations at different temporal locations from the different sensor measurements. tCNNs map a window of multi-channel measurements into a class representation. The channels are measurements from different on-body devices along the three axes, denoted by $D$. The temporal relations are likely to be correlated independently of the type of sensor.
    

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/chapters/04_experiments.tex <==
%\vspace{-1em}
\section{Datasets}
\label{sec:dataset}
    We use various source datasets $D_s$ containing human-pose annotations as the ground-truth annotations of video datasets for HAR and pose estimation, namely the JHMDB, CAD60, Penn Action and the NTU RGB+d benchmark datasets. These pose data comprises 2D (x,y) pixel coordinates or 3D (x,y,z) with an additional depth annotation. Annotations along each axis are treated as a separate channel. Target datasets $D_t$ comprise on-body devices recordings of human activities. These datasets are the Pamap2, Opportunity, and LARa. The $D_s$ are split into training ($70\%$), validation($15\%$), and testing($15\%$) sets, following \cite{ordonez2016deep}.
    
    %A window size of $1$ second is used \cite{banos2014window}.%The $D_s$ and $D_t$ are split into training ($70\%$), validation($15\%$), and testing($15\%$) sets, following \cite{ordonez2016deep}. A window size of $1$ second is used for all datasets.

    
    \subsection{Source Datasets ($D_s$)}
    
        \textbf{JHMDB} \cite{Jhuang:ICCV:2013} contains $928$ video clips of different human actions in the wild. The dataset comprises $21$ activities. The person performing the activity in each frame is manually annotated with their $2D$ joint positions. %, scale, viewpoint, segmentation, puppet mask and puppet flow.
        The joint positions correspond to LA, LL, RA, RL, and N. Every activity class contains $36-55$ video clips, and each clip contains $15-40$ frames. The video clips are recorded at a rate of $25$ Hz. The duration of activities ranges from $0.5-2$ sec. %The JHMDB is a small dataset with a total duration of all video clips of around $20$ min.
            
        \textbf{CAD-60} \cite{sung2014cornell} contains RGB-D video sequences of human activities, which are recorded using the Microsoft Kinect v1 \cite{6190806}. The dataset contains $[320\times 240]$ sized RGB-D motion sequences and skeletal information acquired at $30$ Hz. The skeletal information is composed of $15$ $3D$-joint positions per skeleton. The $3D$ coordinates are extracted from the depth data. The joint positions correspond to LA, LL, RA, RL, and N. The activities are performed by four subjects in five different constrained environments.
        %: office, kitchen, bedroom, bathroom, and living room. 
        The subjects perform $12$ activities. The total recorded time for all the activities is approximately $47$ min.
            
        \textbf{Penn Action} \cite{zhang2013actemes} consists of $2326$ videos, recorded at $50$ Hz, of different human actions in the wild. The annotations comprise $15$ activity classes, $13$ 2D human joint-poses in each video frame, and camera viewpoints. The dataset contains $13$ 2D positions of human joints, specifically from head, shoulders, elbows, wrists, hips, knees and ankles. The total recorded time for all the activities is approximately $55$ min.  
        
        %The dataset consists of the following $15$ action classes.
        %: \textit{baseball pitch}, \textit{baseball swing}, \textit{bench press}, \textit{bowling}, \textit{clean and jerk}, \textit{golf swing}, \textit{jump rope}, \textit{jumping jacks}, \textit{pull up}, \textit{push up}, \textit{sit up}, \textit{squat}, \textit{strum guitar}, \textit{tennis forehand} and \textit{tennis serve}.
        %The authors in \cite{zhang2013actemes} capture discriminative action-specific patches for each frame and compute partial spatiotemporal pose information. Each patch, implicitly captures the intricate pose, dynamics, self-occlusion and spatial appearance of a subset of body parts in a spatiotemporal neighborhood.
            
        \textbf{NTU RGB+D} \cite{shahroudy2016ntu} contains $60$ activity classes and $56,880$ video samples. The dataset contains RGB videos, depth map sequences, 3D skeletal data, and infrared (IR) videos for each sample. Videos are captured from $40$ different subjects, using Microsoft Kinect v2 at $30$ Hz. Skeletal data consists of $3D$ locations of $25$ major body joints for detected and tracked human bodies. The joint locations correspond to LA, LL, RA, RL, and N.
        
        %The actions are  performed in different constrained  environments: $40$ daily actions (drinking, eating, reading, etc.), $9$ health-related actions (sneezing, staggering, falling down, etc.), and $11$ mutual actions (punching, kicking, hugging, etc.).

    \subsection{Target Datasets ($D_t$)}
        \textbf{Pamap2} \cite{reiss2012introducing} contains recordings of three on-body devices from nine subjects performing Activities of daily living. Here, the on-body devices are placed on the dominant ankle, dominant hand, and chest. Pamap2 dataset uses a recording rate of $100$ Hz. The subjects perform $18$ activities. The total recorded time for all the activities is approximately $324$ min. The
        validation set contains recordings from subject $5$, and testing from subject $6$.      
        
        \textbf{LARa} \cite{niemann_friedrich_2020_3862782,niemann2020lara} contains recordings of human poses and inertial measurements from $14$ subjects performing activities in the intralogistics. The dataset provides recordings of an Optical Marker-based Motion Capture (OMoCap), called LARa-MoCap, with a recording rate of $200$ Hz, and two sets of on-body devices, with a recording rate of $100$ Hz, called LARa-Mbientlab (LARa-Mb) and LARa-MotionMiners (LARa-MM). The LARa-MM considers only three on-body devices and on different locations than LARa-Mb. In LARa-MoCap, $3D$ poses of $22$ joints are present. LARa-Mb consists of $3D$ linear and angular acceleration measured from five on-body devices attached to LA, LL, RA, RL, and torso. Whereas, LARa-MM consists of measurements from three on-body devices; LA, RA, and N. The dataset is strongly unbalanced. The \textit{handling (centred)} class constitutes $60\%$ of the complete recordings. For LARa-MoCap, the validation and test set contain recordings from subjects $[5,11,12]$ and $[6,13,14]$ respectively. Similarly, for LARa-Mb and LARa-MM, the validation set consists of measurements from subjects $[11,12]$ and testing from subjects $[13,14]$.
            
        \textbf{Opportunity} \cite{chavarriaga2013opportunity} contains recordings of seven on-body devices from four subjects performing ADLs. Subjects perform the activities in a room simulating a studio flat with a deckchair, a kitchen, doors giving access to the outside, a coffee machine, a table, and a chair. The activities were recorded using seven on-body devices, twelve 3D-acceleration sensors, four 3D localization information, and object sensors, with a recording rate of $30$ Hz. The sensor measurements correspond to LA, LL, RA, RL, and N. The user's activities were annotated on different levels: 17 mid-level gesture classes (Opp-Gest) and five high-level locomotion (Opp-Loc) classes. The validation set contains the ADL3 recordings from subjects $[2,3]$, and testing ADL4 and ADL5 recordings from subjects $[2,3]$. Other recordings are a part of the training set.
        
        %\textcolor{red}{For all the datasets, firstly, the given pose annotations are visualised. Subsequently, the joints are identified, which are mapped to the branches of \textit{IMU-tCNN}. The mapping is available in the repository. However, for Penn Action, there is no clarity of the joints; therefore, mapping is not possible.}
        
        %The ADLs consist of \textit{lying}, \textit{get up}, \textit{groom}, \textit{relax}, \textit{prepare coffee}, \textit{drink coffee}, \textit{prepare sandwich}, \textit{eat}, and \textit{cleanup}. 

\section{Experiments and Results}
\label{sec:exp}
    The \textit{IMU-tCNN} with $five$ branches, each per human limb, and a \textit{tCNN}, in Fig.~\ref{fig:networks}, are pre-trained on different $D_s$. The convolutional layers of the pre-trained networks \textit{IMU-tCNN}$_{D_s}$ and \textit{tCNN}$_{D_s}$ are transferred to a \textit{tCNN} to be trained on the $D_t$, denoted by \textit{tCNN}$_{D_s}^{D_t}$. The number of transferred convolutional layers ($N_{conv}$) and the $\%$ of $D_t$ for fine-tuning vary$^1$. The transferred convolution layers are not frozen$^2$. The non-transferred convolution and fully-connected layers of the \textit{tCNN}$_{D_s}^{D_t}$ are trained from scratch. HAR is a multi-class classification problem, and all datasets are highly unbalanced. Thus, the weighted $F1$ score ($wF1$) \cite{ordonez2016deep} is used as a performance metric. This metric weighs each activity class equally using precision and recall. The results presented in this work are the mean and standard deviation $(\mu\pm \sigma)$ from five runs, with a random seed of $42$. A permutation test is performed to evaluate the performance changes. The testing accuracy will be considered for this permutation test \cite{ojala2010permutation}. For Penn Action, it is not possible to estimate a joint corresponding to a pose estimate in the dataset. As \textit{IMU-tCNN} uses branches for processing measurement from specific joints, therefore Penn Action cannot be trained using \textit{IMU-tCNN}.  %\textcolor{red}{Penn Action is only trained using \textit{tCNN}.} 
    The values in bold in all the tables have the corresponding testing accuracy significantly higher than the baseline one, based on a permutation test.
    
    \def\thefootnote{1}\footnotetext{Implementation of the two architectures, pre-processing of datasets, training and testing are found in https://github.com/shrutarv/Create-Synthetic-IMU-data.}
    \def\thefootnote{2}\footnotetext{Freezing the transferred convolutional layers showed lesser performance: thus, they are not presented here, however they can be found in the github.}
    \def\thefootnote{3}\footnotetext{Considering the joint-pose annotations as multi-channel time-series data for HAR defers from the video-based HAR approaches intended for $D_s$.}
    
    %Permutation test assesses the probability that the difference between the true and predicted accuracy is explained by chance \cite{ojala2010permutation}.

    
    \subsection{HAR from Source Datasets}
    
        Following the method in Fig.~\ref{fig:networks}, HAR will be considered using transfer learning from ground-truth annotations of joint poses to real on-body data. The JHMDB, CAD60, Penn Action, and NTU will be used as $D_s$. Concretely, we consider the sequences of joint-pose annotations in pixel coordinates as multi-channel time-series data for HAR. Besides, their second order-derivatives will also be deployed as a source for multi-channel time-series HAR$^3$. The derivatives will be called synthetic on-body devices. This consideration takes the advantage that the \textit{IMU-tCNN} and \textit{tCNN} process sequences per channel with late fusion and local temporal-neighbourhoods of sequences are likely correlated. 
        The joint poses sequences of $D_s$ are either up-sampled or down-sampled to match the frequency of the $D_t$. The JHMDB, CAD60, Penn, and NTU are up-sampled by factors of $[4,3,2,3]$ respectively for $D_t$=\textit{Pamap2} as target and by factors of $[1,1,0.5,1]$ for $D_t$=\textit{Opp}. We deploy a smooth piecewise spline interpolation of degree five on a small time-interval from a sequence of joint-pose annotations per channel; accordingly, the second order-derivative of the spline approximation is used as synthetic on-body devices. 
        A sliding window approach with $T=1$sec. $W$ depending on the sampling rate, and a stride of $s$ is used for segmenting sequences of human poses; specifically, the following parameters were used: a window size of ($W=25$) and a stride of $s=12$ for JHMDB$_{pose}$, a window size of ($W=30$) and a stride of $s=12$ for the CAD60$_{pose}$, a window size of ($W=50$) and a stride of $s=1$ for the Penn$_{pose}$ and a window size of ($W=30$) and a stride of $s=3$ for the NTU$_{pose}$. 
        
        %\textcolor{red}{The duration of most activities in $D_s$ is between $0.75$ to $2$ sec. Tab.~\ref{tab:window_size} shows that for CAD60, the recognition accuracy was highest when $W=5$. However, the $wF1$ score for transfer learning from CAD60 to $D_t$ was similar for when $W=1$ and $W=5$. The results for $W=5$ are available in the repository. Therefore, for generality and based on results from \cite{reining2019human}, $W=1$ is chosen for training all the $D_s$. Moreover, conclusions from \cite{banos2014window} further support the decision of choosing $W=1$. We performed experiments with step sizes $1,3,5,10,12,15,$ and $20$ and chose the one that gave the best $wF1$ score. Table \ref{tab:step_size} shows the $wF1[\%]$ for HAR on the three $D_s$: $JHMDB_{synth}$, $CAD60_{synth}$ and $Penn_{synth}$. The $W$ is fixed at $1$ and $s$ is varied.  This work aims to show that transfer learning can alleviate the scarcity of data; therefore, extensive experiments with different $W$ and $s$ are not performed.} %window size of $0.5sec$, $1$sec, and $2$sec 
        
        Channels are normalized to zero-mean and unit deviation. Following the pre-processing protocol in \cite{niemann2020lara}, we normalize the joint-poses with respect to the torso for JHMDB and CAD60, head for Penn, and middle of the spine for NTU.
        %\input{Tables/window_size}
        %\input{Tables/step_size}
        We consider multi-channel time-series HAR using the tCNN on the four $D_s$. Table \ref{tab:ss} shows the classification performance in terms of $wF1[\%]$ on their testing sets. The $wF1[\%]$ on the JHMDB$_{synth.}$, CAD$_{synth.}$ and NTU$_{synth.}$, the synthetic on-body devices, decreases when compared to pose data. These results are due to the approximations involved in the creation of synthetic data. The HAR performance increases when up-sampling for JHMDB$_{synth.}$ and NTU$_{synth.}$ to $100$Hz and decreases when down-sampling for Penn$_{synth.}$ to $30$Hz. 
        
        \input{Tables/pose_datasets}
        
        We consider multi-channel time-series HAR using joint poses differently from the approaches in \cite{choutas2018potion,javidani2021learning,usman2019multi} as video-based HAR. Interestingly, for JHMDB$_{synth.}$, upsampled to $100$Hz, we obtain a mean classification accuracy of $90.53\%$, which is significantly higher than the one reported by \cite{choutas2018potion} ($85.5\%$), \cite{javidani2021learning} ($77.54\%$), and \cite{usman2019multi} ($83.1\%$). The predictions were unsegmented, and a majority voting was deployed before computing the $wF1[\%]$ so that a comparison would be fair. All three pieces of research focused on HAR from videos, using RGB frames, Optical Flow and Pose. The authors in \cite{choutas2018potion} introduced the PoTion representation to encode the motion of joint poses over a video clip as an input. They used the 3D ConvNet (I3D), proposed by \cite{carreira2017quo}. In \cite{usman2019multi}, the authors combined a two-streams CNN---RGB and Optical flow---with a prediction and the ground truth of human joints from videos. They utilized a fixed tree-like tensor for representing the joint poses. Besides, they deployed early, middle and late fusion of the streams. In \cite{javidani2021learning}, authors pre-trained a CNN to extract feature maps from optical-flow images. A $1D$-CNN is used to extract temporal information from these flow-feature maps. We consider HAR using the ground-truth of human poses from the $D_s$ as multi-channel time-series and not tree-like tensors. 
        
        %These results are not the goal of this work, but they are worth to be noted.

        %\subsection{HAR from Target Datasets}
        
        \subsection{Transfer learning from $D_s$ to Pamap2\\}
        
            \input{results/Pamap2}
            
            
        \subsection{Transfer Learning from $D_s$ to LARa-Mb and LARa-MM\\}
       
            \input{results/LaraOB}
            \input{results/LaraMM}

        \subsection{Transfer Learning from $D_s$ to Opportunity\\}
        
            \input{results/opportunity}

        
        \subsection{Comparison to state of the art}
            
            Tab.~\ref{tab:wf1} presents the performance of the three pre-trained architectures on the $D_t$. Compared with the Opportunity and Pamap2, pre-training the \textit{tCNN} with the four source datasets, with both the pose annotations or the synthetic on-body devices, significantly influences the HAR's performance on the $D_t$, especially when transferring the first convolutional layer. 
            The more sophisticated networks, \textit{B-LSTM} and \textit{tCNN-LSTM}, present the highest performance. Additional experiments using these types of networks are required. However, following the results in Tab.~\ref{tab:TL_S_Pamap2}-\ref{tab:TL_S_Loc}, the performance in all scenarios with the \textit{tCNN} significantly improves when considering a lesser quantity of training material for the target dataset ($10,30,50,75$)[\%], pre-training with the four source datasets with pose annotations, or the synthetic on-body devices.
       
            \begin{table}
             %\vspace{-3em}
                \centering
                \caption{\scriptsize{The $wF1\%$ of the best $tCNN_{D_s}^{D_t}$ on the four target datasets compared to similar works using the same architecture. The results from \cite{Moya_Rueda2020}, denoted with "*", show the performance of pre-training the network with a large MoCap dataset.}}
                \resizebox{\columnwidth}{!}{
                \begin{tabular}{c|c|c|c| c|c} 
                \hline
                \textbf{Dataset} & \textbf{LARa-Mb} &\textbf{LARa-MM} &\textbf{Pamap2} & \textbf{Opp (Loc.)} & \textbf{Opp (Ges)} \\
                \hline
                B-LSTM \cite{hammerla2016_DCRMHARUW} &- &- & -& - & 90.8\\ 
                tCNN-LSTM\cite{ordonez2016deep}& - &- & - & 89.5 & 91.5\\ 
                tCNN \cite{yang2015deep}& - &- & - & 86.5 & 93.9\\ 
                tCNN\cite{Moya_Rueda2020} & 75.75$\pm$0.4 & - & 87.04 $\pm$0.4 & 84.53 $\pm$0.2 & 88.20$\pm$0.4\\ 
                tCNN*\cite{Moya_Rueda2020} & 76.19$\pm$0.2 & - & 90.95 $\pm$0.4 & 88.43 $\pm$0.3 & 91.31$\pm$0.0\\ 
                \hline
                tCNN(replicated) & 75.06$\pm$0.01  & 65.71 $\pm$0.01 & 86.67 $\pm$0.06  & 85.67 $\pm$0.01 & 87.36 $\pm$0.05\\ [0.4ex] 
                tCNN$_{JHMDB}$ & 75.47 $\pm$0.01  & 65.71$\pm$0.02 & 89.70 $\pm$0.01  & 86.84$\pm$0.41 & 89.05$\pm$0.02\\
                tCNN$_{CAD60}$ & 74.94 $\pm$0.01  & 65.67$\pm$0.01 & 89.73 $\pm$0.00  & 86.87$\pm$0.02 & 89.11$\pm$0.51\\
                tCNN$_{Penn}$ & 75.24 $\pm$0.01  & 65.97$\pm$0.01 & 90.64 $\pm$0.85  & 86.70$\pm$0.01 & 88.96$\pm$0.23\\
                tCNN$_{NTU}$ & 75.90$\pm$0.01  & 64.79$\pm$0.01 & 91.23 $\pm$0.85  & 87.21$\pm$0.18 & 89.19$\pm$0.33\\
                \hline
                %tCNN$_{JHMDB}^{50\%D_t}$ & 62.66$\pm$0.61  & 58.09$\pm$0.68 & 89.63$\pm$0.05  & 85.60$\pm$0.56 & 87.06$\pm$0.08\\
                %tCNN$_{CAD60}^{50\%D_t}$ & 62.36$\pm$0.79  & 52.73 $\pm$0.92 & 89.03$\pm$0.16  & 85.62$\pm$0.36 & 87.01$\pm$0.07\\
                %tCNN$_{Penn}^{50\%D_t}$ & 61.83$\pm$0.62  & 53.30$\pm$0.47 & 83.91$\pm$0.81 & 85.10$\pm$0.29 & 87.52$\pm$0.09\\
                %tCNN$_{NTU}^{50\%D_t}$ & 62.96$\pm$0.40  & 56.42$\pm$0.57 & 85.95$\pm$0.90 & 85.62$\pm$0.25 & 86.96$\pm$0.04\\
                %\hline
                \multicolumn{6}{c}{\vspace{-10mm}}\\
                \end{tabular}
                }
                %\vspace{-3em}
                \label{tab:wf1}
                 
            \end{table}
    

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/chapters/04_experiments_text_comments.tex <==
            \begin{table}[ht]
            \begin{tabular}{|l|l|l|l|}
                \hline
                \textbf{Source Datasets $D_s$}      & \textbf{$\%$ test Accuracy unseg} & \textbf{$\%$ test Accuracy seg} & $\%wF1$\\ \hline
                \textbf{JHMDB}      & 81.45$\pm$0.032 & 91.18$\pm$0.027 &  90.53$\pm$0.003\\ 
                \hline
                \textbf{CAD60}      & 36.78$\pm$0.003 & 56.28$\pm$0.02 &  49.50$\pm$0.015 \\ 
                \hline
                \textbf{Penn Action} & 77.76$\pm$0.002 & 91.82$\pm$0.026 & 90.98$\pm$0.06 \\ 
                \hline
            \end{tabular}
            \caption{Experimentally obtained best ss for $D_s$. The ss is chosen based on the highest obtained unsegmented validation accuracy for each dataset.}
            \label{tab:ss}
        \end{table} 
        
    
    \begin{comment}
    \subsection{Transfer Learning from JHMDB to PAMAP2}
        \label{subsection:TL}
        
        The hyperparameters used for training the network are: (1) momentum of $0.9$, (2) learning rate of $10^{-5}$, (3) 100 epochs, and (4) batch size of 400. 
            
       
        Table \ref{tab:Pose_acc} shows the best result for JHMDB using tCNN trained from scratch for HAR ($tCNN_{JHMDB}$).As observed, the $wF1[\%]$ score is higher for $tCNN_{JHMDB}$ than $tCNN_{JHMDB\_p}$. A possible reason could be that, as the pose data is up-sampled by $4$ and the percent overlap of sliding windows is increased to $88\%$, therefore more data is available for training. The new data is an approximation of the real data. This enables the network to learn generic filter and tCNN is able to generalize better. As a result, the $tCNN_{JHMDB\_S}$ learns better and gives a higher $wF1[\%]$ score.
    
        \begin{table}[]
            \centering
            \resizebox{\columnwidth}{!}{
            \begin{tabular}{|c| c |c| c|c|c|c|} 
            \hline
            Metric
            & $tCNN_{JHMDB}$ & $tCNN_{JHMDB\_S}$& $tCNN_{CAD60}$ & $tCNN_{CAD60\_S}$& $tCNN_{Penn}$ & $tCNN_{Penn\_S}$\\
            \hline
            wF1[\%] & 53.2857 &91.13 &70.90$\pm$0.65 &47.5 $\pm$1.5 & 86.3$\pm$0.27&81.3$\pm$0.32\\ 
            
            \hline
            \end{tabular}
            }
            \caption{The $wF1[\%]$ for HAR using $tCNN_{D_s}$. The network is trained from scratch on the pose data and synthetic IMU data. The target dataset is considered as PAMAP2, therefore $D_s$ are sampled to $100$ fps.}
            \label{tab:Pose_acc}
        \end{table}
        
        
        The $wF1\%$ and $\%$test accuracy for $tCNN_{JHMDB\_pamap2}$ are shown in table \ref{tab:tf_JP}. The obtained $\%wF1$ score is highest for $tCNN_{JHMDB\_pamap2^{c1}}$. Thus, further experiments are performed by fixing the number of transferred layers to $c1$ and varying the target data[\%].
       
        \begin{table}[]
        \centering
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\textbf{$\%D_{t}$}} & \multicolumn{2}{l|}{\textbf{$tCNN_{JHMDB\_PAMAP2}$}}           & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}}             & \multirow{}{}{\textbf{p value}} \\ \cline{3-6}
                                                     layers&                                  & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc}   &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 87.95$\pm$0.06          & 88.98$\pm$0.05          & 86.67$\pm$0.05          & 87.8012$\pm$0.04          & 0.005912                          \\ \hline
        c1,c2,c3                                     & 100                              & 87.70$\pm$0.06          & 88.51$\pm$0.07          & 86.67$\pm$0.05          & 87.8012$\pm$0.04          & 0.100044                          \\ \hline
        c1,c2                                        & 100                              & 88.57$\pm$0.05          & 89.32$\pm$0.06          & 86.67$\pm$0.05          & 87.8012$\pm$0.04          & 0.00034                           \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{88.97$\pm$0.08} & \textbf{89.53$\pm$0.07} & \textbf{86.67$\pm$0.05} & \textbf{87.8012$\pm$0.04} & \textbf{0.00002}                  \\ \hline
        c1                                           & 75                               & 86.15$\pm$0.05          & 87.20$\pm$0.06          & 86.30$\pm$0.06          & 87.10$\pm$0.08            &     0.843                              \\ \hline
        c1                                           & 50                               & 86.10$\pm$0.06          & 86.93$\pm$0.08          & 84.10$\pm$0.08          & 84.98$\pm$0.07            &        0.00004                           \\ \hline
        c1                                           & 30                               & 85.55$\pm$0.04          & 86.13$\pm$0.05          & 84.05$\pm$0.09          & 84.93$\pm$0.06            &   0.0107                                \\ \hline
        \end{tabular}
        }
        \caption{The table shows $wF1[\%]$ for $tCNN_{JHMDB\_pamap2}$. The $wF1[\%]$ and $\%$test accuracy of $tCNN_{PAMAP2}$ is used as the baseline. The number of convolution layers transferred are varied.}
        \label{tab:tf_JP}
        \end{table}
        
        
        
        %\begin{flushleft}
        \it{Discussion}\\
        %\end{flushleft}
         The results in table \ref{tab:tf_JP} show that the performance of HAR using tCNN on PAMAP2 improves when pre-training with JHMDB dataset. The JHMDB and PAMAP2 dataset contain $50\%$ overlapping classes (sit, walking, run, ascending stairs, and stand).\\
        
        Consider the results in table \ref{tab:tf_JP}, when $100\%$ of target data (PAMAP2) was used and the number of transferred layers is varied. The the p value when transferring one, two, or four layers indicate that the increase in $\%wF1$ score is highly significant.  It is observed that the best improvement in $wF1\%$ score occurs when only the first c1 is transferred. As the number of transferred layers increase, the $wF1\%$ gradually decreases. A possible explanation could be that the lower-layers (near the input) of a CNN capture generic or high level features \cite{ordonez2016deep_conv}. Deeper layers (near the output) of the network capture more scenario-specific filters, leading to a decrease in transferability.\\
        
        The number of layers transferred is fixed at $c1$ and the amount of target data used is either $50\%$ or $30\%$ or $70\%$. It is observed in table \ref{tab:tf_JP} that the $wF1\%$ when using a $tCNN_{JHMDB\_PAMAP2}$ is higher than the $wF1\%$ of a $tCNN_{PAMAP2}$. The increase is highly significant when $50\%$ or $30\%$ of target data is used for fine tuning. However, when $75\%$ of target data is used. This implies that using a pre-trained tCNN for HAR improves the performance ($wF1$) significantly when the annotated training data is scarce.\\
        
        Table \ref{tab:TL_PR}, shows the precision and recall values. For comparing the performance of $tCNN_{JHMDB\_PAMAP2}$, the harmonic mean (HM) of precision and recall is computed for each activity. The activities  climb stairs, sit, run, walk, and stand are common between PAMAP2 and JHMDB. It is observed that implementing transfer learning results in an increase in HM of the activities: climb stairs, sit, and stand. As these activities are common between the JHMDB and PAMAP2 dataset, therefore the filters learnt by the initial layers of the tCNN are generic to these common activities and can be transferred.\\
        
        The performance of the activity Run is nearly the same. There is a slight reduction in the harmonic mean for the class walk. A possible explanation could be that the walking activity in JHMDB consists of $41$ videos from internet and all videos have different subjects performing the activity. The walking speed of these subjects varies significantly. In some videos the subjects seems to be running and in some the subject is dawdling. Also, there is a large intra-class variability in the walking class. In some videos have the person dragging or carrying objects while walking. Therefore, the first layer of the pre-trained network might have learnt features which are not generic to the walking activity. Thus, for fro $tCNN_{JHMDB_PAMAP2^{c1}}$, the network might confuse walking activity with other activities.\\
        
        There is also an increase in harmonic mean for activities, which are only present in PAMAP2 dataset: rope jump, descending stairs, vacuum cleaning and ironing. The activity rope jump in PAMAP2 could be considered similar to the Jump action in JHMDB. The ironing action can be considered similar to the pour action in JHMDB. As both ironing and pour actions involve one arm to be stationary and a side-ward movement of the other arm. Also, the persons performing these two actions are mostly standing and perform the actions approximately at a height of their stomach. Similarly, the action of vacuum cleaning could be considered similar to the pick action. As, both actions involve a combination of bending and movement of arms. The action descending stairs can be considered similar to ascending stairs. The harmonic mean for the above mentioned similar activities increases. The performance for actions cycling and lying is nearly the same. However, the performance for action Nordic Walk decreases. A possible reason could be that even the features of the first layer of the pre-trained network are not generic enough to represent the Nordic Walk action. Subsequently, this might hinder with learning of specific features for Nordic Walk action in deeper layers. \\
        
        Summing up the results, it can be said that transfer learning from JHMDB to PAMAP2 significantly improves the performance of tCNN trained on PAMAP2 for HAR. 9 out of 12 activities in PAMAP2 are similar to JHMDB. As a result the lower layers learn features that are generic to human activities. The features of the lower layer are more generic than higher layers. This also suggests that filters learn short temporal-relations from the input sequence per channel independently of the rather related domain. Also, when annotated data is scarce ($30\%$) then transfer learning is advantageous. \\
        \end{comment}
        %%%%%%%%%%%%%%%%%%%%%%%%
        
        
        
        
            
        
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{comment}
    \subsection{Transfer Learning from CAD60 to PAMAP2}
    \label{subsection:TL_C_P}
    
        
       
        The table \ref{tab:Pose_acc} shows the best result for CAD60 dataset, trained from scratch using tCNN. \\
        
        As seen in table \ref{tab:Pose_acc}, the $wF1[\%]$ is higher when tCNN is trained using CAD60 pose data than when tCNN is trained with synthetic IMU data. Fig \ref{fig:J_CAD} represents (a) pose data for two random channels for first 100 frames of JHMDB dataset and (b) CAD60 dataset. Similar time-series signal are observed for all the channels in CAD60 for the entire duration of the recording. As observed in Fig \ref{fig:J_CAD}, the data points that are close to each other in CAD60 dataset have extreme differences in values. This causes incorrect approximations due to smoothing effect. All the channels of the CAD60 dataset show a similar behaviour. Up-sampling could be the reason for the incorrect approximations. Therefore, the approximated values by spline interpolation are not accurate, and the features learnt by the network are inaccurate. This explains the decrease in $wF1$ score.   
        \begin{figure}[]
        \begin{center}
        \includegraphics[scale=0.6]{J_CAD}
        \end{center}
        \caption {shows (a) pose data for $2$ random channels for first 100 frames of JHMDB dataset and (b) pose data for $2$ random channels for first 100 fames of CAD60 dataset.}
        \label{fig:J_CAD}
        \end{figure} 
        
        
        The $wF1\%$ and $|\%$ test accuracy for $tCNN_{JHMDB\_PAMAP2}$ is shown in table \ref{tab:tf_CP}. $tCNN_{PAMAP2}$ is considered as the baseline for comparison. The $wF1$ score is highest when transferring only first layer from CAD60 to PAMAP2. Thus, further experiments are performed by fixing the number of transferred layers to $c1$ and varying the target data[\%].
        \begin{table}[H]
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. layers}} & \multirow{}{}{\textbf{$\%D_{LaraMM}$}} & \multicolumn{2}{l|}{\textbf{$tCNN_{CAD60\_PAMAP2}$}}           & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}}           & \multirow{}{}{\textbf{p value}} \\ \cline{3-6}
                                                     &                                  & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc} &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 70.72$\pm$0.032         & 71.26$\pm$0.22          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2,c3                                     & 100                              & 86.06$\pm$0.007         & 86.83$\pm$0.67          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2                                        & 100                              & 88.19$\pm$0.89          & 86.24$\pm$0.80          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{87.35$\pm$0.01} & \textbf{88.20$\pm$0.36} & \textbf{86.67$\pm$0.05} & \textbf{87.80$\pm$0.04} & \textbf{0.359}                    \\ \hline
        c1                                           & 75                               & 86.649$\pm$0.01         & 87.34$\pm$1.09          & 86.30$\pm$0.06          & 87.10$\pm$0.08          & 0.606                             \\ \hline
        c1                                           & 50                               & 84.80$\pm$0.007         & 85.98$\pm$0.60          & 84.10$\pm$0.08          & 84.98$\pm$0.07          & 0.346                             \\ \hline
        c1                                           & 30                               & 86.40$\pm$0.006        & 87.33$\pm$0.09          & 84.05$\pm$0.09          & 84.93$\pm$0.06          &      0.0                             \\ \hline
        \end{tabular}
        }
        \caption{The $wF1[\%]$ and $|\%$ test accuracy score for $tCNN_{CAD60\_PAMAP2}$.  $tCNN_{PAMAP2}$ (table \ref{tab:wf1}) is considered as baseline. The number of convolution layers transferred and the $[\%]$ of target data used are varied. Numbers in bold shows the hyper-parameters which give the best $wF1[\%]$ score.}
        \label{tab:tf_CP}
        \end{table}
        \end{comment}
        
        
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{comment}
        
        
        \begin{table}[]
        %\vspace{-2em}
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
         ss     & \multicolumn{2}{l|}{\textbf{JHMDB}}                                  & \multicolumn{2}{l|}{\textbf{CAD60}}        & \multicolumn{2}{l|}{\textbf{Penn Action}}  \\ \hline
         \textbf{} & \textbf{\% Acc unseg}             & \textbf{\%Acc seg}               & \textbf{\% Acc unseg} & \textbf{\%Acc seg} & \textbf{\% Acc unseg} & \textbf{\%Acc seg} \\ \hline
         1         & 41.74$\pm$0.023                            & 78.72  $\pm$0.031                           & 40.06 $\pm$0.019                       & 56.375 $\pm$0.027                      & \textbf{74.63}   $\pm$0.013                     & 91.92   $\pm$0.016\\ \cline{2-8} 
    5         & 50.237 $\pm$0.025                           & 76.39$\pm$0.021                            & 43.84 $\pm$0.027                & 54.95 $\pm$0.029             & 71.66   $\pm$0.027              & 88.91  $\pm$0.029            \\ \cline{2-8} 
    12        & \textbf{79.97}  $\pm$0.032                           & 92.31     $\pm$0.027                        &  \textbf{56.16} $\pm$0.028           & 62.26 $\pm$0.022        & 71.85  $\pm$0.031               & 85.07 $\pm$0.021              \\ \cline{2-8} 
    25        & 42.384 $\pm$0.040 & 49.33 $\pm$0.048 & 56.06  $\pm$0.044                & 60.25      $\pm$0.038        & 66   $\pm$0.049                 & 76.96 $\pm$0.046             \\ \cline{2-8} 
    50        & 54.72 $\pm$0.050                            & 63 $\pm$0.051                              & 61.70 $\pm$0.055    & 49.16 $\pm$0.053 & 55.41 $\pm$0.051                 & 66.54 $\pm$0.054             \\ \cline{2-8} 
    75        & 30.82 $\pm$0.062                            & 31.33  $\pm$0.063                          & 53.7  $\pm$0.065                & 51.75 $\pm$0.069             & 48.39  $\pm$0.066               & 50.125  $\pm$0.063           \\ \hline
        \end{tabular}
        }
        \caption{$\%$ Validation accuracy computed for HAR on synthetic IMU data. Valid. Acc. is computed for segmented and unsegmented validation dataset}
        \label{tab:ss}
        %\vspace{-3em}
        \end{table}
        \end{comment}

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{comment}
        
    \subsection{Transfer Learning from Penn Action to PAMAP2 dataset}
        \label{subsection:TL_P_P}
         

        
        As seen in table \ref{tab:Pose_acc}, the $wF1\%$ is higher when tCNN is trained using Penn Action pose data than when tCNN is trained with synthetic IMU data. The explanation for the decrease in $wF1\%$ score is the same as that for CAD60 dataset.\\
        
        The $wF1\%$ and \% test accuracy for $tCNN_{Penn\_PAMAP2}$ is shown in table \ref{tab:tf_CP}. $tCNN_{Penn}$ is considered as the baseline. The wF1 score is highest when transferring only first two layers from Penn to PAMAP2. Thus, further experiments are performed by fixing the number of transferred layers to $c1,c2$ and varying the target data[\%].
        \begin{table}[H]
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{2}{*}{\textbf{Transferred layers}} & \multirow{2}{*}{\textbf{\%D\_t}} & \multicolumn{2}{l|}{\textbf{t}}            & \multicolumn{2}{l|}{\textbf{t}}           & \multirow{2}{*}{\textbf{p value}} \\ \cline{3-6}
                                                     &                                  & \textbf{\%wF1}       & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc} &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 69.84$\pm$0.037          & 71.60$\pm$2.69          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2,c3                                     & 100                              & 85.24$\pm$0.002          & 86.16$\pm$0.22          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2                                        & 100                              & 86.05$\pm$0.006          & 86.94$\pm$0.50          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{86.75$\pm$0.007} & \textbf{87.56$\pm$0.55} & \textbf{86.67$\pm$0.05} & \textbf{87.80$\pm$0.04} & \textbf{-}                        \\ \hline
        c1                                           & 75                               & 86.91$\pm$0.013          & 87.68$\pm$1.04          & 86.30$\pm$0.06          & 87.10$\pm$0.08          & 0.202                             \\ \hline
        c1                                           & 50                               & 84.82$\pm$0.006          & 85.91$\pm$0.50          & 84.10$\pm$0.08          & 84.98$\pm$0.07          &   0.05                                \\ \hline
        c1                                           & 30                               & 86.64$\pm$0.006          & 87.42$\pm$0.44          & 84.05$\pm$0.09          & 84.93$\pm$0.06          &   0.0                                \\ \hline
        \end{tabular}
        }
        \caption{The $wF1[\%]$ of tCNN pre-trained on Penn Action and fine tuned on target dataset  PAMAP2. The $wF1[\%]$  of the $tCNN_{PAMAP2}$ (table \ref{tab:wf1}) is considered as baseline. Numbers in bold shows the hyper-parameters which give the best $wF1[\%]$ score.}
        \label{tab:tf_PP}
        \end{table}
        \end{comment}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
          
        \begin{comment}
    \subsection{Summarizing transfer learning $tCNN_{D_{s}\_PAMAP2}$}
        Fig \ref{fig:TL_PAMAP2} and Fig \ref{fig:TL_PAMAP22} summarizes the results for Transfer Learning from all source datasets to PAMAP2. Among all the source datasets, a significant increase in $wF1[\%]$ is obtained only for $tCNN_{JHMDB\_PAMAP2}$.
       
        \begin{figure}[]
        
        \begin{center}
        \vspace{-1.8em}
        Varying the number of transferred layers
        \begin{tikzpicture}[scale=0.7]
            \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
                \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
                \begin{axis}
                    [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.23cm) rectangle (1cm,0.3cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.6, 0.9, 3.2, 5.2},
                    xticklabels={c1,(c1,c2),(c1,c2,c3),(c1,c2,c3,c4)},
                    xticklabel style={rotate=0},
        	        xlabel={Transferred convolutional layers }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.5)}, anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(.020,0.5)}},
                    ymin=68, ymax=91,
                    ytick={68,72,76,80,84,88,91},
                    nodes near coords,]
                    
                    \legend{PAMAP(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
                     \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.67)}; %A1        
                   
                    
                    \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,88.97)}; %a1
                     \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,88.45)}; %a1
                    
                    \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.61)};
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.85)};
                    
                    \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.75)};
                    
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.56)};
                    
                    %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
                    %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.67)}; %Random Forest        
                    %\addlegendentry{unseen}
            
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,88.57) }; %a2   
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,88.25)};
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,85.38) }; %a2 
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.17)};
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.05) }; %a2   
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.87)};
                    
                   
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.67)}; %SVM linear       
                    %\addlegendentry{a3}
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,87.57)}; %a3
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,88.45)};
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.06)}; %SVM linear       
                    %\addlegendentry{a3}
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.40)};
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,85.24)}; %a3            
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,88.68)};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.67) }; %Softmax 
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,87.95) }; %Softmax 
                    %\addlegendentry{a4}
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,90.98) };
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,70.72) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,69.7) };
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,69.84) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,87.99)};
                      
                    \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
                \end{axis}
        \end{tikzpicture}
        
        \end{center}
        %\vspace{-1.7em}
        \caption{The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D{S}\_PAMAP2}$. The tCNN is trained from scratch on PAMAP2 or pretrained on JHMDB, CAD60, Penn Action or pose dataset. The bars in grey colour correspond to the transfer learning performance when using the pose data as source.  $100\%$ of LARa OB dataset is used for fine tuning the pretrained model}
        \vspace{-2.5em}
        \label{fig:TL_PAMAP2}
        \end{figure}
       
        
        \begin{figure}
        \begin{center}
        \vspace{-2em}
        Varying \% PAMAP2 data
        \begin{tikzpicture}[scale=0.7]
            \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
                \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
                \begin{axis}
                    [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.5, 0.9, 2.6, 4.2},
                    xticklabels={PAMAP2 [30\%],PAMAP2 [50\%],PAMAP2 [75\%],PAMAP2 [100\%]},
                    xticklabel style={rotate=0},
        	    xlabel={\% PAMAP2 data used for tuning }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.55)}, anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(0.02,0.5)}},
                    ymin=80, ymax=91,
                    ytick={80,82,84,86,88,91},
                    nodes near coords,]
                    
                    \legend{PAMAP(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
                    \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,84.05)}; %A1        
                    %\addlegendentry{seen}
                    
                    \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,85.55)}; %a1
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,90.9)};
                    
                    \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,86.40)};
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,84.87)};
                    %\node[node1, above] at ($(axis cs:8.2,0)$) {\textbf{a1}};  
                    
                    \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,86.64)};
                   \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,82.53)};
                    
                    %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.1)}; %Random Forest        
                    %\addlegendentry{unseen}
            
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.1) }; %a2   
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,85.57) }; %a2   
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.80) }; %a2   
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.38) }; %a2  
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.82) }; %a2   
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.26) }; %a2  
                    
                    %\node[node1, above] at ($(axis cs:10.9,69)$) {\textbf{99.2\%}};
                    
            
            
                    
                    %\node[node1, above] at ($(axis cs:-4.2,70)$) {\textbf{64.3\%}};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.2)}; %SVM linear       
                    %\addlegendentry{a3}
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.15)}; %a3
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,87.95)}; %a3
                    
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.64)}; %CAD60 75%       
                    %\addlegendentry{a3}
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.33)}; %a3
                    
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.91)}; %Penn 75%            
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,85.80)}; %a3
                    
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.65) }; %Softmax 
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,88.97) }; %Softmax 
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,90.98) };
                    %\addlegendentry{a4}
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.61) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.85) };
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.75) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,88.68) };
                    
                    \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
                \end{axis}
        \end{tikzpicture}
        \vspace{-2.7em}
        \end{center}
        \caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_PAMAP2}$. Percent of PAMAP2 data used for fine tuning is varied.}
        \vspace{-2.5em}
        \label{fig:TL_PAMAP22}
        \end{figure}
    \end{comment}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
     Source to PAMAP2
 
 \begin{table}[]
    %\vspace{-1.5em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\textbf{$\%D_t$}}& \multicolumn{2}{l|}{\textbf{$tCNN_{CAD60_{sy}\_PAMAP2}$}}             & \multicolumn{2}{l|}{\textbf{$tCNN_{CAD60_p\_PAMAP2}$}}    & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}(Baseline)} \\ \cline{3-8} 
         Layers        &                                  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}    & \textbf{\%Test acc} & \textbf{\%wF1}    & \textbf{\%Test acc}   \\ \hline
        \textbf{$c_1$}                              & 100                              & 87.35+0.004          & 88.19+0.36          & 86.85+0.001       & 87.57+0.005           & 86.67+0.05          & 87.80+0.04          \\ \hline
        \textbf{$c_{1,2}$}                           & 100                              & 85.38+0.009          & 86.24+0.80          & 86.17+0.005       & 87.09+0.004           & \textbf{86.67+0.05} & \textbf{87.80+0.04} \\ \hline
        \textbf{$c_{1,2,3}$}                        & 100                              & 86.06+0.007          & 86.83+0.67          & 86.40+0.001       & 87.29+0.062           & 86.67+0.05          & 87.80+0.04          \\ \hline
        \textbf{$c_{1,2,3,4}$}                     & 100                              & 70.72+0.032          & 71.26+0.27          & 69.700.038        & 71.76+0.81            & \textbf{86.67+0.05} & \textbf{87.80+0.04} \\ 
        \hline
        \hline
        \textbf{c1}                              & 75                               & 86.31+0.007          & 87.19+0.75          & 86.33+0.003       & 87.20+0.27            & 86.30+0.06          & 87.10+0.08          \\ \hline
        \textbf{c1}                              & 50                               & \textbf{85.74+0.004} & \textbf{86.69+0.40} & 84.38+0.005       & 85.58+0.429           & 84.10+0.08          & 84.98+0.07          \\ \hline
        \textbf{c1}                              & 30                               & \textbf{85.77+0.005} & \textbf{86.70+0.58} & 84.87+0.002       & 85.86+0.24            & 84.05+0.09          & 84.93+0.06          \\ \hline
    
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{CAD60\_PAMAP2}$.}
    \label{tab:TL_C_PAMAP2}
    %\vspace{-2em}
\end{table}
 
\begin{table}[]
    %\vspace{-3em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf.} } & \multirow{}{}{\textbf{$\%D_t$}}& \multicolumn{2}{l|}{\textbf{$tCNN_{Penn_{sy}\_PAMAP2}$}}             & \multicolumn{2}{l|}{\textbf{$tCNN_{Penn_p\_PAMAP2}$}}    & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}(Baseline)} \\ \cline{3-8} 
        Layers & & \textbf{\%wF1}                      & \textbf{\%Test acc}                & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        {c1}                               & 100                               & 86.80$\pm$0.004                         & 87.63$\pm$0.40                         & 87.43$\pm$0.27          & 86.56$\pm$0.002         & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1,c2}                            & 100                               &86.05$\pm$0.006 & 86.94$\pm$0.49 & 87.77$\pm$0.56          & 86.87$\pm$0.005         & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1,c2,c3}                         & 100                               & 85.24$\pm$0.002                         & 86.158$\pm$0.22                        & \textbf{89.13$\pm$0.85} & \textbf{88.68$\pm$0.02} & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1,c2,c3,c4}                      & 100                               & 69.84$\pm$0.037                         & 71.60$\pm$0.27                         & 88.92$\pm$0.27          & 87.99$\pm$0.04          & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1}                               & 75                                & 85.85$\pm$0.004                         & 86.81$\pm$0.35                         & 85.72$\pm$0.02          & 85.80$\pm$0.002         & 86.30$\pm$0.06      & 87.10$\pm$0.08           \\ \hline
        {c1}                               & 50                                & 84.58$\pm$0.006                & 85.61$\pm$0.49                & 85.26$\pm$0.09          & 84.26$\pm$0.02          & 84.10$\pm$0.08      & 84.98$\pm$0.07           \\ \hline
        {c1}                               & 30                                & \textbf{86.64$\pm$0.0058}               & \textbf{87.421$\pm$0.44}               & 83.90$\pm$0.56          & 82.53$\pm$0.02          & 84.05$\pm$0.09      & 84.93$\pm$0.06           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{Penn\_PAMAP2}$.}
    \label{tab:TL_P_PAMAP2}
    %\vspace{-3em}
\end{table}
 
 
 
\begin{table}[]
    % \vspace{-2em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf.} } & \multirow{}{}{\bm{$\%D_t$}} &\multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_{sy}\_PAMAP2}$}}             & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_p\_PAMAP2}$}}    & \multicolumn{2}{l|}{\bm{$tCNN_{PAMAP2}$(Baseline)}} \\ \cline{3-8} 
        
        Layers & & \textbf{\%wF1}                              & \textbf{\%Test acc}                         & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        {c1}                               & 100                               & \textbf{88.97+0.07}                         & \textbf{89.53+0.03}                         & \textbf{88.45+0.001} & \textbf{89.23+0.02}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1,c2}                            & 100                               & \textbf{88.57+0.05} & \textbf{89.32+0.07} & \textbf{88.25+0.006} & \textbf{89.10+0.01}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1,c2,c3}                         & 100                               & 87.57+0.06                                  & 88.51+0.07                                  & \textbf{88.55+0.01}  & \textbf{89.26+0.03}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1,c2,c3,c4}                      & 100                               & \textbf{87.95+0.06}                         & \textbf{88.98+0.05}                         & \textbf{90.98+0.03}  & \textbf{92.01+0.07}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1}                               & 75                                & 86.15+0.05                                  & 87.20+0.09                                  & \textbf{87.95+0.04}  & \textbf{89.10+0.03}  & 86.30+0.06      & 87.10+0.08           \\ \hline
        {c1}                               & 50                                & \textbf{86.1+0.01}                          & \textbf{86.93+0.05}                         & \textbf{85.57+0.002} & \textbf{86.60+0.02}  & 84.10+0.08      & 84.98+0.07           \\ \hline
        {c1}                               & 30                                & \textbf{85.55+0.04}                         & \textbf{86.13+0.05}                         & \textbf{90.99+0.01}   & \textbf{91.87+0.008} & 84.05+0.09      & 84.93+0.06           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics for $tCNN_{JHMDB\_PAMAP2}$. The layers are fixed at c1 for $tCNN_{JHMDB_{sy}\_PAMAP2}$ and c1,c2,c3,c4 for $tCNN_{JHMDB_p\_PAMAP2}$.}
    \label{tab:TL_J_PAMAP2}
    %\vspace{-3em}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SOurce dataset to LARAOB

\begin{table}[]
    %\vspace{-1em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_{sy}\_LARaIMU}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_p\_LARaIMU}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{LARaIMU}$(Baseline)}}      \\ \cline{3-8} 
         \textbf{Layers} &                                  & \textbf{\%wF1}       & \textbf{\%Test acc} & \textbf{\%wF1}         & \textbf{\%Test acc}   & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        c1                                                                                  & 100                              & 66.56$\pm$0.009          & 68.81$\pm$0.05          & 66.15$\pm$0.0034           & 69.59$\pm$0.389           & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1,c2                                                                               & 100                              & 66.27$\pm$0.005          & 68.50$\pm$0.04          & 65.86$\pm$0.0016           & 69.61$\pm$0.34          & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1,c2,c3                                                                            & 100                              & 66.32$\pm$0.06           & 68.52$\pm$0.06          & 65.36$\pm$0.08             & 69.06$\pm$0.08            & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1,c2,c3,c4                                                                         & 100                              & 66.76$\pm$0.01           & 68.80$\pm$0.008         & 53.97$\pm$0.0056           & 63.20$\pm$0.48            & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1                                                                                  & 75                               & \textbf{66.15$\pm$0.007} & \textbf{68.74$\pm$0.03} & \textbf{65.805$\pm$0.0075} & \textbf{69.61$\pm$0.376} & 65.68$\pm$0.008     & 66.91$\pm$0.03           \\ \hline
        c1                                                                                  & 50                               & \textbf{66.65$\pm$0.08}  & \textbf{68.05$\pm$0.03} & 62.16$\pm$0.023            & 67.33$\pm$0.61            & 65.66$\pm$0.02      & 66.88$\pm$0.06           \\ \hline
        c1                                                                                  & 30                               & 65.81$\pm$0.04           & 67.65$\pm$0.01          & 57.75$\pm$0.09             & 65.11$\pm$0.07            & 65.81$\pm$0.04      & 67.05$\pm$0.02           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{JHMDB\_LARaIMU}$.}
    \label{tab:TL_J_Lara}
    %\vspace{-2em}
\end{table}



\begin{table}[]
    %\vspace{-2em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }}& \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_{sy}\_LARaIMU}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_p\_LARaIMU}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{LARaIMU}$(Baseline)}}      \\ \cline{3-8} 
        \textbf{Layers }            &                                  & \textbf{\%wF1}      & \textbf{\%Test acc}  & \textbf{\%wF1}      & \textbf{\%Test acc}  & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        c1                                       & 100                              & 69.67+0.59          & 66.33+0.01           & 69.02+0.26          & 65.03+0.005          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2                                    & 100                              & 66.76+0.77          & 61.25+0.017          & 65.12+0.21          & 62.35+0.008          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3                                 & 100                              & 65.58+0.49          & 59.01+0003           & 60.51+0.08          & 60.24+0.006          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3,c4                              & 100                              & 52.78+0.008         & 36.48+0.001          & 63.84+0.037         & 56.19+0.001          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1                                       & 75                               & 69.30+0.30 & 65.80+0.006 & 67.07+0.81 & 61.81+0.003 & 65.68+0.008     & 66.91+0.03           \\ \hline
        c1                                       & 50                               & 66.57+0.64 & 60.99+0.014 & 66.00+0.07          & 60.20+.002           & 65.66+0.02      & 66.88+0.06           \\ \hline
        c1                                       & 30                               & 64.93+0.76          & 58.54+0.019          & 64.38+0.50          & 56.98+0.011          & 65.81+0.04      & 67.05+0.02           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{CAD60\_LARaIMU}$.}
    \label{tab:TL_C_Lara}
    ´%\vspace{-3em}
\end{table}       
        

\begin{table}[]
    %\vspace{-2em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}}& \multicolumn{2}{l|}{\boldsymbol { $tCNN_{Penn_{sy}\_LARaIMU}$}}             & \multicolumn{2}{l|}{\boldsymbol {$tCNN_{Penn_p\_LARaIMU}$}}    & \multicolumn{2}{l|}{\boldsymbol {$tCNN_{LARaIMU}$(Baseline)}} \\ \cline{3-8} 
                                      \textbf{Layers}       &                                  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}        & \textbf{\%Test acc}  & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        c1                                       & 100                              & 67.24+0.003          & 69.54+0.32           & 66.26+0.001           & 69.80+0.14           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2                                    & 100                              & 65.85+0.01           & 69.27+0.68           & 65.90+0.004           & 69.40+0.01           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3                                 & 100                              & 61.38+0.03           & 66.68+0.14           & 65.75+0.059           & 69.43+0.32           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3,c4                              & 100                              & 36.53+0.003          & 52.80+0.01           & 64.627+0.003          & 68.77+0.15           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1                                       & 75                               & \textbf{66.37+0.004} & \textbf{69.73+0.004} & \textbf{66.476+0.008} & \textbf{69.97+0.42}  & 65.68+0.008     & 66.91+0.03           \\ \hline
        c1                                       & 50                               & \textbf{65.66+0.006} & \textbf{69.43+0.37}  & \textbf{66.68+0.010}  & \textbf{70.365+0.66} & 65.66+0.02      & 66.88+0.06           \\ \hline
        c1                                       & 30                               & 62.37+0.20           & 67.267+0.13          & 61.07+0.022           & 66.69+0.74           & 65.81+0.04      & 67.05+0.02           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{Penn\_LARaIMU}$.}
    \label{tab:TL_P_Lara}
    %\vspace{-3em}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SOurce to Loc

\begin{table}[]
    %\vspace{-0.5em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf.}} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_{sy}\_Loc}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_p\_Loc}$}}    & \multicolumn{2}{l|}{\bm{$tCNN_{Loc}$(Baseline)}}      \\ \cline{3-8} 
                                           \textbf{Layers}        &                                  & \textbf{\%wF1} & \textbf{\%Test acc} & \textbf{\%wF1}       & \textbf{\%Test acc}   & \textbf{\%wF1}       & \textbf{\%Test acc}  \\ \hline
        c1,c2,c3,c4                                  & 100                              & 74.68$\pm$0.007    & 74.95$\pm$0.005         & 79.12$\pm$0.002          & 79.51$\pm$0.002           & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2,c3                                     & 100                              & 84.99$\pm$0.01     & 85.22$\pm$0.01          & 81.24$\pm$0.004          & 82.35$\pm$0.007           & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2                                        & 100                              & 85.68$\pm$0.008    & 85.85$\pm$0.007         & 86.44$\pm$0.006 & 86.60$\pm$0.006  & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & 85.32$\pm$0.01     & 86.49$\pm$0.009         & 86.10$\pm$0.02  & 86.30$\pm$0.02   & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        c1                                           & 75                               & 85.60$\pm$0.006    & 85.82$\pm$0.009         & 85.86$\pm$0.003 & 86.17$\pm$0.003  & 85.87$\pm$0.002          & 86.17$\pm$0.002          \\ \hline
        c1                                           & 50                               & \textbf{86.03$\pm$0.01}     & \textbf{86.27$\pm$0.001}         & 83.77$\pm$0.001          & 84.12$\pm$0.001           & 84.44$\pm$0.008 & 84.61$\pm$0.007 \\ \hline
        c1                                           & 30                               & 83.04$\pm$0.007    & 83.40$\pm$0.009         & \textbf{83.97$\pm$0.003} & \textbf{84.35$\pm$0.0031} & 83.11$\pm$0.002          & 83.30$\pm$0.002          \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{JHMDB\_Loc}$.}
    \label{tab:TL_J_L}
    %\vspace{-1em}
\end{table}


\begin{table}[]
    %\vspace{-1em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_{sy}\_Loc}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_p\_Loc}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{Loc}$(Baseline)}}      \\ \cline{3-8} 
        \textbf{ Layers} &                                  & \textbf{\%wF1} & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}       & \textbf{\%Test acc}  \\ \hline
        c1,c2,c3,c4                                                                         & 100                              & 74.98+0.007    & 73.54+0.005         & 80.60+0.15          & 80.00+0.02          & \textbf{85.38+0.009} & \textbf{85.65+0.009} \\ \hline
        c1,c2,c3                                                                            & 100                              & 78.71+0.02     & 79.68+0.016         & 84.7+0.034          & 84.85+0.53          & 85.38+0.009 & 85.65+0.009 \\ \hline
        c1,c2                                                                               & 100                              & 82.52+0.009    & 82.93+0.008         & 85.61+0.07 & 85.83+0.62 & 85.38+0.009          & 85.65+0.009          \\ \hline
        \textbf{c1}                                                                         & \textbf{100}                     & 83.92+0.007    & 84.20+0.007         & \textbf{87.27+0.02} & \textbf{87.46+0.02} & 85.38+0.009          & 85.65+0.009          \\ \hline
        c1                                                                                  & 75                               & 85.97+0.001    & 86.23+0.001         & 85.13+0.06 & 85.33+0.05 & 85.87+0.002         & 86.17+0.003         \\ \hline
        c1                                                                                  & 50                               & \textbf{85.79+0.004}    & \textbf{86.09+0.003}         & \textbf{85.88+0.03}          & \textbf{86.14+0.22}          & 84.44+0.008 & 84.61+0.007 \\ \hline
        c1                                                                                  & 30                               & 83.04+0.01     & 83.40+0.009         & 83.08+0.01 & 83.46+0.54 & 83.11+0.002          & 83.30+0.002          \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{CAD60\_Loc}$.}
    \label{tab:TL_C_L}
    %\vspace{-1em}
\end{table}


\begin{table}[]
    %\vspace{-1.5em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{Penn_{sy}\_Loc}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{Penn_p\_Loc}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{Loc}$(Baseline)}}      \\ \cline{3-8} 
                                                                                            \textbf{Layers}       &                                  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}       & \textbf{\%Test acc}  \\ \hline
        c1,c2,c3,c4                                                                         & 100                              & 68.95$\pm$0.04           & 70.46$\pm$0.20           & 64.95$\pm$0.07           & 66.85$\pm$0.07           & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2,c3                                                                            & 100                              & 71.52$\pm$0.40           & 73.41$\pm$0.06           & 82.78$\pm$0.001          & 83.16$\pm$0.001          & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2                                                                               & 100                              & 85.43$\pm$0.007          & 85.73$\pm$0.006          & 85.61$\pm$0.07           & 85.83$\pm$0.06           & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        \textbf{c1}                                                                         & \textbf{100}                     & 86.17$\pm$0.008          & 86.41$\pm$0.008          & \textbf{86.73$\pm$0.005} & \textbf{86.84$\pm$0.004} & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        c1                                                                                  & 75                               & 85.41$\pm$0.009          & 85.61$\pm$0.009          & 86.39$\pm$0.02           & 86.57$\pm$0.03           & 85.87$\pm$0.002          & 86.16$\pm$0.009          \\ \hline
        c1                                                                                  & 50                               & \textbf{85.60$\pm$0.004} & \textbf{86.09$\pm$0.003} & 85.11$\pm$0.08           & 85.42$\pm$0.07           & 84.44$\pm$0.008          & 84.61$\pm$0.007          \\ \hline
        c1                                                                                  & 30                               & 83.04$\pm$0.005          & 83.50$\pm$0.004          & 83.50$\pm$0.01           & 83.88$\pm$0.02           & 83.11$\pm$0.002          & 83.30$\pm$0.002          \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{Penn\_Loc}$.}
    \label{tab:TL_P_L}
    %\vspace{-3em}
\end{table}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[]
\vspace{-2em}
\begin{center}
Varying number of transferred layers
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
             [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.23cm) rectangle (1cm,0.3cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.6, 0.9, 3.2, 5.2},
                    xticklabels={c1,(c1,c2),(c1,c2,c3),(c1,c2,c3,c4)},
                    xticklabel style={rotate=0},
        	        xlabel={Transferred convolutional layers }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.5)},
                    %legend style={column sep=0.01cm},
                    anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(.020,0.5)}},
                    ymin=64, ymax=88,
                    ytick={70,74,78,82,88},
                    nodes near coords,every node near coord/.append style={anchor=west,rotate=60}]
                   
                    
            \legend{Opp-Loc(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
         
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,85.65)}; %A1        
            %\addlegendentry{seen}
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.32)}; %a1
            \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.1)};
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.79)};
           \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,87.24)}; 
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.41)};
             \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.70)};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.65)}; %Random Forest        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.68) }; %a2   
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,86.20) };
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.88) }; %a2
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.61) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.92) }; %a2 
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,86.22) };
            
              
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.65)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,81.24)}; %a3
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,81.41)}; %a3
            
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,81.11)};       
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,84.7)}; %a3
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,72.68)}; %a3            
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,82.78)}; %a3
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,85.65) }; %Softmax 
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,76.84) }; %Softmax 
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,79.12) };
           
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,77.06) }; %a4
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,80) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,70.56) }; %a4
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,64.95) };
            
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
         
\end{tikzpicture}
\end{center}
\vspace{-2em}
\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_Loc}$. $tCNN_{Loc}$ is used as the baseline. $100\%$ of Opp-Loc dataset is used for fine tuning.}
\label{fig:TL_loc}
\vspace{-2em}
\end{figure}
 
\begin{figure}[]
\vspace{-1em}
\begin{center}
Varying \% Opp-Loc data
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
            [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.5, 0.9, 2.6, 4.2},
                    xticklabels={Loc [30\%],Loc [50\%],Loc [75\%],Loc [100\%]},
                    xticklabel style={rotate=0},
        	    xlabel={\% PAMAP2 data used for tuning }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.55)}, anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(0.02,0.5)}},
                     ymin=80, ymax=90,
                     ytick={80,82,84,86,88,90},
                     nodes near coords,every node near coord/.append style={anchor=west,rotate=60}]
                   
                    
             \legend{LARaOB(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
           
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.11)}; %A1        
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.04)}; %a1
            \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.97)};
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.04)};
            \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.08)};  
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.39)};
     \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.50)};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,84.44)};        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,86.03) }; %a2   
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,83.77) };
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.8) }; %CAD  
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.88) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.60) }; %a2   
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.11) };
    
    
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.87)}; %SVM linear       
          
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.60)}; 
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.86)};
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.42)}; %CAD60 75%       
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.13)};
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.41)}; %Penn 75%            
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,86.39)}; %Penn 75% 
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,85.65) };  
            
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.32) }; %Softmax 
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.10) };
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.79) }; %a4
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,87.27) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.41) }; %a4
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.73) };
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
\end{tikzpicture}
\end{center}
\vspace{-2em}
\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_s\_Loc}$. Percent of Opp-loc data used for fine tuning is varied.}
\label{fig:TL_loc2}
%\vspace{-2em}
\end{figure}
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SOurce to LARaMM


\begin{figure}[H]
\begin{center}
Varying number of transferred layers
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
            [name=main plot,ybar,
            every axis legend/.append style={nodes={right}},
            legend image code/.code={%
                \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
            width=150mm, height=95mm,
            axis x line=bottom, 
            axis y line=left,
            ymajorgrids,
            xtick={-0.5, 0.9, 2.6, 4.2},
            xticklabels={c1,(c1,c2),(c1,c2,c3),(c1,c2,c3,c4)},
            xticklabel style={rotate=0},
	        xlabel={No. of transferred layers }, 
            bar width=12.5,  
            xmin=-1.6,xmax=6,
            legend style={at={(0.5,-0.25)}, anchor=south,legend columns=-1}, 
            ylabel={weighted F1 [\%]}, 
            ylabel style={align=center, at={(-0.02,0.5)}},
            ymin=30, ymax=65,
            ytick={30,35,40,45,50,55,57,59,61,63,65},
            nodes near coords,]
            
            \legend{LaraMM(scratch), JHMDB, CAD60, Penn}
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,63.06)}; %A1        
            %\addlegendentry{seen}
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,58.55)}; %a1
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,55.85)};
            %\node[node1, above] at ($(axis cs:8.2,0)$) {\textbf{a1}};  
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,57.66)};
    
            
            %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,63.06)}; %Random Forest        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,55.51) }; %a2   
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,56.59) }; %a2   
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,57.32) }; %a2   
            
            %\node[node1, above] at ($(axis cs:10.9,69)$) {\textbf{99.2\%}};
            
    
    
            
            %\node[node1, above] at ($(axis cs:-4.2,70)$) {\textbf{64.3\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,63.06)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,52.90)}; %a3
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,57.95)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,59.09)}; %a3            
    
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,63.06) }; %Softmax 
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,37.07) }; %Softmax 
            %\addlegendentry{a4}
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,53.34) }; %a4
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,51.44) }; %a4
            
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
         
\end{tikzpicture}
\end{center}
\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_LaraMM}$. $tCNN_{LARaMM}$ is used as the baseline. $100\%$ of LaraMM dataset is used for fine tuning.}
\label{fig:TL_LaraMM}
\end{figure}

Fig \ref{fig:TL_LaraMM2} summarises the results for the case when the number of transferred layers is fixed at c1. The percent of LARaMM data used for fine tuning is varied. It is observed that transfer learning does not improve the performance even when LARaMM dataset is scarce. The difference between LARaOB and LARaMM is the position and number of IMUs used. Therefore, in addition to the environment in which an activity is performed the location of IMUs also affects transfer learning performance. 
\begin{figure}[H]
\begin{center}
Varying \% LARa MM data
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
            [name=main plot,ybar,
            every axis legend/.append style={nodes={right}},
            legend image code/.code={%
                \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
            width=150mm, height=95mm,
            axis x line=bottom, 
            axis y line=left,
            ymajorgrids,
            xtick={-0.5, 0.9, 2.6, 4.2},
            xticklabels={LARaMM [30\%],LARaMM [50\%],LARaMM [75\%],LARaMM [100\%]},
            xticklabel style={rotate=0},
	        xlabel={\% LARa MM data used for tuning }, 
            bar width=12.5,  
            xmin=-1.6,xmax=6,
            legend style={at={(0.5,-0.25)}, anchor=south,legend columns=-1}, 
            ylabel={weighted F1 [\%]}, 
            ylabel style={align=center, at={(-0.02,0.5)}},
            ymin=49, ymax=64,
            ytick={49,50,51,52,53,54,55,56,57,58,59,60,61,62,63,64},
            nodes near coords,]
            
            \legend{LaraMM(scratch), JHMDB, CAD60, Penn}
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,52.88)}; %A1        
            %\addlegendentry{seen}
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,50.20)}; %a1
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,51.91)};
            %\node[node1, above] at ($(axis cs:8.2,0)$) {\textbf{a1}};  
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,52.98)};
    
            
            %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,55.55)};        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,54.7) }; %a2   
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,53.50) }; %a2   
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,53.29) }; %a2   
            
            %\node[node1, above] at ($(axis cs:10.9,69)$) {\textbf{99.2\%}};
            
    
    
            
            %\node[node1, above] at ($(axis cs:-4.2,70)$) {\textbf{64.3\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,59.05)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,55.02)}; %a3
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,57.43)}; %CAD60 75%       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,56.13)}; %Penn 75%            
    
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,63.06) }; %Softmax 
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,58.55) }; %Softmax 
            %\addlegendentry{a4}
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,55.85) }; %a4
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,57.66) }; %a4
            
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
\end{tikzpicture}
\end{center}

\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_LaraMM}$. Percent of LaraMM data used for fine tuning is varied.}
\label{fig:TL_LaraMM2}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
 
 \begin{table}[]
        \centering
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\textbf{$\%D_{t}$}} & \multicolumn{2}{l|}{\textbf{$tCNN_{JHMDB\_PAMAP2}$}}           & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$(Baseline)}}             & \multirow{}{}{\textbf{p value}} \\ \cline{3-6}
                                                     layers&                                  & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc}   &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 87.95$\pm$0.06          & 88.98$\pm$0.05          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & 0.005912                          \\ \hline
        c1,c2,c3                                     & 100                              & 87.70$\pm$0.06          & 88.51$\pm$0.07          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & 0.100044                          \\ \hline
        c1,c2                                        & 100                              & 88.57$\pm$0.05          & 89.32$\pm$0.06          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & 0.00034                           \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{88.97$\pm$0.08} & \textbf{89.53$\pm$0.07} & \textbf{86.67$\pm$0.05} & \textbf{87.80$\pm$0.04} & \textbf{0.00002}                  \\ \hline
        c1                                           & 75                               & 86.15$\pm$0.05          & 87.20$\pm$0.06          & 86.30$\pm$0.06          & 87.10$\pm$0.08            &     0.843                              \\ \hline
        c1                                           & 50                               & 86.10$\pm$0.06          & 86.93$\pm$0.08          & 84.10$\pm$0.08          & 84.98$\pm$0.07            &        0.00004                           \\ \hline
        c1                                           & 30                               & 85.55$\pm$0.04          & 86.13$\pm$0.05          & 84.05$\pm$0.09          & 84.93$\pm$0.06            &   0.0107                                \\ \hline
        \end{tabular}
        }
        \caption{The table shows $wF1[\%]$ for $tCNN_{JHMDB\_pamap2}$. The $wF1[\%]$ and $\%$test accuracy of $tCNN_{PAMAP2}$ is used as the baseline. The number of convolution layers transferred are varied.}
        \label{tab:tf_JP}
        \end{table}
        \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/chapters/05_conclusions.tex <==

\section{Conclusion}
\label{sec:conclusion}


This paper proposes to use pose annotations from video datasets as an input stream for solving multichannel-time series human activity recognition (HAR) using transfer learning. Four different datasets comprising ground truth pose estimation from videos are deployed as the $D_s$. The sequences of pixel coordinates of human joints are considered as simplifications of pose estimations. A temporal CNN that processes inertial measurements per channel with late fusion is trained, considering the pixel coordinates as individual channels. The learned temporal convolutional layers are used to initialize architectures on three benchmark datasets for HAR. Experiments regarding the number of transferred layers, the two versions of the $D_s$, and a proportion of the $D_t$ are carried out. In general, when transferring only the first convolutional layer, the performance showed a positive influence on the task, independently of the data source. Transfer learning helps when a small proportion of the training target set is available. Besides, source and target datasets with shared activities showed some improvements. These findings suggest that simple local temporal relations are rather generic, thus transferable. The more complex and task-related filters are not transferable. Experimentation using the networks, such as \textit{RNNs} or Fully-convolutional \textit{CNN}, could further improve the results. 

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/chapters/response_reviews.tex <==
\section*{Answer to Reviewers}

    We would like to thank the reviewers for their helpful comments and suggestions on the manuscript, as these led us to improve our work. Detailed responses to reviewers are given below.
    
    \subsection*{Reviewer $2353$}
    
        \begin{itemize}
            \item \textbf{Why window size of 1 second is used? What would be the scenario if authors would use 3 seconds window with 50\% overlap? Or with 0\% overlap?}

            ANSWER: \textit{We have experimented with varying step size and decided the window size based on a publication. 
            %We have added the text in section V.A.
            The duration of most activities in $D_s$ is between $0.75$ to $2$ sec. Tab.~\ref{tab:window_size} shows that for CAD60, the recognition accuracy was highest when $W=5$. However, the $wF1$ score for transfer learning from CAD60 to $D_t$ was similar for when $W=1$ and $W=5$. The results for $W=5$ are available in the repository, https://github.com/shrutarv/Create-Synthetic-IMU-data. Therefore, for generality and based on results from \cite{reining2019human}, $W=1$ is chosen for training all the $D_s$. Moreover, conclusions from \cite{banos2014window} further support the decision of choosing $W=1$. We performed experiments with step sizes $1,3,5,10,12,15,$ and $20$ and chose the one that gave the best $wF1$ score. Table \ref{tab:step_size} shows the $wF1[\%]$ for HAR on the three $D_s$: $JHMDB_{synth}$, $CAD60_{synth}$ and $Penn_{synth}$. The $W$ is fixed at $1$ and $s$ is varied.  This work aims to show that transfer learning can alleviate the scarcity of data; therefore, extensive experiments with different $W$ and $s$ are not performed. The performance on these datasets are interesting comparing with the results including video-based HAR using poses as tree-like tensors. Due to limited amount of space, these results are not included into the main document.} %window size of $0.5sec$, $1$sec, and $2$sec.
            \input{Tables/window_size}
            \input{Tables/step_size}
                
            \item \textbf{Training, validation and the testing split were across the whole dataset (for instance Opportunity dataset) or across the users? How can we generalize it?}
            
            ANSWER:\textit{We have followed the training, validation, and testing splits according to the original publications of the datasets, with fix set of users/subjects per set, i.e., the sets do not contain overlapping recordings of the same user/subject. We have included the splits in the text in section IV 2nd paragraph and under every target dataset.}
            
            \item \textbf{Why only batch gradient descent with RMS-Prop was introduced?}\\
            
            ANSWER: \textit{We have chosen this SGD with RMS-Prop based on SOA and previous exploration of different SGD approaches. Besides, we have concentrated on the primary goal of using transfer learning for solving the problem of scarcity of data as number of pages is limited. Added the text in section III.A}
            
            \item \textbf{Three different learning rates were introduced, which one showed significant performance?}\\
            
            ANSWER: \textit{We had experimented using the three learning rates and chosen the one giving the nest classification performance on the validation set---we did not include the results for each of the learning rates as number of pages is limited---, however, the repository allows for evaluating easily different training hyperparameters, see https://github.com/shrutarv/Create-Synthetic-IMU-data. We have included some explanation in text, Section III.A}
        \end{itemize}
        
        Though the results are mixed on different datasets. The proportion of Target datasets used really influenced the results, which opens new ways to explore HAR via transfer learning.
    
    \subsection*{Reviewer $2371$}
    
        \begin{itemize}
            \item \textbf{More detail regarding the synthetic data generation, and the role that the synthetic data and "raw" data from the video are needed. The way this is presented in Section III is misleading as the synthetic data is introduced as though it is being used to provide additional samples, whereas it is simulating the on-body sensors. This discussion should be clarified with detail added to allow someone else to reproduce the system}
            
            Answer: \textit{We use the second derivative of a smooth piecewise spline interpolation of degree five on a small-time interval from sequences of human joint-poses for simulating on-body devices attached to the poses, a sort of synthetic data. In line with  \cite{gurjar2018_LDRWSUWS,Moya_Rueda2020}, synthetic data could also be beneficial for transfer learning, improving performance on a limited-sized dataset. We have added the explanation in Section III. For reproducing the preprocessing, the authors make available the repository, https://github.com/shrutarv/Create-Synthetic-IMU-data.}
            
            \item \textbf{Details are on the IMU-tCNN, and how features are combined from multiple branches prior to classification, are missing. Is the IMU-tCNN the same as that shown in Fig 1? Five braches are trained (one per limb), but it's unclear what skeleton point these correspond to in the video data. It's also unclear how the branches are adapted when the target dataset does not have five IMUs (Pamap2 has devices on the ankle, hand and chest, are the other two branches just removed?). More details are needed here.}
            
            ANSWER: \textit{For all the datasets, firstly, the given pose annotations are visualised. Subsequently, the joints are mapped to the branches of \textit{IMU-tCNN}. The mapping is available in the repository, https://github.com/shrutarv/Create-Synthetic-IMU-data. However, for Penn Action, there is no clarity of the joints, as they did not form a skeleton-like figure when visualising and their joint names were not semantically clear; therefore, mapping is not possible. We have added some clarification of the mapping human limbs-branches of the architecture in Section III.A and also for all datasets in Section IV.}
            
            \item \textbf{Window size is fixed at 1s, yet datasets are captured at different sampling rates. There does seem to be resampling performed from the results tables, however any details of this (I assume that simple interpolation is used?) are missing.}
            
            ANSWER: \textit{We deploy a smooth spline interpolation of degree five on a small time-interval from a sequence of joint-pose annotations per channel. This part is  explained in Section V.A.}
            
            \item \textbf{The authors note that "Penn Action is not trained using IMU-tCNN", but it's unclear how it is trained, or used given this. This further muddies the role of the IMU-tCNN and clarification is needed here.}
            
            ANSWER: \textit{For all the datasets, firstly, the given pose annotations are visualised. Subsequently, the joints are mapped to the branches of IMU-tCNN. However, for Penn Action, there is no clarity of the joints, as they did not form a skeleton-like figure when visualising and their joint names were not semantically clear; therefore, mapping is not possible. We have added some clarification of the mapping human limbs-branches of the architecture in Section III.A and also for all datasets in Section IV.}
        \end{itemize}

    
    \subsection*{Reviewer 3349}
    
        \begin{itemize}
            \item \textbf{The methodology section is instead quite short and, in fact, I could not find a significant technical contribution, which is, to my understanding, mostly focused on the capability of achieving good performances with limited data. }
            
            ANSWER: \textit{Transferability and data exploiting from sources with domain, e.g., different domains, sensor setup, scenarios, number of subjects, different to the one of the target is still relevant, and not entirely solved. Besides, works for multichannel time-series HAR could benefit from data for video-based HAR, as the latter fuses RGB data and pose information for improving performance. Moreover, methods for semi-automated annotation, e.g., using human activity retrieval for annotating multichannel time-series HAR efficiently could also benefit from pose information. Semi-Automated methods have used pose data for boosting the annotation process deploying a model that retrieves results similar to a requested activity query. Thus, an evaluation of models for improving performance with limited data becomes handy when annotating IMU data \cite{avsar_2021}, see ARDUOUS Annotation workshop {https://text2hbm.org/arduous/}, Retrieval-based annotation of multi-channel time series data for HAR.}
            
        \end{itemize}


==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/figures/network.tex <==
\begin{figure}[!ht]

%\begin{wrapfigure}[1]{!ht}{0pt}
    \centering

    \begin{tikzpicture} [x=0.4cm,y=0.4cm][scale=0.2]
        %node distance = 1mm and -5mm,
        \tikzstyle{node1}=[text=black, font=\tiny \bfseries];
        \tikzstyle{node2}=[text=black, font=\tiny \bfseries];
        \tikzstyle{node3}=[text=black, font=\tiny];
        \tikzstyle{node4}=[text=black, font=\tiny];
        \tikzstyle{arrow1} = [line width=0.5]
        \tikzstyle{circle1}=[circle,draw=black, minimum size=0.1cm, line width=0.2mm, inner sep=0pt]
        \tikzstyle{circle2}=[circle,draw=black, minimum size=0.05cm, line width=0.1mm, inner sep=0pt, fill=black]
        %\node (label) at (0.0 - 6.2, 0.0 + 0.8)[draw=white, line width=0.0]{
       
       \node (label) at (0.0 - 15.5, 2.2 + -0.2)[]{
                \includegraphics[width= 0.05\textwidth]{video5.png}
                };
       
       \node (label) at (0.0 - 15.5, 2.2 + 0.1)[]{
                \includegraphics[width= 0.05\textwidth]{video4.png}
                };
       
        \node (label) at (0.0 - 15.5, 2.2 + 0.6)[]{
                \includegraphics[width= 0.05\textwidth]{video3.png}
                };
        \node (label) at (0.0 - 15.5, 2.2 + 1.0)[]{
                \includegraphics[width= 0.05\textwidth]{video2.png}
                };
        \node (label) at (0.0 - 15.5, 2.2 + 1.4)[]{
                \includegraphics[width= 0.05\textwidth]{video1.png}
                };
        %\draw [-latex](0.0 -6.2,0+0.9) -- (0.0 - 5.5, 0.0 + 0.9);
        \node [node1] at (0.0-14.5,1.5 - 0.9){Annotated Pose Data};
         \draw [-latex](0-13.5,0+3.2) -- (0.0 -11.5, 0.0 + 3.2);
        \node [node1] at (0.0-9.3,0.9 + 3.8){Human Pose};
        \node [node1] at (0.0-16,0.9 + 3.8){Video};
        %\node [node1] at (0.0-13.8,0.9 + 4){Pose};
        \node [node1] at (0.0-12.5,0.9 + 4.2){Source Dataset};
         \node (label) at (0.0 - 9, 0.0 + 0.7 + 2)[]{
                \includegraphics[width= 0.072\textwidth]{human.jpg}
              };
        %\draw [-latex](0-11.5,0+0.9) -- (0.0 -10.7, 0.0 + 0.9);
        
        \node (label) at (0.0 -14, 0.0 - 1.7)[]{
                \includegraphics[width= 0.14\textwidth]{pose.png}
              }; 
        
        \node (label) at (0.0 -9.5, 0.0 - 1.7)[]{
                \includegraphics[width= 0.14\textwidth]{Images/derivatives.png}
              }; 
           
        \node (label) at (0.0 -1 , 0.0 + 0.7)[]{
                \includegraphics[width= 0.23\textwidth]{synthetic.png}
              }; 
        \draw [rounded corners,line width=0.05mm, opacity=0.8] (0.0-17.2,0.0-4 ) rectangle +(11,9.5);
        
        
        %\node[arrow1] at (0.0 - 1.8, 0.0 + 0.5)
        %\draw [-latex](0 -0.5,0+0.9) -- (0.0 + 0.5, 0.0 + 0.9);
        \node [node1] at (0.0-9.1,0.6){Synthetic Data};
        \node [node3] at (0.0+2,-2.8){Time};
        
        %\node (label) at (-4.3 , 0.0 +0.67)[]{
         %       \includegraphics[width= 0.09\textwidth]{acceleration2.png}
          %    }; 
              
        %\draw [line width=0.05mm, opacity=0.8] (0.0-17.2,0.0 -2) rectangle +(9.5,6);
        \node [node3] at (0.0-12.5,-1.5){D};
        \node [node3] at (0.0-9.2,-3.8){Time};
        \node [node3] at (0.0-5.9,+0.8){D};
        %\draw [line width=0.05mm,fill=tucol11, opacity=0.3](1.4 + 2.4,1.8)--(0.4 + 2.4,1.8)--(0 + 2.4,1.5)--(1 + 2.4,1.5)--(1.4 + %2.4,1.8)--(1.4 + 2.4,0.3)--(1 + 2.4,0)--(0 + 2.4,0)--(0 + 2.4,1.5)--(1 + 2.4,1.5)--cycle;
        %\draw  [arrow1](1 + 2.4,0.0) edge (1 + 2.4,1.5);
        %\node (label) at (0.0 + 6.7, 0.0 + 0.9)[]{
         %       \includegraphics[width= %0.5\textwidth]{conv_layers.png}
        %      };
        \node [node3] at (0.0-1.2,0.9 -5.7){Convolution layers};
        \node [node3] at (0.0-11.8,0.9 -5.7){Convolution layers};
        
        \node [node3] at (0.0-12,0.0-7.2){$C=64$};
        %\node [node3] at (0.0+0.6,0-0.3){$C=64$};
        %\node [node3] at (0.0+1.9,0-0.3){$C=64$};
        %\node [node3] at (0.0+3.1,0.0-0.3){$C=64$};
        \node [node3] at (0.0-8.8,0 - 4.8){FC};
        %\node [node3] at (0.0+4.7,0.0-0.3){$256$};
        %\node [node3] at (0.0+5.45,0.0-0.3){$256$};
        %\node [node1] at (0.0+10,0.9 + 1.55){Softmax};
        \node [node3] at (0.0+5.9-13,0.9 - 5.7){Softmax};
        \node [node3] at (0.0+6.4-13.5,0+1.7-7){Walk};
        \node [node3] at (0.0+6.4-13.7,0+1.3-7){Sit};     
        \node [node3] at (0.0+6.4-13.6,0+0.9-7){Run}; 
        \node [circle2] at (0.0+6.4-13.5,0.5-7){};
        \node [circle2] at (0.0+6.4-13.5,0.2-7){};
        \node [circle2] at (0.0+6.4-13.5,0-7.1){};
        \draw [rounded corners,line width=0.05mm, opacity=0.8] (0.0-14,0.0 - 7.5) rectangle +(4.2,2.5);
        \draw [rounded corners,line width=0.05mm, opacity=0.8] (0.0-9.6,0.0 - 7.5) rectangle +(1.5,2.5);
        %\draw (0+9,0-2.05) -- (0.0 + 9.2, 0.0 + 1.05);
        \draw [rounded corners,line width=0.05mm, opacity=0.8] (0.0-7.8,0.0 - 7.5) rectangle +(1.5,2.5);
        %\draw [line width=0.05mm,fill=tucol4, opacity=0.3](1.4 + 4.0,1.8)--(0.4 + 4.0,1.8)--(0 + 4.0,1.5)--(1 + 4.0,1.5)--(1.4 + 4.0,1.8)--(1.4 + 4.0,0.3)--(1 + 4.0,0)--(0 + 4.0,0)--(0 + 4.0,1.5)--(1 + 4.0,1.5)--cycle;
        %\draw  [arrow1](1 + 4.0,0.0) edge (1 + 4.0,1.5);
            \draw (1.1-10.6,0-6.2) -- (2.5 -10.6, 0.0 -6.2);
         \draw (1.1,0-6.2) -- (2.5 , 0.0 -6.2);
        
        %\node [node3] at (0.0+6.0,0.0-0.3){$C=64$};
        
        %\draw [line width=0.05mm,fill=tucol4, opacity=0.3](1.2  + 5.6,1.8)--(0.4  + 5.6,1.8)--(0  + 5.6,1.5)--(0.8  + 5.6,1.5)--(1.2  + 5.6,1.8)--(1.2  + 5.6,0.3)--(0.8  + 5.6,0)--(0  + 5.6,0)--(0  + 5.6,1.5)--(0.8  + 5.6,1.5)--cycle;
        %\draw  [arrow1](0.8  + 5.6,0.0) edge (0.8  + 5.6,1.5);
        
        %\node [node3] at (0.0+7.4,0.0-0.3){$C=64$};
 \draw [line width=0.05mm,fill=tucol11, scale=0.7, opacity=1](1.2 + 2.8-22.5,2.2-10)--(0.4 + 2.8-22.5,2.2-10)--(0 + 2.8-22.5,1.9-10)--(0.8 + 2.8-22.5,1.9-10)--(1.2 + 2.8-22.5,2.2-10)--(1.2 + 2.8-22.5,0.3-10)--(0.8 + 2.8-22.5,0-10)--(0 + 2.8-22.5,0-10)--(0 + 2.8-22.5,1.9-10)--(0.8 + 2.8-22.5,1.9-10)--cycle; 
         \draw [line width=0.05mm,scale=1](-13.16,4.35-10)--(-13.16,3-10);
       %\draw  [arrow1](0.8 + 7.0,0.0) edge (0.8 + 7.0,1.5);
      \draw [line width=0.05mm,fill=tucol11, scale=0.7, opacity=1](1.2 + 4.15-22.5,2.2-10)--(0.4 + 4.15-22.5,2.2-10)--(0 + 4.15-22.5,1.9-10)--(0.8 + 4.15-22.5,1.9-10)--(1.2 + 4.15-22.5,2.2-10)--(1.2 + 4.15-22.5,0.3-10)--(0.8 + 4.15-22.5,0-10)--(0 + 4.15-22.5,0-10)--(0 + 4.15-22.5,1.9-10)--(0.8 + 4.15-22.5,1.9-10)--cycle; 
        \draw [line width=0.05mm,scale=1](-12.24,4.35-10)--(-12.24,3-10);
       %
     \draw [line width=0.05mm,fill=tucol11, scale=0.7, opacity=1](1.2 + 5.5-22.5,2.2-10)--(0.4 + 5.5-22.5,2.2-10)--(0 + 5.5-22.5,1.9-10)--(0.8 + 5.5-22.5,1.9-10)--(1.2 + 5.5-22.5,2.2-10)--(1.2 + 5.5-22.5,0.3-10)--(0.8 + 5.5-22.5,0-10)--(0 + 5.5-22.5,0-10)--(0 + 5.5-22.5,1.9-10)--(0.8 + 5.5-22.5,1.9-10)--cycle; 
       \draw [line width=0.05mm,scale=1](-11.32,4.35-10)--(-11.32,3-10);
     %
        \draw [line width=0.05mm,fill=tucol11, scale=0.7, opacity=1](1.2 + 6.85-22.5,2.2-10)--(0.4 + 6.85-22.5,2.2-10)--(0 + 6.85-22.5,1.9-10)--(0.8 + 6.85-22.5,1.9-10)--(1.2 + 6.85-22.5,2.2-10)--(1.2 + 6.85-22.5,0.3-10)--(0.8 + 6.85-22.5,0-10)--(0 + 6.85-22.5,0-10)--(0 + 6.85-22.5,1.9-10)--(0.8 + 6.85-22.5,1.9-10)--cycle; 
       \draw [line width=0.05mm,scale=1](-10.42,4.35-10)--(-10.42,3-10);
       
       %\draw (1.1-6,0-6) -- (2.5-6 , 0.0 -6)
        %\draw (0+5.7,0+1.05) -- (0.0 + 5.8, 0.0 + 1.05);
       \draw [fill=tucol11, line width=0.05mm, opacity=1] (1.5-10.7,-5.5) rectangle +(0.2,-1.5);
        %\draw (0+4.1,0-2.9) -- (0.0 + 5.1,0-2.9);
        \draw [fill=tucol11, line width=0.05mm, opacity=1] (2-10.7,-5.5) rectangle +(0.2,-1.5);
     


       % \node [circle2] (c5) at (0.0+1.3-10,1.0-6.5) {};
        
        %\node [circle2] (c6) at (0.0+1.3-10,0.8-6.5) {};
        
        %\node [circle2] (c7) at (0.0+1.3-10,0.6-6.5) {};



        % Second block of the network %%%%%%%%%%
        
        
        %\node [node1] at (0.0+0.1,0.9-1.6){Limb m};
        
        \node [node1] at (0-0.5,4.7){Real On-body data};
        \node [node1] at (0-0.5,4.2){(Target Dataset)};
       % \node (label) at (0.0 - 4, 0.0 - 4.0)[]{
        %        \includegraphics[width= 0.13\textwidth]{acceleration.png}
       %       }; 
              
        %\node (label) at (0.0 + 6.7, 0.0 - 3.2)[]{
         %       \includegraphics[width= 0.53\textwidth]{conv_layers2.png}
         %     };
         \draw [-latex,line width=1pt](0-0.6,0 - 2.8) -- (0-0.6, 0.0 - 4.2);
         
       \draw [line width=1pt,scale=1](-15,3-7)--(-15,2-8);
       \draw [-latex,line width=1pt](0 -15,0-6) -- (0.0 -14, 0.0 - 6);
       \node [node1] at (0-16.1,0-5){Annotated};
       \node [node1] at (0-16,0-5.5){Pose};
       \node [node1] at (0-16,0-6){(or)};
       \node [node1] at (0-15.6,0-6.5){Synthetic Data};
       \node [node1] at (0-5,0-5.2){Transferring};
       \node [node1] at (0-4.9,0-5.6){Convolutional};
       \node [node1] at (0-5,0-6.3){Layers};
       \draw [-latex,line width=1pt](0-6.1,0-6) -- (-3.5, 0.0 -6);
       
        \node [node3] at (0.0 - 1,0.0-7.2){$C=64$};
        %\node [node3] at (0.0+0.7,0-6){$C=64$};
        %\node [node3] at (0.0+1.8,0-6){$C=64$};
        %\node [node3] at (0.0+2.9,0.0-6){$C=64$};
        \node [node3] at (0.0+1.9,0 - 4.7){FC};
        %\node [node3] at (0.0+4.55,0.0-4.3){$256$};
        %\node [node3] at (0.0+5.2,0.0-4.3){$256$};
        %\node [node1] at (0.0+6.5,0-4.2){Softmax};
        \node [node3] at (0.0+3.5,3-7.7){Softmax};
        \node [node3] at (0.0+3.5,1.7-7){Wave};
        \node [node3] at (0.0+3.5,1.3-7){Drink};     
        \node [node3] at (0.0+3.5,0.9-7.1){Jump}; 
        \node [circle2] at (0.0+3.5,0.5-7){};
        \node [circle2] at (0.0+3.5,0.2-7){};
        \node [circle2] at (0.0+3.5,0-7.1){};
        \draw [rounded corners,line width=0.05mm, opacity=0.8] (0.0-3.3,0.0 - 7.5) rectangle +(4.2,2.5);
        \draw [rounded corners,line width=0.05mm, opacity=0.8] (1.1,0.0 - 7.5) rectangle +(1.5,2.5);
        \draw [rounded corners,line width=0.05mm, opacity=0.8] (2.8,0.0 - 7.5) rectangle +(1.4,2.5);
        
        %\draw [line width=0.05mm, opacity=0.4] (0.0+0.6,0.0 - 3.1) rectangle +(1.4,2.0);
\draw [line width=0.05mm,fill=tucol11, scale=0.7, opacity=1](1-4.1,2.2-10)--(0.2-4.1,2.2-10)--(-0.2-4.1,1.9-10)--(0.6-4.1,1.9-10)--(1-4.1,2.2-10)--(1-4.1,0.3-10)--(0.6-4.1,0-10)--(-0.2-4.1,0-10)--(-0.2-4.1,1.9-10)--(0.6-4.1,1.9-10)--cycle; 
        \draw [line width=0.05mm,scale=1](-2.45,4.35-10)--(-2.45,3-10);
      %\draw  [arrow1](0.8 + 7.0,0.0) edge (0.8 + 7.0,1.5);
       \draw [line width=0.05mm,fill=tucol11, scale=0.7, opacity=1](1-4.1+1.35,2.2-10)--(0.2-4.1+1.35,2.2-10)--(-0.2-4.1+1.35,1.9-10)--(0.6-4.1+1.35,1.9-10)--(1-4.1+1.35,2.2-10)--(1-4.1+1.35,0.3-10)--(0.6-4.1+1.35,0-10)--(-0.2-4.1+1.35,0-10)--(-0.2-4.1+1.35,1.9-10)--(0.6-4.1+1.35,1.9-10)--cycle; 
        \draw [line width=0.05mm,scale=1](-1.5,4.35-10)--(-1.5,3-10);
       %
     \draw [line width=0.05mm,fill=blue, scale=0.7, opacity=1](1-4.1+2.7,2.2-10)--(0.2-4.1+2.7,2.2-10)--(-0.2-4.1+2.7,1.9-10)--(0.6-4.1+2.7,1.9-10)--(1-4.1+2.7,2.2-10)--(1-4.1+2.7,0.3-10)--(0.6-4.1+2.7,0-10)--(-0.2-4.1+2.7,0-10)--(-0.2-4.1+2.7,1.9-10)--(0.6-4.1+2.7,1.9-10)--cycle; 
       \draw [line width=0.05mm,scale=1](-0.53,4.35-10)--(-0.53,3-10);
       
      \draw [line width=0.05mm,fill=blue, scale=0.7, opacity=1](1-4.1+4.05,2.2-10)--(0.2-4.1+4.05,2.2-10)--(-0.2-4.1+4.05,1.9-10)--(0.6-4.1+4.05,1.9-10)--(1-4.1+4.05,2.2-10)--(1-4.1+4.05,0.3-10)--(0.6-4.1+4.05,0-10)--(-0.2-4.1+4.05,0-10)--(-0.2-4.1+4.05,1.9-10)--(0.6-4.1+4.05,1.9-10)--cycle; 
        \draw [line width=0.05mm,scale=1](+0.42,4.35-10)--(+0.42,3-10);
      
      %\draw (0+7.6,0-2.9) -- (0.0 + 7.5, 0-2.9);
        \draw [fill=blue, line width=0.05mm, opacity=1] (1.5,-5.5) rectangle +(0.2,-1.5);
        %\draw (0+4.1,0-2.9) -- (0.0 + 5.1,0-2.9);
        \draw [fill=blue, line width=0.05mm, opacity=1] (2,-5.5) rectangle +(0.2,-1.5);
        
       
        %\draw [line width=0.05mm,fill=tucol4, opacity=0.3](1.4 + 2.4,1.8- 3.0)--(0.4 + 2.4,1.8 - 3.0)--(0 + 2.4,1.5 - 3.0)--(1 + 2.4,1.5 - 3.0)--(1.4 + 2.4,1.8 - 3.0)--(1.4 + 2.4,0.3- 3.0)--(1 + 2.4,0- 3.0)--(0 + 2.4,0- 3.0)--(0 + 2.4,1.5- 3.0)--(1 + 2.4,1.5- 3.0)--cycle;
        %\draw  [arrow1](1 + 2.4,0.0- 3.0) edge (1 + 2.4,1.5- 3.0);


        %\draw [line width=0.05mm,fill=tucol4, opacity=0.3](1.4 + 4.0,1.8- 3.0)--(0.4 + 4.0,1.8- 3.0)--(0 + 4.0,1.5- 3.0)--(1 + 4.0,1.5- 3.0)--(1.4 + 4.0,1.8- 3.0)--(1.4 + 4.0,0.3- 3.0)--(1 + 4.0,0- 3.0)--(0 + 4.0,0- 3.0)--(0 + 4.0,1.5- 3.0)--(1 + 4.0,1.5- 3.0)--cycle;
        %\draw  [arrow1](1 + 4.0,0.0- 3.0) edge (1 + 4.0,1.5- 3.0);
        
        
        %\draw [line width=0.05mm,fill=tucol4, opacity=0.3](1.2  + 5.6,1.8- 3.0)--(0.4  + 5.6,1.8- 3.0)--(0  + 5.6,1.5- 3.0)--(0.8  + 5.6,1.5- 3.0)--(1.2  + 5.6,1.8- 3.0)--(1.2  + 5.6,0.3- 3.0)--(0.8  + 5.6,0- 3.0)--(0  + 5.6,0- 3.0)--(0  + 5.6,1.5- 3.0)--(0.8  + 5.6,1.5- 3.0)--cycle;
        %\draw  [arrow1](0.8  + 5.6,0.0- 3.0) edge (0.8  + 5.6,1.5- 3.0);
        

        %\draw [line width=0.05mm,fill=tucol4, opacity=0.3](1.2 + 7.0,1.8- 3.0)--(0.4 + 7.0,1.8- 3.0)--(0 + 7.0,1.5- 3.0)--(0.8 + 7.0,1.5- 3.0)--(1.2 + 7.0,1.8- 3.0)--(1.2 + 7.0,0.3- 3.0)--(0.8 + 7.0,0- 3.0)--(0 + 7.0,0- 3.0)--(0 + 7.0,1.5- 3.0)--(0.8 + 7.0,1.5- 3.0)--cycle;
        %\draw  [arrow1](0.8 + 7.0,0.0- 3.0) edge (0.8 + 7.0,1.5- 3.0);
        
        
        %\draw [fill=tucol2, line width=0.05mm, opacity=0.4] (8.5,0.0- 3.0) rectangle +(0.2,1.8);
        
        
        
        % Last layers
        
        %\draw [line width=0.05mm, fill=tucol8, opacity=0.1](6.7+2.0,1.8)--(6.7+2.0,-0.3-2.7)--(6.7+2.5,-0.2-1.3)--(6.7+2.5,1.6-1.3)--cycle;
        
        %\node [node4] at (0.0+0.5+8.0,0.0-0.5){concat.};
        
        %\draw [fill=tucol8, line width=0.05mm, opacity=0.4] (8.7 + 0.5,0.0- 1.5) rectangle +(0.2,1.8);
        
       % \node [node4] at (0.0+10.0,0.0+0.3){$C=256$};
        
        %\draw [fill=tucol2, line width=0.05mm, opacity=0.4] (8.7 + 1.0,0.2- 1.5) rectangle +(0.2,1.4);
        
        %\node [node4] at (0.0+10.6,0.0-1.6){Softmax};
        
        %\draw [fill=tucol5, line width=0.05mm, opacity=0.4] (8.7 + 1.8,0.2- 1.5) rectangle +(0.2,1.4);
        
        
        %Explanation layers
        %\draw [fill=tucol4, line width=0.05mm, opacity=0.4] (8.7 + 0.5,0.2- 2.8) rectangle +(0.2,0.2);
        
        %\node [node2] at (8.7 + 2.3,0.2- 2.7){[$5\times1$] temporal-conv};
        
        %\draw [fill=tucol1, line width=0.05mm, opacity=0.4] (8.7 + 0.5,0.2- 3.2) rectangle +(0.2,0.2);
        
        %\node [node2] at (8.7 + 2.4,0.2- 3.1){[$2\times1$] max-pooling};
        
        %\draw [fill=tucol5, line width=0.05mm, opacity=0.4] (8.7 + 0.5,0.2- 3.6) rectangle +(0.2,0.2);
        
        %\node [node2] at (8.7 + 2.4,0.2- 3.5){Sigmoid act-function};
               
    \end{tikzpicture}

   \caption{\scriptsize{A tCNN is pre-trained on either pixel-coordinate sequences of joints or their derivatives for HAR. The convolutional layers from the pre-trained network are transferred to a tCNN being trained on three on-body devices datasets for HAR.
   \vspace{-5mm}
   }}
    \label{fig:networks}
%\end{wrapfigure}
\end{figure}


%The tCNN architecture contains 4 temporal convolutional layers. The output is forwarded to a fully connected (FC) layer. The output layer is a softmax function \cite{niemann2020lara}.

==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/results/LaraMM.tex <==
There is no published research for HAR using LARa-MM. The baseline for LARa-MM is computed using a batch size of $200$ and $10$ epochs. However, the $\%wF1$ score for all the $D_s$ is comparable or significantly lower than the LARa-MM baseline, except for a few cases when the $D_t$ is less than $100\%$. These results constitute the first HAR performance for LARa-MM.
    
\begin{table}
    \caption{\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{LARa-MM}$ using the joint poses and the synthetic data. The $N_{conv}$ changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $N_{conv}$ corresponding to highest $wF1[\%]$ is fixed and $\%D_t$ is varied. \textit{tCNN}$_{LARa-MM}$ is the baseline. Std $wF1[\%]$ lies around $0.01$. The performance of the \textit{tCNN-IMU}$_{D_s}^{MM}$ is similar, thus, not shown.}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c c|c}
        \hline
        \multicolumn{10}{c}{\bm{$tCNN_{D_s}^{MM}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c|}{D$_s$=CAD60} & \multicolumn{2}{c|}{D$_s$=Penn} & \multicolumn{2}{c|}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-9} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\
        [0.1em]
        \hline
        \hline
        $c_1$  & 65.14  & 64.72 & 65.01  & 65.67    & 64.27 & 65.97 & 64.33 & 64.79  & \multirow{4}{*}{65.71} \\ 
        [0.1em]
        %\cline{2-9}
        $c_{1,2}$  & 65.21 & 64.12 & 64.80  & 65.05  & 63.73 & 64.81  & 64.09 & 63.21  &  \\
        [0.1em]
        %\cline{2-9}
        $c_{1-3}$ & 65.45 & 62.04  & 64.56  & 60.26  & 63.19 & 62.35 & 63.51 & 63.11  &\\ 
        [0.1em]
        %\cline{2-9}
        $c_{1-4}$  & 65.71 & 47.72 & 64.38 & 53.25 & 62.74 & 44.31 & 62.81 & 61.91  & \\ 
        [0.1em]
        \hline
        \hline
        75\bm{$\%D_t$} & \textbf{65.26} &   60.93 & 62.90  & 62.90 & 63.12   & 63.73 & 62.61 & 62.95  & 63.83 \\ 
        [0.1em]
        %\cline{2-9}
        50\bm{$\%D_t$}  & \textbf{59.37} & {54.74} & 51.70  &  52.73 & \textbf{56.98} & 54.73 & {53.42} & \textbf{57.67}  & 53.14   \\ 
        [0.1em]
        %\cline{2-9}
        30\bm{$\%D_t$}  & 53.80 &  50.09  & 45.75 & 52.20 & 49.90 & 45.88 & 51.12 & 50.84 & 51.19 \\ 
        %\cline{2-9}
        10\bm{$\%D_t$}  & 47.41 & 46.81   & \textbf{51.36} & 48.95 & 49.01 & 46.59 & \textbf{51.57} & 43.32 & 47.06 \\ 
        \hline
        \multicolumn{6}{c}{\vspace{-3mm}}\\
    \end{tabular}
    }
    \label{tab:TL_S_LARaMM}
\end{table}


==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/results/LaraOB.tex <==
\label{subsection:TL_S_L}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}
    \centering
    \caption {\scriptsize{Mean $wF1[\%]$ of the \textit{tCNN}$_{D_s}^{LARa-Mb}$ and \textit{tCNN-IMU}$_{D_s}^{LARa-Mb}$ using the joint poses and the synthetic data. The $N_{conv}$ changes from $c_1$ to $c_{1,2,3,4}$ keeping $100\%$ of the $D_t$. Subsequently, the $N_{conv}$ corresponding to highest $wF1[\%]$ is fixed and $[10, 30, 50, 75]\%$ of the $D_t$ are deployed for fine-tuning. The \textit{tCNN}$^{LARa-Mb}$, trained on the training set of the LARa-OB, denotes the baseline. Std $wF1[\%]$ lies around $0.01$.}}
    \label{tab:TL_S_LARaOB}
    %\subcaption*{\bm{$tCNN_{D_s}^{Pamap2}$}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c c|c}
        \hline
        \multicolumn{10}{c}{\bm{$tCNN_{D_s}^{LARa-Mb}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c}{D$_s$=JHMDB} & \multicolumn{2}{c}{D$_s$=CAD60} & \multicolumn{2}{c}{D$_s$=Penn} & \multicolumn{2}{c}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-11} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\  
        [0.1em]
        \hline
        \hline
        $c_1$ & {75.47}  & {74.77}  & 74.47 & 74.94       & 75.24  & 74.78 & 75.90  & 74.95 &    \multirow{4}{*}{75.06}      \\  
        [0.1em]
        %\cline{2-9}
        $c_{1,2}$  & {75.10}  & {74.70}  &  74.53 & 74.85  & 75.21 & 74.20 & 75.82 & 74.90 &             \\ 
        [0.1em]
        %\cline{2-9}
        $c_{1-3}$     & 74.29  & 74.46   & 74.69 & 74.66 &  75.01  & {70.91}    & 74.59 & 75.55 & \\ 
        [0.1em]
        %\cline{2-9}
        $c_{1-4}$  & {73.37}   & {74.33}  & 74.85 & 74.53       & 74.85 & 54.20 & 75.37 & 74.46& \\ 
        [0.1em]
        \hline
        \hline
        75\bm{$\%D_t$}  & \textbf{73.06}  & \textbf{73.49} & \textbf{73.46} &  \textbf{73.10} &  \textbf{73.92}  & \textbf{73.75} & \textbf{73.21} & \textbf{73.77} & 71.08     \\ 
        %\cline{2-9}
        50\bm{$\%D_t$}  & \textbf{72.24}   & \textbf{71.02}   & \textbf{71.89}  & \textbf{72.08} & \textbf{73.01}   & \textbf{70.66}  & \textbf{72.53}     & \textbf{72.02} & 69.01      \\ 
        [0.1em]
        %\cline{2-9}
        30\bm{$\%D_t$}  & \textbf{67.80}   & \textbf{64.81}    & \textbf{66.65}  & \textbf{66.20} & \textbf{67.42}      & \textbf{67.94} & \textbf{67.69} & \textbf{65.90} &  62.71     \\
        %\cline{2-9}
        10\bm{$\%D_t$}  & \textbf{58.57}   & \textbf{59.66}   & \textbf{61.83}  & \textbf{59.79} & \textbf{60.50}   & \textbf{59.41}  & \textbf{61.93}     & \textbf{59.68} & 52.92      \\ 
        [0.1em]
        \hline
        \multicolumn{8}{c}{\vspace{-1mm}}\\
    \end{tabular}
    }
    %\bigskip
    \vspace{2mm}
    %\subcaption*{\bm{$tCNN-IMU_{D_s}^{Pamap2}$}}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{10mm} c c|c c|c c|c}
        \hline
        \multicolumn{8}{c}{\bm{$tCNN-IMU{D_s}^{LARa-Mb}$}} \\
        [0.2em]
        %\hline
        \textbf{Transf.} & \multicolumn{2}{c|}{D$_s$=JHMDB} & \multicolumn{2}{c}{D$_s$=CAD60} & \multicolumn{2}{c}{D$_s$=NTU RGB+D} & \textbf{Baseline} \\ 
        [0.1em]
        %\cline{3-11} 
        \textbf{layers} &  \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth}  & \textbf{Pose}  & \textbf{Synth} & \textbf{Pose} &  \\  
        [0.1em]
        \hline
        \hline
        $c_1$ & {75.52}  & 76.04 & 75.36 & 75.32    & {75.05}  & {75.52} &    \multirow{4}{*}{75.09}      \\  
        [0.1em]
        %\cline{2-7}
        $c_{1,2}$  & 75.23 & 75.69 & 74.99  & 75.02 &  {74.75} & 75.19&             \\ 
        [0.1em]
        %\cline{2-7}
        $c_{1-3}$     & 75.02  & 75.11   & 74.32 & 74.69 &  {74.33} & 74.59 & \\ 
        [0.1em]
        %\cline{2-7}
        $c_{1-4}$  & 74.82   & 74.86  & 73.99 & 74.36 &   {74.05} & 73.99 & \\ 
        [0.1em]
        \hline
        \hline
        75\bm{$\%D_t$}  & \textbf{74.82}  & \textbf{74.75} & 72.28 &   \textbf{73.65} & \textbf{73.92} & 73.33  & 73.51     \\ 
        %\cline{2-7}
        50\bm{$\%D_t$}  & \textbf{71.26}   & \textbf{73.88}  &  \textbf{71.10} & \textbf{70.91} & \textbf{71.50}  & \textbf{70.91} & 70.30     \\ 
        [0.1em]
        %\cline{2-7}
        30\bm{$\%D_t$}  & {66.38}   & {66.48}    & {67.01}  & \textbf{68.34} &  {67.45} &  {67.31} & 67.54    \\ 
        %\cline{2-7}
        10\bm{$\%D_t$}  & \textbf{65.99}   & \textbf{65.18}    & \textbf{66.12}  & \textbf{66.95} &  \textbf{65.44} &  \textbf{62.80} & 57.47    \\
        \hline
        \multicolumn{6}{c}{\vspace{-10mm}}\\
    \end{tabular}
    }
\end{table}


Tab.~\ref{tab:TL_S_LARaOB} shows the performance of the transfer learning on the LARa-Mb as the target scenario. In this case, the performance of the four networks \textit{tCNN}$_{JHMDB}^{LARa-Mb}$, \textit{tCNN}$_{CAD60}^{LARa-Mb}$, \textit{tCNN}$_{Penn}^{LARa-Mb}$ and \textit{tCNN}$_{NTU}^{LARa-Mb}$ for both data sources, pose annotations and synthetic data, and different transferable layers remains similar to the \textit{tCNN}$^{LARa-Mb}$. The activities in the LARa-Mb dataset are performed in a warehouse environment, whereas the source datasets consider ADLs. The performance improves only when considering the $75\%$, $50\%$, $30\%$ or $10\%$ of the LARa-Mb. 


==> Video-based Pose-Estimation Data as Source for Transfer Learning in Human Activity Recognition ICPR2022_arxiv/results/opportunity.tex <==


\input{Tables/locomotion_cnn}
%\input{Tables/locomotion_cnnimu}

Tab.~\ref{tab:TL_S_Loc} shows the classification performance of the transfer learning on the Opp-Loc dataset. The \textit{tCNN}$^{Loc}$ is considered as baseline. Only the \textit{tCNN}$_{JHMDB_{Pose}}^{Loc}$ using pose annotations and \textit{tCNN}$_{NTU_{}}^{Loc}$ improve the performance. In the case of having $[10,30,50]\%$ of the $D_t$, the pre-trained networks on JHMDB, CAD60 and Penn significantly improved the performance.
Tab.~\ref{tab:TL_S_Loc} also presents the performance of the three pre-trained architectures on the Opp-Ges $D_t$. In comparison with the Opp-Loc, pre-training the \textit{tCNN} with the three source datasets with both the pose annotations or the synthetic on-body devices influences the performance on the $D_t$ significantly, especially when transferring the first convolutional layer. The performance in all scenarios improves significantly when considering $50\%$ or $30\%$ of the $D_t$ and pre-training with the three $D_s$ using pose annotations or the synthetic on-body devices.

%\input{Tables/gestures_cnn}
%\input{Tables/gestures_cnnimu}



==> chapters/04_experiments_text_comments.tex <==
            \begin{table}[ht]
            \begin{tabular}{|l|l|l|l|}
                \hline
                \textbf{Source Datasets $D_s$}      & \textbf{$\%$ test Accuracy unseg} & \textbf{$\%$ test Accuracy seg} & $\%wF1$\\ \hline
                \textbf{JHMDB}      & 81.45$\pm$0.032 & 91.18$\pm$0.027 &  90.53$\pm$0.003\\ 
                \hline
                \textbf{CAD60}      & 36.78$\pm$0.003 & 56.28$\pm$0.02 &  49.50$\pm$0.015 \\ 
                \hline
                \textbf{Penn Action} & 77.76$\pm$0.002 & 91.82$\pm$0.026 & 90.98$\pm$0.06 \\ 
                \hline
            \end{tabular}
            \caption{Experimentally obtained best ss for $D_s$. The ss is chosen based on the highest obtained unsegmented validation accuracy for each dataset.}
            \label{tab:ss}
        \end{table} 
        
    
    \begin{comment}
    \subsection{Transfer Learning from JHMDB to PAMAP2}
        \label{subsection:TL}
        
        The hyperparameters used for training the network are: (1) momentum of $0.9$, (2) learning rate of $10^{-5}$, (3) 100 epochs, and (4) batch size of 400. 
            
       
        Table \ref{tab:Pose_acc} shows the best result for JHMDB using tCNN trained from scratch for HAR ($tCNN_{JHMDB}$).As observed, the $wF1[\%]$ score is higher for $tCNN_{JHMDB}$ than $tCNN_{JHMDB\_p}$. A possible reason could be that, as the pose data is up-sampled by $4$ and the percent overlap of sliding windows is increased to $88\%$, therefore more data is available for training. The new data is an approximation of the real data. This enables the network to learn generic filter and tCNN is able to generalize better. As a result, the $tCNN_{JHMDB\_S}$ learns better and gives a higher $wF1[\%]$ score.
    
        \begin{table}[]
            \centering
            \resizebox{\columnwidth}{!}{
            \begin{tabular}{|c| c |c| c|c|c|c|} 
            \hline
            Metric
            & $tCNN_{JHMDB}$ & $tCNN_{JHMDB\_S}$& $tCNN_{CAD60}$ & $tCNN_{CAD60\_S}$& $tCNN_{Penn}$ & $tCNN_{Penn\_S}$\\
            \hline
            wF1[\%] & 53.2857 &91.13 &70.90$\pm$0.65 &47.5 $\pm$1.5 & 86.3$\pm$0.27&81.3$\pm$0.32\\ 
            
            \hline
            \end{tabular}
            }
            \caption{The $wF1[\%]$ for HAR using $tCNN_{D_s}$. The network is trained from scratch on the pose data and synthetic IMU data. The target dataset is considered as PAMAP2, therefore $D_s$ are sampled to $100$ fps.}
            \label{tab:Pose_acc}
        \end{table}
        
        
        The $wF1\%$ and $\%$test accuracy for $tCNN_{JHMDB\_pamap2}$ are shown in table \ref{tab:tf_JP}. The obtained $\%wF1$ score is highest for $tCNN_{JHMDB\_pamap2^{c1}}$. Thus, further experiments are performed by fixing the number of transferred layers to $c1$ and varying the target data[\%].
       
        \begin{table}[]
        \centering
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\textbf{$\%D_{t}$}} & \multicolumn{2}{l|}{\textbf{$tCNN_{JHMDB\_PAMAP2}$}}           & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}}             & \multirow{}{}{\textbf{p value}} \\ \cline{3-6}
                                                     layers&                                  & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc}   &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 87.95$\pm$0.06          & 88.98$\pm$0.05          & 86.67$\pm$0.05          & 87.8012$\pm$0.04          & 0.005912                          \\ \hline
        c1,c2,c3                                     & 100                              & 87.70$\pm$0.06          & 88.51$\pm$0.07          & 86.67$\pm$0.05          & 87.8012$\pm$0.04          & 0.100044                          \\ \hline
        c1,c2                                        & 100                              & 88.57$\pm$0.05          & 89.32$\pm$0.06          & 86.67$\pm$0.05          & 87.8012$\pm$0.04          & 0.00034                           \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{88.97$\pm$0.08} & \textbf{89.53$\pm$0.07} & \textbf{86.67$\pm$0.05} & \textbf{87.8012$\pm$0.04} & \textbf{0.00002}                  \\ \hline
        c1                                           & 75                               & 86.15$\pm$0.05          & 87.20$\pm$0.06          & 86.30$\pm$0.06          & 87.10$\pm$0.08            &     0.843                              \\ \hline
        c1                                           & 50                               & 86.10$\pm$0.06          & 86.93$\pm$0.08          & 84.10$\pm$0.08          & 84.98$\pm$0.07            &        0.00004                           \\ \hline
        c1                                           & 30                               & 85.55$\pm$0.04          & 86.13$\pm$0.05          & 84.05$\pm$0.09          & 84.93$\pm$0.06            &   0.0107                                \\ \hline
        \end{tabular}
        }
        \caption{The table shows $wF1[\%]$ for $tCNN_{JHMDB\_pamap2}$. The $wF1[\%]$ and $\%$test accuracy of $tCNN_{PAMAP2}$ is used as the baseline. The number of convolution layers transferred are varied.}
        \label{tab:tf_JP}
        \end{table}
        
        
        
        %\begin{flushleft}
        \it{Discussion}\\
        %\end{flushleft}
         The results in table \ref{tab:tf_JP} show that the performance of HAR using tCNN on PAMAP2 improves when pre-training with JHMDB dataset. The JHMDB and PAMAP2 dataset contain $50\%$ overlapping classes (sit, walking, run, ascending stairs, and stand).\\
        
        Consider the results in table \ref{tab:tf_JP}, when $100\%$ of target data (PAMAP2) was used and the number of transferred layers is varied. The the p value when transferring one, two, or four layers indicate that the increase in $\%wF1$ score is highly significant.  It is observed that the best improvement in $wF1\%$ score occurs when only the first c1 is transferred. As the number of transferred layers increase, the $wF1\%$ gradually decreases. A possible explanation could be that the lower-layers (near the input) of a CNN capture generic or high level features \cite{ordonez2016deep_conv}. Deeper layers (near the output) of the network capture more scenario-specific filters, leading to a decrease in transferability.\\
        
        The number of layers transferred is fixed at $c1$ and the amount of target data used is either $50\%$ or $30\%$ or $70\%$. It is observed in table \ref{tab:tf_JP} that the $wF1\%$ when using a $tCNN_{JHMDB\_PAMAP2}$ is higher than the $wF1\%$ of a $tCNN_{PAMAP2}$. The increase is highly significant when $50\%$ or $30\%$ of target data is used for fine tuning. However, when $75\%$ of target data is used. This implies that using a pre-trained tCNN for HAR improves the performance ($wF1$) significantly when the annotated training data is scarce.\\
        
        Table \ref{tab:TL_PR}, shows the precision and recall values. For comparing the performance of $tCNN_{JHMDB\_PAMAP2}$, the harmonic mean (HM) of precision and recall is computed for each activity. The activities  climb stairs, sit, run, walk, and stand are common between PAMAP2 and JHMDB. It is observed that implementing transfer learning results in an increase in HM of the activities: climb stairs, sit, and stand. As these activities are common between the JHMDB and PAMAP2 dataset, therefore the filters learnt by the initial layers of the tCNN are generic to these common activities and can be transferred.\\
        
        The performance of the activity Run is nearly the same. There is a slight reduction in the harmonic mean for the class walk. A possible explanation could be that the walking activity in JHMDB consists of $41$ videos from internet and all videos have different subjects performing the activity. The walking speed of these subjects varies significantly. In some videos the subjects seems to be running and in some the subject is dawdling. Also, there is a large intra-class variability in the walking class. In some videos have the person dragging or carrying objects while walking. Therefore, the first layer of the pre-trained network might have learnt features which are not generic to the walking activity. Thus, for fro $tCNN_{JHMDB_PAMAP2^{c1}}$, the network might confuse walking activity with other activities.\\
        
        There is also an increase in harmonic mean for activities, which are only present in PAMAP2 dataset: rope jump, descending stairs, vacuum cleaning and ironing. The activity rope jump in PAMAP2 could be considered similar to the Jump action in JHMDB. The ironing action can be considered similar to the pour action in JHMDB. As both ironing and pour actions involve one arm to be stationary and a side-ward movement of the other arm. Also, the persons performing these two actions are mostly standing and perform the actions approximately at a height of their stomach. Similarly, the action of vacuum cleaning could be considered similar to the pick action. As, both actions involve a combination of bending and movement of arms. The action descending stairs can be considered similar to ascending stairs. The harmonic mean for the above mentioned similar activities increases. The performance for actions cycling and lying is nearly the same. However, the performance for action Nordic Walk decreases. A possible reason could be that even the features of the first layer of the pre-trained network are not generic enough to represent the Nordic Walk action. Subsequently, this might hinder with learning of specific features for Nordic Walk action in deeper layers. \\
        
        Summing up the results, it can be said that transfer learning from JHMDB to PAMAP2 significantly improves the performance of tCNN trained on PAMAP2 for HAR. 9 out of 12 activities in PAMAP2 are similar to JHMDB. As a result the lower layers learn features that are generic to human activities. The features of the lower layer are more generic than higher layers. This also suggests that filters learn short temporal-relations from the input sequence per channel independently of the rather related domain. Also, when annotated data is scarce ($30\%$) then transfer learning is advantageous. \\
        \end{comment}
        %%%%%%%%%%%%%%%%%%%%%%%%
        
        
        
        
            
        
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{comment}
    \subsection{Transfer Learning from CAD60 to PAMAP2}
    \label{subsection:TL_C_P}
    
        
       
        The table \ref{tab:Pose_acc} shows the best result for CAD60 dataset, trained from scratch using tCNN. \\
        
        As seen in table \ref{tab:Pose_acc}, the $wF1[\%]$ is higher when tCNN is trained using CAD60 pose data than when tCNN is trained with synthetic IMU data. Fig \ref{fig:J_CAD} represents (a) pose data for two random channels for first 100 frames of JHMDB dataset and (b) CAD60 dataset. Similar time-series signal are observed for all the channels in CAD60 for the entire duration of the recording. As observed in Fig \ref{fig:J_CAD}, the data points that are close to each other in CAD60 dataset have extreme differences in values. This causes incorrect approximations due to smoothing effect. All the channels of the CAD60 dataset show a similar behaviour. Up-sampling could be the reason for the incorrect approximations. Therefore, the approximated values by spline interpolation are not accurate, and the features learnt by the network are inaccurate. This explains the decrease in $wF1$ score.   
        \begin{figure}[]
        \begin{center}
        \includegraphics[scale=0.6]{J_CAD}
        \end{center}
        \caption {shows (a) pose data for $2$ random channels for first 100 frames of JHMDB dataset and (b) pose data for $2$ random channels for first 100 fames of CAD60 dataset.}
        \label{fig:J_CAD}
        \end{figure} 
        
        
        The $wF1\%$ and $|\%$ test accuracy for $tCNN_{JHMDB\_PAMAP2}$ is shown in table \ref{tab:tf_CP}. $tCNN_{PAMAP2}$ is considered as the baseline for comparison. The $wF1$ score is highest when transferring only first layer from CAD60 to PAMAP2. Thus, further experiments are performed by fixing the number of transferred layers to $c1$ and varying the target data[\%].
        \begin{table}[H]
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. layers}} & \multirow{}{}{\textbf{$\%D_{LaraMM}$}} & \multicolumn{2}{l|}{\textbf{$tCNN_{CAD60\_PAMAP2}$}}           & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}}           & \multirow{}{}{\textbf{p value}} \\ \cline{3-6}
                                                     &                                  & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc} &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 70.72$\pm$0.032         & 71.26$\pm$0.22          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2,c3                                     & 100                              & 86.06$\pm$0.007         & 86.83$\pm$0.67          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2                                        & 100                              & 88.19$\pm$0.89          & 86.24$\pm$0.80          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{87.35$\pm$0.01} & \textbf{88.20$\pm$0.36} & \textbf{86.67$\pm$0.05} & \textbf{87.80$\pm$0.04} & \textbf{0.359}                    \\ \hline
        c1                                           & 75                               & 86.649$\pm$0.01         & 87.34$\pm$1.09          & 86.30$\pm$0.06          & 87.10$\pm$0.08          & 0.606                             \\ \hline
        c1                                           & 50                               & 84.80$\pm$0.007         & 85.98$\pm$0.60          & 84.10$\pm$0.08          & 84.98$\pm$0.07          & 0.346                             \\ \hline
        c1                                           & 30                               & 86.40$\pm$0.006        & 87.33$\pm$0.09          & 84.05$\pm$0.09          & 84.93$\pm$0.06          &      0.0                             \\ \hline
        \end{tabular}
        }
        \caption{The $wF1[\%]$ and $|\%$ test accuracy score for $tCNN_{CAD60\_PAMAP2}$.  $tCNN_{PAMAP2}$ (table \ref{tab:wf1}) is considered as baseline. The number of convolution layers transferred and the $[\%]$ of target data used are varied. Numbers in bold shows the hyper-parameters which give the best $wF1[\%]$ score.}
        \label{tab:tf_CP}
        \end{table}
        \end{comment}
        
        
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{comment}
        
        
        \begin{table}[]
        %\vspace{-2em}
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
         ss     & \multicolumn{2}{l|}{\textbf{JHMDB}}                                  & \multicolumn{2}{l|}{\textbf{CAD60}}        & \multicolumn{2}{l|}{\textbf{Penn Action}}  \\ \hline
         \textbf{} & \textbf{\% Acc unseg}             & \textbf{\%Acc seg}               & \textbf{\% Acc unseg} & \textbf{\%Acc seg} & \textbf{\% Acc unseg} & \textbf{\%Acc seg} \\ \hline
         1         & 41.74$\pm$0.023                            & 78.72  $\pm$0.031                           & 40.06 $\pm$0.019                       & 56.375 $\pm$0.027                      & \textbf{74.63}   $\pm$0.013                     & 91.92   $\pm$0.016\\ \cline{2-8} 
    5         & 50.237 $\pm$0.025                           & 76.39$\pm$0.021                            & 43.84 $\pm$0.027                & 54.95 $\pm$0.029             & 71.66   $\pm$0.027              & 88.91  $\pm$0.029            \\ \cline{2-8} 
    12        & \textbf{79.97}  $\pm$0.032                           & 92.31     $\pm$0.027                        &  \textbf{56.16} $\pm$0.028           & 62.26 $\pm$0.022        & 71.85  $\pm$0.031               & 85.07 $\pm$0.021              \\ \cline{2-8} 
    25        & 42.384 $\pm$0.040 & 49.33 $\pm$0.048 & 56.06  $\pm$0.044                & 60.25      $\pm$0.038        & 66   $\pm$0.049                 & 76.96 $\pm$0.046             \\ \cline{2-8} 
    50        & 54.72 $\pm$0.050                            & 63 $\pm$0.051                              & 61.70 $\pm$0.055    & 49.16 $\pm$0.053 & 55.41 $\pm$0.051                 & 66.54 $\pm$0.054             \\ \cline{2-8} 
    75        & 30.82 $\pm$0.062                            & 31.33  $\pm$0.063                          & 53.7  $\pm$0.065                & 51.75 $\pm$0.069             & 48.39  $\pm$0.066               & 50.125  $\pm$0.063           \\ \hline
        \end{tabular}
        }
        \caption{$\%$ Validation accuracy computed for HAR on synthetic IMU data. Valid. Acc. is computed for segmented and unsegmented validation dataset}
        \label{tab:ss}
        %\vspace{-3em}
        \end{table}
        \end{comment}

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \begin{comment}
        
    \subsection{Transfer Learning from Penn Action to PAMAP2 dataset}
        \label{subsection:TL_P_P}
         

        
        As seen in table \ref{tab:Pose_acc}, the $wF1\%$ is higher when tCNN is trained using Penn Action pose data than when tCNN is trained with synthetic IMU data. The explanation for the decrease in $wF1\%$ score is the same as that for CAD60 dataset.\\
        
        The $wF1\%$ and \% test accuracy for $tCNN_{Penn\_PAMAP2}$ is shown in table \ref{tab:tf_CP}. $tCNN_{Penn}$ is considered as the baseline. The wF1 score is highest when transferring only first two layers from Penn to PAMAP2. Thus, further experiments are performed by fixing the number of transferred layers to $c1,c2$ and varying the target data[\%].
        \begin{table}[H]
        \resizebox{\columnwidth}{!}{%
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{2}{*}{\textbf{Transferred layers}} & \multirow{2}{*}{\textbf{\%D\_t}} & \multicolumn{2}{l|}{\textbf{t}}            & \multicolumn{2}{l|}{\textbf{t}}           & \multirow{2}{*}{\textbf{p value}} \\ \cline{3-6}
                                                     &                                  & \textbf{\%wF1}       & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc} &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 69.84$\pm$0.037          & 71.60$\pm$2.69          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2,c3                                     & 100                              & 85.24$\pm$0.002          & 86.16$\pm$0.22          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        c1,c2                                        & 100                              & 86.05$\pm$0.006          & 86.94$\pm$0.50          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & -                                 \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{86.75$\pm$0.007} & \textbf{87.56$\pm$0.55} & \textbf{86.67$\pm$0.05} & \textbf{87.80$\pm$0.04} & \textbf{-}                        \\ \hline
        c1                                           & 75                               & 86.91$\pm$0.013          & 87.68$\pm$1.04          & 86.30$\pm$0.06          & 87.10$\pm$0.08          & 0.202                             \\ \hline
        c1                                           & 50                               & 84.82$\pm$0.006          & 85.91$\pm$0.50          & 84.10$\pm$0.08          & 84.98$\pm$0.07          &   0.05                                \\ \hline
        c1                                           & 30                               & 86.64$\pm$0.006          & 87.42$\pm$0.44          & 84.05$\pm$0.09          & 84.93$\pm$0.06          &   0.0                                \\ \hline
        \end{tabular}
        }
        \caption{The $wF1[\%]$ of tCNN pre-trained on Penn Action and fine tuned on target dataset  PAMAP2. The $wF1[\%]$  of the $tCNN_{PAMAP2}$ (table \ref{tab:wf1}) is considered as baseline. Numbers in bold shows the hyper-parameters which give the best $wF1[\%]$ score.}
        \label{tab:tf_PP}
        \end{table}
        \end{comment}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
          
        \begin{comment}
    \subsection{Summarizing transfer learning $tCNN_{D_{s}\_PAMAP2}$}
        Fig \ref{fig:TL_PAMAP2} and Fig \ref{fig:TL_PAMAP22} summarizes the results for Transfer Learning from all source datasets to PAMAP2. Among all the source datasets, a significant increase in $wF1[\%]$ is obtained only for $tCNN_{JHMDB\_PAMAP2}$.
       
        \begin{figure}[]
        
        \begin{center}
        \vspace{-1.8em}
        Varying the number of transferred layers
        \begin{tikzpicture}[scale=0.7]
            \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
                \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
                \begin{axis}
                    [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.23cm) rectangle (1cm,0.3cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.6, 0.9, 3.2, 5.2},
                    xticklabels={c1,(c1,c2),(c1,c2,c3),(c1,c2,c3,c4)},
                    xticklabel style={rotate=0},
        	        xlabel={Transferred convolutional layers }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.5)}, anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(.020,0.5)}},
                    ymin=68, ymax=91,
                    ytick={68,72,76,80,84,88,91},
                    nodes near coords,]
                    
                    \legend{PAMAP(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
                     \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.67)}; %A1        
                   
                    
                    \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,88.97)}; %a1
                     \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,88.45)}; %a1
                    
                    \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.61)};
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.85)};
                    
                    \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.75)};
                    
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.7,86.56)};
                    
                    %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
                    %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.67)}; %Random Forest        
                    %\addlegendentry{unseen}
            
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,88.57) }; %a2   
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,88.25)};
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,85.38) }; %a2 
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.17)};
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.05) }; %a2   
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.87)};
                    
                   
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.67)}; %SVM linear       
                    %\addlegendentry{a3}
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,87.57)}; %a3
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,88.45)};
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.06)}; %SVM linear       
                    %\addlegendentry{a3}
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.40)};
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,85.24)}; %a3            
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,88.68)};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.67) }; %Softmax 
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,87.95) }; %Softmax 
                    %\addlegendentry{a4}
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,90.98) };
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,70.72) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,69.7) };
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,69.84) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,87.99)};
                      
                    \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
                \end{axis}
        \end{tikzpicture}
        
        \end{center}
        %\vspace{-1.7em}
        \caption{The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D{S}\_PAMAP2}$. The tCNN is trained from scratch on PAMAP2 or pretrained on JHMDB, CAD60, Penn Action or pose dataset. The bars in grey colour correspond to the transfer learning performance when using the pose data as source.  $100\%$ of LARa OB dataset is used for fine tuning the pretrained model}
        \vspace{-2.5em}
        \label{fig:TL_PAMAP2}
        \end{figure}
       
        
        \begin{figure}
        \begin{center}
        \vspace{-2em}
        Varying \% PAMAP2 data
        \begin{tikzpicture}[scale=0.7]
            \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
                \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
                \begin{axis}
                    [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.5, 0.9, 2.6, 4.2},
                    xticklabels={PAMAP2 [30\%],PAMAP2 [50\%],PAMAP2 [75\%],PAMAP2 [100\%]},
                    xticklabel style={rotate=0},
        	    xlabel={\% PAMAP2 data used for tuning }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.55)}, anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(0.02,0.5)}},
                    ymin=80, ymax=91,
                    ytick={80,82,84,86,88,91},
                    nodes near coords,]
                    
                    \legend{PAMAP(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
                    \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,84.05)}; %A1        
                    %\addlegendentry{seen}
                    
                    \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,85.55)}; %a1
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,90.9)};
                    
                    \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,86.40)};
                    \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,84.87)};
                    %\node[node1, above] at ($(axis cs:8.2,0)$) {\textbf{a1}};  
                    
                    \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,86.64)};
                   \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (1.8,82.53)};
                    
                    %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.1)}; %Random Forest        
                    %\addlegendentry{unseen}
            
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,86.1) }; %a2   
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,85.57) }; %a2   
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.80) }; %a2   
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.38) }; %a2  
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.82) }; %a2   
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2,84.26) }; %a2  
                    
                    %\node[node1, above] at ($(axis cs:10.9,69)$) {\textbf{99.2\%}};
                    
            
            
                    
                    %\node[node1, above] at ($(axis cs:-4.2,70)$) {\textbf{64.3\%}};
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.2)}; %SVM linear       
                    %\addlegendentry{a3}
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.15)}; %a3
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,87.95)}; %a3
                    
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.64)}; %CAD60 75%       
                    %\addlegendentry{a3}
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.33)}; %a3
                    
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,86.91)}; %Penn 75%            
                     \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.2,85.80)}; %a3
                    
                    
                    \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.65) }; %Softmax 
                    
                    \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,88.97) }; %Softmax 
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,90.98) };
                    %\addlegendentry{a4}
                    
                    \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.61) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.85) };
                    
                    \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,86.75) }; %a4
                    \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
                    coordinates
                    { (2.4,88.68) };
                    
                    \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
                \end{axis}
        \end{tikzpicture}
        \vspace{-2.7em}
        \end{center}
        \caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_PAMAP2}$. Percent of PAMAP2 data used for fine tuning is varied.}
        \vspace{-2.5em}
        \label{fig:TL_PAMAP22}
        \end{figure}
    \end{comment}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
     Source to PAMAP2
 
 \begin{table}[]
    %\vspace{-1.5em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\textbf{$\%D_t$}}& \multicolumn{2}{l|}{\textbf{$tCNN_{CAD60_{sy}\_PAMAP2}$}}             & \multicolumn{2}{l|}{\textbf{$tCNN_{CAD60_p\_PAMAP2}$}}    & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}(Baseline)} \\ \cline{3-8} 
         Layers        &                                  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}    & \textbf{\%Test acc} & \textbf{\%wF1}    & \textbf{\%Test acc}   \\ \hline
        \textbf{$c_1$}                              & 100                              & 87.35+0.004          & 88.19+0.36          & 86.85+0.001       & 87.57+0.005           & 86.67+0.05          & 87.80+0.04          \\ \hline
        \textbf{$c_{1,2}$}                           & 100                              & 85.38+0.009          & 86.24+0.80          & 86.17+0.005       & 87.09+0.004           & \textbf{86.67+0.05} & \textbf{87.80+0.04} \\ \hline
        \textbf{$c_{1,2,3}$}                        & 100                              & 86.06+0.007          & 86.83+0.67          & 86.40+0.001       & 87.29+0.062           & 86.67+0.05          & 87.80+0.04          \\ \hline
        \textbf{$c_{1,2,3,4}$}                     & 100                              & 70.72+0.032          & 71.26+0.27          & 69.700.038        & 71.76+0.81            & \textbf{86.67+0.05} & \textbf{87.80+0.04} \\ 
        \hline
        \hline
        \textbf{c1}                              & 75                               & 86.31+0.007          & 87.19+0.75          & 86.33+0.003       & 87.20+0.27            & 86.30+0.06          & 87.10+0.08          \\ \hline
        \textbf{c1}                              & 50                               & \textbf{85.74+0.004} & \textbf{86.69+0.40} & 84.38+0.005       & 85.58+0.429           & 84.10+0.08          & 84.98+0.07          \\ \hline
        \textbf{c1}                              & 30                               & \textbf{85.77+0.005} & \textbf{86.70+0.58} & 84.87+0.002       & 85.86+0.24            & 84.05+0.09          & 84.93+0.06          \\ \hline
    
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{CAD60\_PAMAP2}$.}
    \label{tab:TL_C_PAMAP2}
    %\vspace{-2em}
\end{table}
 
\begin{table}[]
    %\vspace{-3em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf.} } & \multirow{}{}{\textbf{$\%D_t$}}& \multicolumn{2}{l|}{\textbf{$tCNN_{Penn_{sy}\_PAMAP2}$}}             & \multicolumn{2}{l|}{\textbf{$tCNN_{Penn_p\_PAMAP2}$}}    & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$}(Baseline)} \\ \cline{3-8} 
        Layers & & \textbf{\%wF1}                      & \textbf{\%Test acc}                & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        {c1}                               & 100                               & 86.80$\pm$0.004                         & 87.63$\pm$0.40                         & 87.43$\pm$0.27          & 86.56$\pm$0.002         & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1,c2}                            & 100                               &86.05$\pm$0.006 & 86.94$\pm$0.49 & 87.77$\pm$0.56          & 86.87$\pm$0.005         & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1,c2,c3}                         & 100                               & 85.24$\pm$0.002                         & 86.158$\pm$0.22                        & \textbf{89.13$\pm$0.85} & \textbf{88.68$\pm$0.02} & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1,c2,c3,c4}                      & 100                               & 69.84$\pm$0.037                         & 71.60$\pm$0.27                         & 88.92$\pm$0.27          & 87.99$\pm$0.04          & 86.67$\pm$0.05      & 87.80$\pm$0.04           \\ \hline
        {c1}                               & 75                                & 85.85$\pm$0.004                         & 86.81$\pm$0.35                         & 85.72$\pm$0.02          & 85.80$\pm$0.002         & 86.30$\pm$0.06      & 87.10$\pm$0.08           \\ \hline
        {c1}                               & 50                                & 84.58$\pm$0.006                & 85.61$\pm$0.49                & 85.26$\pm$0.09          & 84.26$\pm$0.02          & 84.10$\pm$0.08      & 84.98$\pm$0.07           \\ \hline
        {c1}                               & 30                                & \textbf{86.64$\pm$0.0058}               & \textbf{87.421$\pm$0.44}               & 83.90$\pm$0.56          & 82.53$\pm$0.02          & 84.05$\pm$0.09      & 84.93$\pm$0.06           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{Penn\_PAMAP2}$.}
    \label{tab:TL_P_PAMAP2}
    %\vspace{-3em}
\end{table}
 
 
 
\begin{table}[]
    % \vspace{-2em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf.} } & \multirow{}{}{\bm{$\%D_t$}} &\multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_{sy}\_PAMAP2}$}}             & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_p\_PAMAP2}$}}    & \multicolumn{2}{l|}{\bm{$tCNN_{PAMAP2}$(Baseline)}} \\ \cline{3-8} 
        
        Layers & & \textbf{\%wF1}                              & \textbf{\%Test acc}                         & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        {c1}                               & 100                               & \textbf{88.97+0.07}                         & \textbf{89.53+0.03}                         & \textbf{88.45+0.001} & \textbf{89.23+0.02}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1,c2}                            & 100                               & \textbf{88.57+0.05} & \textbf{89.32+0.07} & \textbf{88.25+0.006} & \textbf{89.10+0.01}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1,c2,c3}                         & 100                               & 87.57+0.06                                  & 88.51+0.07                                  & \textbf{88.55+0.01}  & \textbf{89.26+0.03}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1,c2,c3,c4}                      & 100                               & \textbf{87.95+0.06}                         & \textbf{88.98+0.05}                         & \textbf{90.98+0.03}  & \textbf{92.01+0.07}  & 86.67+0.05      & 87.80+0.04           \\ \hline
        {c1}                               & 75                                & 86.15+0.05                                  & 87.20+0.09                                  & \textbf{87.95+0.04}  & \textbf{89.10+0.03}  & 86.30+0.06      & 87.10+0.08           \\ \hline
        {c1}                               & 50                                & \textbf{86.1+0.01}                          & \textbf{86.93+0.05}                         & \textbf{85.57+0.002} & \textbf{86.60+0.02}  & 84.10+0.08      & 84.98+0.07           \\ \hline
        {c1}                               & 30                                & \textbf{85.55+0.04}                         & \textbf{86.13+0.05}                         & \textbf{90.99+0.01}   & \textbf{91.87+0.008} & 84.05+0.09      & 84.93+0.06           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics for $tCNN_{JHMDB\_PAMAP2}$. The layers are fixed at c1 for $tCNN_{JHMDB_{sy}\_PAMAP2}$ and c1,c2,c3,c4 for $tCNN_{JHMDB_p\_PAMAP2}$.}
    \label{tab:TL_J_PAMAP2}
    %\vspace{-3em}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SOurce dataset to LARAOB

\begin{table}[]
    %\vspace{-1em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_{sy}\_LARaIMU}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_p\_LARaIMU}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{LARaIMU}$(Baseline)}}      \\ \cline{3-8} 
         \textbf{Layers} &                                  & \textbf{\%wF1}       & \textbf{\%Test acc} & \textbf{\%wF1}         & \textbf{\%Test acc}   & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        c1                                                                                  & 100                              & 66.56$\pm$0.009          & 68.81$\pm$0.05          & 66.15$\pm$0.0034           & 69.59$\pm$0.389           & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1,c2                                                                               & 100                              & 66.27$\pm$0.005          & 68.50$\pm$0.04          & 65.86$\pm$0.0016           & 69.61$\pm$0.34          & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1,c2,c3                                                                            & 100                              & 66.32$\pm$0.06           & 68.52$\pm$0.06          & 65.36$\pm$0.08             & 69.06$\pm$0.08            & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1,c2,c3,c4                                                                         & 100                              & 66.76$\pm$0.01           & 68.80$\pm$0.008         & 53.97$\pm$0.0056           & 63.20$\pm$0.48            & 66.7$\pm$0.06       & 69.21$\pm$0.05           \\ \hline
        c1                                                                                  & 75                               & \textbf{66.15$\pm$0.007} & \textbf{68.74$\pm$0.03} & \textbf{65.805$\pm$0.0075} & \textbf{69.61$\pm$0.376} & 65.68$\pm$0.008     & 66.91$\pm$0.03           \\ \hline
        c1                                                                                  & 50                               & \textbf{66.65$\pm$0.08}  & \textbf{68.05$\pm$0.03} & 62.16$\pm$0.023            & 67.33$\pm$0.61            & 65.66$\pm$0.02      & 66.88$\pm$0.06           \\ \hline
        c1                                                                                  & 30                               & 65.81$\pm$0.04           & 67.65$\pm$0.01          & 57.75$\pm$0.09             & 65.11$\pm$0.07            & 65.81$\pm$0.04      & 67.05$\pm$0.02           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{JHMDB\_LARaIMU}$.}
    \label{tab:TL_J_Lara}
    %\vspace{-2em}
\end{table}



\begin{table}[]
    %\vspace{-2em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }}& \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_{sy}\_LARaIMU}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_p\_LARaIMU}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{LARaIMU}$(Baseline)}}      \\ \cline{3-8} 
        \textbf{Layers }            &                                  & \textbf{\%wF1}      & \textbf{\%Test acc}  & \textbf{\%wF1}      & \textbf{\%Test acc}  & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        c1                                       & 100                              & 69.67+0.59          & 66.33+0.01           & 69.02+0.26          & 65.03+0.005          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2                                    & 100                              & 66.76+0.77          & 61.25+0.017          & 65.12+0.21          & 62.35+0.008          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3                                 & 100                              & 65.58+0.49          & 59.01+0003           & 60.51+0.08          & 60.24+0.006          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3,c4                              & 100                              & 52.78+0.008         & 36.48+0.001          & 63.84+0.037         & 56.19+0.001          & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1                                       & 75                               & 69.30+0.30 & 65.80+0.006 & 67.07+0.81 & 61.81+0.003 & 65.68+0.008     & 66.91+0.03           \\ \hline
        c1                                       & 50                               & 66.57+0.64 & 60.99+0.014 & 66.00+0.07          & 60.20+.002           & 65.66+0.02      & 66.88+0.06           \\ \hline
        c1                                       & 30                               & 64.93+0.76          & 58.54+0.019          & 64.38+0.50          & 56.98+0.011          & 65.81+0.04      & 67.05+0.02           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{CAD60\_LARaIMU}$.}
    \label{tab:TL_C_Lara}
    ´%\vspace{-3em}
\end{table}       
        

\begin{table}[]
    %\vspace{-2em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}}& \multicolumn{2}{l|}{\boldsymbol { $tCNN_{Penn_{sy}\_LARaIMU}$}}             & \multicolumn{2}{l|}{\boldsymbol {$tCNN_{Penn_p\_LARaIMU}$}}    & \multicolumn{2}{l|}{\boldsymbol {$tCNN_{LARaIMU}$(Baseline)}} \\ \cline{3-8} 
                                      \textbf{Layers}       &                                  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}        & \textbf{\%Test acc}  & \textbf{\%wF1}  & \textbf{\%Test acc}  \\ \hline
        c1                                       & 100                              & 67.24+0.003          & 69.54+0.32           & 66.26+0.001           & 69.80+0.14           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2                                    & 100                              & 65.85+0.01           & 69.27+0.68           & 65.90+0.004           & 69.40+0.01           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3                                 & 100                              & 61.38+0.03           & 66.68+0.14           & 65.75+0.059           & 69.43+0.32           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1,c2,c3,c4                              & 100                              & 36.53+0.003          & 52.80+0.01           & 64.627+0.003          & 68.77+0.15           & 66.7+0.06       & 69.21+0.05           \\ \hline
        c1                                       & 75                               & \textbf{66.37+0.004} & \textbf{69.73+0.004} & \textbf{66.476+0.008} & \textbf{69.97+0.42}  & 65.68+0.008     & 66.91+0.03           \\ \hline
        c1                                       & 50                               & \textbf{65.66+0.006} & \textbf{69.43+0.37}  & \textbf{66.68+0.010}  & \textbf{70.365+0.66} & 65.66+0.02      & 66.88+0.06           \\ \hline
        c1                                       & 30                               & 62.37+0.20           & 67.267+0.13          & 61.07+0.022           & 66.69+0.74           & 65.81+0.04      & 67.05+0.02           \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{Penn\_LARaIMU}$.}
    \label{tab:TL_P_Lara}
    %\vspace{-3em}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SOurce to Loc

\begin{table}[]
    %\vspace{-0.5em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf.}} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_{sy}\_Loc}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{JHMDB_p\_Loc}$}}    & \multicolumn{2}{l|}{\bm{$tCNN_{Loc}$(Baseline)}}      \\ \cline{3-8} 
                                           \textbf{Layers}        &                                  & \textbf{\%wF1} & \textbf{\%Test acc} & \textbf{\%wF1}       & \textbf{\%Test acc}   & \textbf{\%wF1}       & \textbf{\%Test acc}  \\ \hline
        c1,c2,c3,c4                                  & 100                              & 74.68$\pm$0.007    & 74.95$\pm$0.005         & 79.12$\pm$0.002          & 79.51$\pm$0.002           & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2,c3                                     & 100                              & 84.99$\pm$0.01     & 85.22$\pm$0.01          & 81.24$\pm$0.004          & 82.35$\pm$0.007           & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2                                        & 100                              & 85.68$\pm$0.008    & 85.85$\pm$0.007         & 86.44$\pm$0.006 & 86.60$\pm$0.006  & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & 85.32$\pm$0.01     & 86.49$\pm$0.009         & 86.10$\pm$0.02  & 86.30$\pm$0.02   & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        c1                                           & 75                               & 85.60$\pm$0.006    & 85.82$\pm$0.009         & 85.86$\pm$0.003 & 86.17$\pm$0.003  & 85.87$\pm$0.002          & 86.17$\pm$0.002          \\ \hline
        c1                                           & 50                               & \textbf{86.03$\pm$0.01}     & \textbf{86.27$\pm$0.001}         & 83.77$\pm$0.001          & 84.12$\pm$0.001           & 84.44$\pm$0.008 & 84.61$\pm$0.007 \\ \hline
        c1                                           & 30                               & 83.04$\pm$0.007    & 83.40$\pm$0.009         & \textbf{83.97$\pm$0.003} & \textbf{84.35$\pm$0.0031} & 83.11$\pm$0.002          & 83.30$\pm$0.002          \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{JHMDB\_Loc}$.}
    \label{tab:TL_J_L}
    %\vspace{-1em}
\end{table}


\begin{table}[]
    %\vspace{-1em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_{sy}\_Loc}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{CAD60_p\_Loc}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{Loc}$(Baseline)}}      \\ \cline{3-8} 
        \textbf{ Layers} &                                  & \textbf{\%wF1} & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}       & \textbf{\%Test acc}  \\ \hline
        c1,c2,c3,c4                                                                         & 100                              & 74.98+0.007    & 73.54+0.005         & 80.60+0.15          & 80.00+0.02          & \textbf{85.38+0.009} & \textbf{85.65+0.009} \\ \hline
        c1,c2,c3                                                                            & 100                              & 78.71+0.02     & 79.68+0.016         & 84.7+0.034          & 84.85+0.53          & 85.38+0.009 & 85.65+0.009 \\ \hline
        c1,c2                                                                               & 100                              & 82.52+0.009    & 82.93+0.008         & 85.61+0.07 & 85.83+0.62 & 85.38+0.009          & 85.65+0.009          \\ \hline
        \textbf{c1}                                                                         & \textbf{100}                     & 83.92+0.007    & 84.20+0.007         & \textbf{87.27+0.02} & \textbf{87.46+0.02} & 85.38+0.009          & 85.65+0.009          \\ \hline
        c1                                                                                  & 75                               & 85.97+0.001    & 86.23+0.001         & 85.13+0.06 & 85.33+0.05 & 85.87+0.002         & 86.17+0.003         \\ \hline
        c1                                                                                  & 50                               & \textbf{85.79+0.004}    & \textbf{86.09+0.003}         & \textbf{85.88+0.03}          & \textbf{86.14+0.22}          & 84.44+0.008 & 84.61+0.007 \\ \hline
        c1                                                                                  & 30                               & 83.04+0.01     & 83.40+0.009         & 83.08+0.01 & 83.46+0.54 & 83.11+0.002          & 83.30+0.002          \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{CAD60\_Loc}$.}
    \label{tab:TL_C_L}
    %\vspace{-1em}
\end{table}


\begin{table}[]
    %\vspace{-1.5em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\bm{$\%D_t$}} & \multicolumn{2}{l|}{\bm{$tCNN_{Penn_{sy}\_Loc}$}}      & \multicolumn{2}{l|}{\bm{$tCNN_{Penn_p\_Loc}$}} & \multicolumn{2}{l|}{\bm{$tCNN_{Loc}$(Baseline)}}      \\ \cline{3-8} 
                                                                                            \textbf{Layers}       &                                  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}       & \textbf{\%Test acc}  & \textbf{\%wF1}       & \textbf{\%Test acc}  \\ \hline
        c1,c2,c3,c4                                                                         & 100                              & 68.95$\pm$0.04           & 70.46$\pm$0.20           & 64.95$\pm$0.07           & 66.85$\pm$0.07           & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2,c3                                                                            & 100                              & 71.52$\pm$0.40           & 73.41$\pm$0.06           & 82.78$\pm$0.001          & 83.16$\pm$0.001          & \textbf{85.38$\pm$0.009} & \textbf{85.65$\pm$0.009} \\ \hline
        c1,c2                                                                               & 100                              & 85.43$\pm$0.007          & 85.73$\pm$0.006          & 85.61$\pm$0.07           & 85.83$\pm$0.06           & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        \textbf{c1}                                                                         & \textbf{100}                     & 86.17$\pm$0.008          & 86.41$\pm$0.008          & \textbf{86.73$\pm$0.005} & \textbf{86.84$\pm$0.004} & 85.38$\pm$0.009          & 85.65$\pm$0.009          \\ \hline
        c1                                                                                  & 75                               & 85.41$\pm$0.009          & 85.61$\pm$0.009          & 86.39$\pm$0.02           & 86.57$\pm$0.03           & 85.87$\pm$0.002          & 86.16$\pm$0.009          \\ \hline
        c1                                                                                  & 50                               & \textbf{85.60$\pm$0.004} & \textbf{86.09$\pm$0.003} & 85.11$\pm$0.08           & 85.42$\pm$0.07           & 84.44$\pm$0.008          & 84.61$\pm$0.007          \\ \hline
        c1                                                                                  & 30                               & 83.04$\pm$0.005          & 83.50$\pm$0.004          & 83.50$\pm$0.01           & 83.88$\pm$0.02           & 83.11$\pm$0.002          & 83.30$\pm$0.002          \\ \hline
    \end{tabular}
    }
    \caption {The table summarizes the metrics obtained for $tCNN_{Penn\_Loc}$.}
    \label{tab:TL_P_L}
    %\vspace{-3em}
\end{table}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[]
\vspace{-2em}
\begin{center}
Varying number of transferred layers
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
             [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.23cm) rectangle (1cm,0.3cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.6, 0.9, 3.2, 5.2},
                    xticklabels={c1,(c1,c2),(c1,c2,c3),(c1,c2,c3,c4)},
                    xticklabel style={rotate=0},
        	        xlabel={Transferred convolutional layers }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.5)},
                    %legend style={column sep=0.01cm},
                    anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(.020,0.5)}},
                    ymin=64, ymax=88,
                    ytick={70,74,78,82,88},
                    nodes near coords,every node near coord/.append style={anchor=west,rotate=60}]
                   
                    
            \legend{Opp-Loc(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
         
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,85.65)}; %A1        
            %\addlegendentry{seen}
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.32)}; %a1
            \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.1)};
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.79)};
           \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,87.24)}; 
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.41)};
             \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,86.70)};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.65)}; %Random Forest        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.68) }; %a2   
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,86.20) };
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.88) }; %a2
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.61) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.92) }; %a2 
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,86.22) };
            
              
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.65)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,81.24)}; %a3
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,81.41)}; %a3
            
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,81.11)};       
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,84.7)}; %a3
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,72.68)}; %a3            
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,82.78)}; %a3
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,85.65) }; %Softmax 
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,76.84) }; %Softmax 
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,79.12) };
           
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,77.06) }; %a4
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,80) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,70.56) }; %a4
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,64.95) };
            
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
         
\end{tikzpicture}
\end{center}
\vspace{-2em}
\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_Loc}$. $tCNN_{Loc}$ is used as the baseline. $100\%$ of Opp-Loc dataset is used for fine tuning.}
\label{fig:TL_loc}
\vspace{-2em}
\end{figure}
 
\begin{figure}[]
\vspace{-1em}
\begin{center}
Varying \% Opp-Loc data
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
            [name=main plot,ybar,
                    every axis legend/.append style={nodes={right}},
                    legend image code/.code={%
                        \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
                    width=178mm, height=40mm,
                    axis x line=bottom, 
                    axis y line=left,
                    ymajorgrids,
                    xtick={-0.5, 0.9, 2.6, 4.2},
                    xticklabels={Loc [30\%],Loc [50\%],Loc [75\%],Loc [100\%]},
                    xticklabel style={rotate=0},
        	    xlabel={\% PAMAP2 data used for tuning }, 
                    bar width=12.5,  
                    xmin=-1.6,xmax=6,
                    legend style={at={(0.5,-0.55)}, anchor=south,legend columns=-1}, 
                    ylabel={weighted F1 [\%]}, 
                    ylabel style={align=center, at={(0.02,0.5)}},
                     ymin=80, ymax=90,
                     ytick={80,82,84,86,88,90},
                     nodes near coords,every node near coord/.append style={anchor=west,rotate=60}]
                   
                    
             \legend{LARaOB(scratch), JHMDB, $JHMDB_p$, CAD60,$CAD60_p$, Penn,$Penn_p$}
           
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.11)}; %A1        
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.04)}; %a1
            \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.97)};
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.04)};
            \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.08)};  
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.39)};
     \addplot[fill=tucol10, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.8,83.50)};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,84.44)};        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,86.03) }; %a2   
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,83.77) };
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.8) }; %CAD  
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.88) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.60) }; %a2   
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2,85.11) };
    
    
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.87)}; %SVM linear       
          
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.60)}; 
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.86)};
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.42)}; %CAD60 75%       
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.13)};
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,85.41)}; %Penn 75%            
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.2,86.39)}; %Penn 75% 
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,85.65) };  
            
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.32) }; %Softmax 
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.10) };
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.79) }; %a4
             \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,87.27) };
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.41) }; %a4
            \addplot[fill=tucol10,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.4,86.73) };
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
\end{tikzpicture}
\end{center}
\vspace{-2em}
\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_s\_Loc}$. Percent of Opp-loc data used for fine tuning is varied.}
\label{fig:TL_loc2}
%\vspace{-2em}
\end{figure}
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
SOurce to LARaMM


\begin{figure}[H]
\begin{center}
Varying number of transferred layers
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
            [name=main plot,ybar,
            every axis legend/.append style={nodes={right}},
            legend image code/.code={%
                \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
            width=150mm, height=95mm,
            axis x line=bottom, 
            axis y line=left,
            ymajorgrids,
            xtick={-0.5, 0.9, 2.6, 4.2},
            xticklabels={c1,(c1,c2),(c1,c2,c3),(c1,c2,c3,c4)},
            xticklabel style={rotate=0},
	        xlabel={No. of transferred layers }, 
            bar width=12.5,  
            xmin=-1.6,xmax=6,
            legend style={at={(0.5,-0.25)}, anchor=south,legend columns=-1}, 
            ylabel={weighted F1 [\%]}, 
            ylabel style={align=center, at={(-0.02,0.5)}},
            ymin=30, ymax=65,
            ytick={30,35,40,45,50,55,57,59,61,63,65},
            nodes near coords,]
            
            \legend{LaraMM(scratch), JHMDB, CAD60, Penn}
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,63.06)}; %A1        
            %\addlegendentry{seen}
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,58.55)}; %a1
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,55.85)};
            %\node[node1, above] at ($(axis cs:8.2,0)$) {\textbf{a1}};  
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,57.66)};
    
            
            %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,63.06)}; %Random Forest        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,55.51) }; %a2   
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,56.59) }; %a2   
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,57.32) }; %a2   
            
            %\node[node1, above] at ($(axis cs:10.9,69)$) {\textbf{99.2\%}};
            
    
    
            
            %\node[node1, above] at ($(axis cs:-4.2,70)$) {\textbf{64.3\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,63.06)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,52.90)}; %a3
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,57.95)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,59.09)}; %a3            
    
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,63.06) }; %Softmax 
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,37.07) }; %Softmax 
            %\addlegendentry{a4}
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,53.34) }; %a4
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,51.44) }; %a4
            
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
         
\end{tikzpicture}
\end{center}
\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_LaraMM}$. $tCNN_{LARaMM}$ is used as the baseline. $100\%$ of LaraMM dataset is used for fine tuning.}
\label{fig:TL_LaraMM}
\end{figure}

Fig \ref{fig:TL_LaraMM2} summarises the results for the case when the number of transferred layers is fixed at c1. The percent of LARaMM data used for fine tuning is varied. It is observed that transfer learning does not improve the performance even when LARaMM dataset is scarce. The difference between LARaOB and LARaMM is the position and number of IMUs used. Therefore, in addition to the environment in which an activity is performed the location of IMUs also affects transfer learning performance. 
\begin{figure}[H]
\begin{center}
Varying \% LARa MM data
\begin{tikzpicture}[scale=0.7]
    \tikzstyle{node1}=[text=black, font=\footnotesize \bfseries];
        \tikzstyle{node2}=[text=black, font=\normalsize \bfseries];
        \begin{axis}
            [name=main plot,ybar,
            every axis legend/.append style={nodes={right}},
            legend image code/.code={%
                \draw[####1, draw=black] (0cm,0.25cm) rectangle (1cm,0.4cm);},
            width=150mm, height=95mm,
            axis x line=bottom, 
            axis y line=left,
            ymajorgrids,
            xtick={-0.5, 0.9, 2.6, 4.2},
            xticklabels={LARaMM [30\%],LARaMM [50\%],LARaMM [75\%],LARaMM [100\%]},
            xticklabel style={rotate=0},
	        xlabel={\% LARa MM data used for tuning }, 
            bar width=12.5,  
            xmin=-1.6,xmax=6,
            legend style={at={(0.5,-0.25)}, anchor=south,legend columns=-1}, 
            ylabel={weighted F1 [\%]}, 
            ylabel style={align=center, at={(-0.02,0.5)}},
            ymin=49, ymax=64,
            ytick={49,50,51,52,53,54,55,56,57,58,59,60,61,62,63,64},
            nodes near coords,]
            
            \legend{LaraMM(scratch), JHMDB, CAD60, Penn}
            \addplot[fill=tucol8, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,52.88)}; %A1        
            %\addlegendentry{seen}
            
            \addplot[fill=tucol7, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,50.20)}; %a1
            
            \addplot[fill=tucol6, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,51.91)};
            %\node[node1, above] at ($(axis cs:8.2,0)$) {\textbf{a1}};  
            
            \addplot[fill=tucol5, error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.1,52.98)};
    
            
            %\node[node1, above] at ($(axis cs:-7.4,70)$) {\textbf{64.8\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,55.55)};        
            %\addlegendentry{unseen}
    
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,54.7) }; %a2   
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,53.50) }; %a2   
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (1.5,53.29) }; %a2   
            
            %\node[node1, above] at ($(axis cs:10.9,69)$) {\textbf{99.2\%}};
            
    
    
            
            %\node[node1, above] at ($(axis cs:-4.2,70)$) {\textbf{64.3\%}};
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,59.05)}; %SVM linear       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,55.02)}; %a3
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,57.43)}; %CAD60 75%       
            %\addlegendentry{a3}
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.0,56.13)}; %Penn 75%            
    
            
            \addplot[fill=tucol8,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,63.06) }; %Softmax 
            
            \addplot[fill=tucol7,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,58.55) }; %Softmax 
            %\addlegendentry{a4}
            
            \addplot[fill=tucol6,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,55.85) }; %a4
            
            \addplot[fill=tucol5,error bars/.cd,y dir=both,y explicit] 
            coordinates
            { (2.5,57.66) }; %a4
            
            
            \node[node2, above] at ($(axis cs:1.6,98.0)$) {\textbf{Locomotion}};
        \end{axis}
\end{tikzpicture}
\end{center}

\caption {The bar graph summarizes the $wF1[\%]$ obtained for $tCNN_{D_{s}\_LaraMM}$. Percent of LaraMM data used for fine tuning is varied.}
\label{fig:TL_LaraMM2}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
 
 \begin{table}[]
        \centering
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{|l|l|l|l|l|l|l|}
        \hline
        \multirow{}{}{\textbf{Transf. }} & \multirow{}{}{\textbf{$\%D_{t}$}} & \multicolumn{2}{l|}{\textbf{$tCNN_{JHMDB\_PAMAP2}$}}           & \multicolumn{2}{l|}{\textbf{$tCNN_{PAMAP2}$(Baseline)}}             & \multirow{}{}{\textbf{p value}} \\ \cline{3-6}
                                                     layers&                                  & \textbf{\%wF1}      & \textbf{\%Test acc} & \textbf{\%wF1}      & \textbf{\%Test acc}   &                                   \\ \hline
        c1,c2,c3,c4                                  & 100                              & 87.95$\pm$0.06          & 88.98$\pm$0.05          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & 0.005912                          \\ \hline
        c1,c2,c3                                     & 100                              & 87.70$\pm$0.06          & 88.51$\pm$0.07          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & 0.100044                          \\ \hline
        c1,c2                                        & 100                              & 88.57$\pm$0.05          & 89.32$\pm$0.06          & 86.67$\pm$0.05          & 87.80$\pm$0.04          & 0.00034                           \\ \hline
        \textbf{c1}                                  & \textbf{100}                     & \textbf{88.97$\pm$0.08} & \textbf{89.53$\pm$0.07} & \textbf{86.67$\pm$0.05} & \textbf{87.80$\pm$0.04} & \textbf{0.00002}                  \\ \hline
        c1                                           & 75                               & 86.15$\pm$0.05          & 87.20$\pm$0.06          & 86.30$\pm$0.06          & 87.10$\pm$0.08            &     0.843                              \\ \hline
        c1                                           & 50                               & 86.10$\pm$0.06          & 86.93$\pm$0.08          & 84.10$\pm$0.08          & 84.98$\pm$0.07            &        0.00004                           \\ \hline
        c1                                           & 30                               & 85.55$\pm$0.04          & 86.13$\pm$0.05          & 84.05$\pm$0.09          & 84.93$\pm$0.06            &   0.0107                                \\ \hline
        \end{tabular}
        }
        \caption{The table shows $wF1[\%]$ for $tCNN_{JHMDB\_pamap2}$. The $wF1[\%]$ and $\%$test accuracy of $tCNN_{PAMAP2}$ is used as the baseline. The number of convolution layers transferred are varied.}
        \label{tab:tf_JP}
        \end{table}
        \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> chapters/response_reviews.tex <==
\section*{Answer to Reviewers}

    We would like to thank the reviewers for their helpful comments and suggestions on the manuscript, as these led us to improve our work. Detailed responses to reviewers are given below.
    
    \subsection*{Reviewer $2353$}
    
        \begin{itemize}
            \item \textbf{Why window size of 1 second is used? What would be the scenario if authors would use 3 seconds window with 50\% overlap? Or with 0\% overlap?}

            ANSWER: \textit{We have experimented with varying step size and decided the window size based on a publication. 
            %We have added the text in section V.A.
            The duration of most activities in $D_s$ is between $0.75$ to $2$ sec. Tab.~\ref{tab:window_size} shows that for CAD60, the recognition accuracy was highest when $W=5$. However, the $wF1$ score for transfer learning from CAD60 to $D_t$ was similar for when $W=1$ and $W=5$. The results for $W=5$ are available in the repository, https://github.com/shrutarv/Create-Synthetic-IMU-data. Therefore, for generality and based on results from \cite{reining2019human}, $W=1$ is chosen for training all the $D_s$. Moreover, conclusions from \cite{banos2014window} further support the decision of choosing $W=1$. We performed experiments with step sizes $1,3,5,10,12,15,$ and $20$ and chose the one that gave the best $wF1$ score. Table \ref{tab:step_size} shows the $wF1[\%]$ for HAR on the three $D_s$: $JHMDB_{synth}$, $CAD60_{synth}$ and $Penn_{synth}$. The $W$ is fixed at $1$ and $s$ is varied.  This work aims to show that transfer learning can alleviate the scarcity of data; therefore, extensive experiments with different $W$ and $s$ are not performed. The performance on these datasets are interesting comparing with the results including video-based HAR using poses as tree-like tensors. Due to limited amount of space, these results are not included into the main document.} %window size of $0.5sec$, $1$sec, and $2$sec.
            \input{Tables/window_size}
            \input{Tables/step_size}
                
            \item \textbf{Training, validation and the testing split were across the whole dataset (for instance Opportunity dataset) or across the users? How can we generalize it?}
            
            ANSWER:\textit{We have followed the training, validation, and testing splits according to the original publications of the datasets, with fix set of users/subjects per set, i.e., the sets do not contain overlapping recordings of the same user/subject. We have included the splits in the text in section IV 2nd paragraph and under every target dataset.}
            
            \item \textbf{Why only batch gradient descent with RMS-Prop was introduced?}\\
            
            ANSWER: \textit{We have chosen this SGD with RMS-Prop based on SOA and previous exploration of different SGD approaches. Besides, we have concentrated on the primary goal of using transfer learning for solving the problem of scarcity of data as number of pages is limited. Added the text in section III.A}
            
            \item \textbf{Three different learning rates were introduced, which one showed significant performance?}\\
            
            ANSWER: \textit{We had experimented using the three learning rates and chosen the one giving the nest classification performance on the validation set---we did not include the results for each of the learning rates as number of pages is limited---, however, the repository allows for evaluating easily different training hyperparameters, see https://github.com/shrutarv/Create-Synthetic-IMU-data. We have included some explanation in text, Section III.A}
        \end{itemize}
        
        Though the results are mixed on different datasets. The proportion of Target datasets used really influenced the results, which opens new ways to explore HAR via transfer learning.
    
    \subsection*{Reviewer $2371$}
    
        \begin{itemize}
            \item \textbf{More detail regarding the synthetic data generation, and the role that the synthetic data and "raw" data from the video are needed. The way this is presented in Section III is misleading as the synthetic data is introduced as though it is being used to provide additional samples, whereas it is simulating the on-body sensors. This discussion should be clarified with detail added to allow someone else to reproduce the system}
            
            Answer: \textit{We use the second derivative of a smooth piecewise spline interpolation of degree five on a small-time interval from sequences of human joint-poses for simulating on-body devices attached to the poses, a sort of synthetic data. In line with  \cite{gurjar2018_LDRWSUWS,Moya_Rueda2020}, synthetic data could also be beneficial for transfer learning, improving performance on a limited-sized dataset. We have added the explanation in Section III. For reproducing the preprocessing, the authors make available the repository, https://github.com/shrutarv/Create-Synthetic-IMU-data.}
            
            \item \textbf{Details are on the IMU-tCNN, and how features are combined from multiple branches prior to classification, are missing. Is the IMU-tCNN the same as that shown in Fig 1? Five braches are trained (one per limb), but it's unclear what skeleton point these correspond to in the video data. It's also unclear how the branches are adapted when the target dataset does not have five IMUs (Pamap2 has devices on the ankle, hand and chest, are the other two branches just removed?). More details are needed here.}
            
            ANSWER: \textit{For all the datasets, firstly, the given pose annotations are visualised. Subsequently, the joints are mapped to the branches of \textit{IMU-tCNN}. The mapping is available in the repository, https://github.com/shrutarv/Create-Synthetic-IMU-data. However, for Penn Action, there is no clarity of the joints, as they did not form a skeleton-like figure when visualising and their joint names were not semantically clear; therefore, mapping is not possible. We have added some clarification of the mapping human limbs-branches of the architecture in Section III.A and also for all datasets in Section IV.}
            
            \item \textbf{Window size is fixed at 1s, yet datasets are captured at different sampling rates. There does seem to be resampling performed from the results tables, however any details of this (I assume that simple interpolation is used?) are missing.}
            
            ANSWER: \textit{We deploy a smooth spline interpolation of degree five on a small time-interval from a sequence of joint-pose annotations per channel. This part is  explained in Section V.A.}
            
            \item \textbf{The authors note that "Penn Action is not trained using IMU-tCNN", but it's unclear how it is trained, or used given this. This further muddies the role of the IMU-tCNN and clarification is needed here.}
            
            ANSWER: \textit{For all the datasets, firstly, the given pose annotations are visualised. Subsequently, the joints are mapped to the branches of IMU-tCNN. However, for Penn Action, there is no clarity of the joints, as they did not form a skeleton-like figure when visualising and their joint names were not semantically clear; therefore, mapping is not possible. We have added some clarification of the mapping human limbs-branches of the architecture in Section III.A and also for all datasets in Section IV.}
        \end{itemize}

    
    \subsection*{Reviewer 3349}
    
        \begin{itemize}
            \item \textbf{The methodology section is instead quite short and, in fact, I could not find a significant technical contribution, which is, to my understanding, mostly focused on the capability of achieving good performances with limited data. }
            
            ANSWER: \textit{Transferability and data exploiting from sources with domain, e.g., different domains, sensor setup, scenarios, number of subjects, different to the one of the target is still relevant, and not entirely solved. Besides, works for multichannel time-series HAR could benefit from data for video-based HAR, as the latter fuses RGB data and pose information for improving performance. Moreover, methods for semi-automated annotation, e.g., using human activity retrieval for annotating multichannel time-series HAR efficiently could also benefit from pose information. Semi-Automated methods have used pose data for boosting the annotation process deploying a model that retrieves results similar to a requested activity query. Thus, an evaluation of models for improving performance with limited data becomes handy when annotating IMU data \cite{avsar_2021}, see ARDUOUS Annotation workshop {https://text2hbm.org/arduous/}, Retrieval-based annotation of multi-channel time series data for HAR.}
            
        \end{itemize}


==> results/PAMAP2.tex <==
Tab.~\ref{tab:TL_S_Pamap2} shows the performance of the networks \textit{tCNN}$^{D_t}$ and \textit{tCNN-IMU}$^{D_t}$ on the Pamap2 dataset as target. The $\textit{tCNN}_{D_s}^{Pamap2}$ is pre-trained using the $D_s$: JHMDB, CAD60, Penn Action and NTU datasets. The performance on the Pamap2 dataset significantly increases when pre-training with the JHMDB. The \textit{tCNN}$_{JHMDB}^{Pamap2^{c1}}$ and \textit{tCNN}$_{JHMDB}^{Pamap2^{c1,c2}}$ significantly improve the HAR performance. These results suggest that the features learnt by lower layers of a \textit{tCNN} are rather generic, thus, transferable. Besides, transferring deeper layers affects the performance drastically, as deeper layers learn data-specific features. This finding can be concluded as the activity classes in CAD60 and Pamap2 are dissimilar. Considering a limited amount of dataset for training, i.e., $[10, 30, 50,75]\%$, the synthetic datasets from the three $D_s$ show a positive influence.

%Performance of the tCNN$_{CAD60}^{Pamap2}$ and tCNN$_{Penn}^{Pamap2}$ do not show major improvement with respect to tCNN$^{Pamap2}$.Besides, transferring deeper layers affects the performance drastically, as deeper layers learn data-specific features. This finding can be concluded as the activity classes among these two source datasets with the Pamap2 are dissimilar. Considering a limited amount of dataset for training, i.e., $[10, 30, 50,75]\%$, the synthetic datasets from the three source datasets show a positive influence.

\input{Tables/pamap2_cnn}

%\input{Tables/pamap2_cnnimu}

Table~\ref{tab:TL_PR} shows the precision and recall for each activity class of the Pamap2 and the shared ones in the JHMDB datasets. The \textit{tCNN}$_{JHMDB}^{Pamap2}$ using the network with the $c1$ pretrained on the synthetic on-body devices of the JHMDB and finetuned on the Pamap2. For comparing the performance of the networks, the harmonic mean (HM) of precision and recall are computed for each activity---the highest HMs are highlighted in bold. The activities \textit{Climb Stairs}, \textit{Sit}, \textit{Run}, \textit{Walk}, and \textit{Stand} are common between the Pamap2 and JHMDB. The performance of these shared activities increase. Activities that are only in Pamap2, but are semantically near to those in JHMDB, also showed a boost in performance, e.g.,  %\textit{Jump}$_{JHMDB}$-\textit{Rope Jump}$_{Pamap2}$, 
\textit{Climb Stairs}$_{JHMDB}$-\textit{Desc. Stairs}$_{Pamap2}$, 
%\textit{Desc. Stairs}$_{JHMDB}$-\textit{Climb Stairs}$_{Pamap2}$, 
\textit{Stand}$_{JHMDB}$-\textit{Ironing}$_{Pamap2}$, as person performs the activity standing and the activity is picking centred.

%The \textit{Walk} in JHMDB considers different amount of subjects with or without carrying or dragging objects in the wild. This is rather different to the constraint walking scenario in Pamap2. 

%, e.g.,  \textit{Jump}$_{JHMDB}$-\textit{Rope Jump}$_{Pamap2}$, \textit{Climb Stairs}$_{JHMDB}$-\textit{Descending Stairs}$_{Pamap2}$, \textit{Descending Stairs}$_{JHMDB}$-\textit{Climb Stairs}$_{Pamap2}$, \textit{Stand}$_{JHMDB}$-\textit{Ironing}$_{Pamap2}$, as person stands and perform picking centred.

\input{Tables/pamap2_activities}
%
